Interactive Model Cards: A Human-Centered Approach to Model Documentation

Deep learning models for natural language processing (NLP) are increasingly adopted and deployed by analysts without formal training in NLP or machine learning (ML). However, the documentation intended to convey the model's details and appropriate use is tailored primarily to individuals with ML or NLP expertise. To address this gap, we conduct a design inquiry into interactive model cards, which augment traditionally static model cards with affordances for exploring model documentation and interacting with the models themselves. Our investigation consists of an initial conceptual study with experts in ML, NLP, and AI Ethics, followed by a separate evaluative study with non-expert analysts who use ML models in their work. Using a semi-structured interview format coupled with a think-aloud protocol, we collected feedback from a total of 30 participants who engaged with different versions of standard and interactive model cards. Through a thematic analysis of the collected data, we identified several conceptual dimensions that summarize the strengths and limitations of standard and interactive model cards, including: stakeholders; design; guidance; understandability & interpretability; sensemaking & skepticism; and trust & safety. Our findings demonstrate the importance of carefully considered design and interactivity for orienting and supporting non-expert analysts using deep learning models, along with a need for consideration of broader sociotechnical contexts and organizational dynamics. We have also identified design elements, such as language, visual cues, and warnings, among others, that support interactivity and make non-interactive content accessible. We summarize our findings as design guidelines and discuss their implications for a human-centered approach towards AI/ML documentation.

==> Interactive Model Cards/tables/study_one_participants.tex <==
\begin{wraptable}{r}{0.46\textwidth}
\vspace{-5mm}
\caption{Overview of roles and expertise of participants.}
\Description{A table that shows an overview of the ten expert participants in our first study. The table has five columns : a unique ID, the participant role (or job title), their area of expertise, their familiarity with standard model cards, and their familiarity with Robustness Gym reports. The summary statistics of this table are summarized in the main text.}
\vspace{-3mm}
\scriptsize
\centering
\begin{tabular}{p{1.5em}p{10em}p{4em}p{3.5em}p{3.5em}}
\toprule
ID & Role & Expertise & SMC\newline Familiarity & RGR\newline Familiarity \\ \midrule
E01 & User Research Director & Ethics & No& No\\
E02 & AI Ethics Lead & Ethics &Y es & Yes \\ 
E03 & Ethics Data Scientist & Ethics &Yes &No \\ 
E04 & Doctoral Student - CS & Auditability&Yes &No \\ 
E05 & Doctoral Student - ML & Developer &No& No \\ 
E06 & User Research Lead & Ethics &Yes &No \\ 
E07 & Senior Researcher - NLP & NLP & Yes& Yes\\ 
E08 & Postdoctoral Fellow - NLP/HCI & NLP &No &No \\ 
E09 & Policy Research Fellow & Ethics &Yes &No \\ 
% E010 & Data Science\newline Ethnographer & Ethics & No& No\\ 
E010 & Data Ethnographer & Ethics & No& No\\ 
\bottomrule
\end{tabular}%
\vspace{-3mm}
\end{wraptable}


==> Interactive Model Cards/tables/study_one_quotes.tex <==
{\renewcommand{\arraystretch}{1.30}%
\begin{table*}[t!]
\caption{Themes from our concept studies with experts in ML/AI, NLP, ethics, and auditability. Support quotes for each theme are also presented in the interview context from which they were elicited: SMC = Standard Model Card; IMC = Interactive Model Card; RGR = Robustness Gym Report; All = general comments not directed toward any specific model card type.} %Some quotes are abbreviated to remove bridging utterances (i.e. ummm, like, so, yeah, etc.).}
\Description{A table with quotations that from the first study with ML/AI experts. The table has three columns, the last column has two nested columns. The first three columns are overall themes of the quotes, the second column has sub themes that emerged, and the last column has example quotations from the interviews. This last column is further broken down into two nested columns. The first is the context, indicates whether the participant's comment is toward the standard model card (SMC), robustness gym report (RGR), interactive model card (IMC), or all three (all). The second nested column contains the quote with the participants ID at the end. }
\vspace{-1mm}
\label{tab:studyone_tab}
\scriptsize
\centering
\begin{tabular}{p{8em}p{12em}p{3.5em}p{41.5em}}
\toprule
\textbf{Theme}     & \textbf{Subthemes} & \multicolumn{2}{l}{\textbf{Example from interviews}} \\
& & Context & Quote \\ \midrule
%% PEOPLE AND DATA WORK
\multirow[t]{4}{*}{Stakeholders} & \multirow[t]{4}{11.5em}{Stakeholders, Language} 
&SMC&\textit{``Model cards look a lot more like a summary of an academic paper compared to getting  a more general understanding of model.''} [E07]  \\ 
& &SMC&\textit{``Obviously, this, this standard model card is fantastic for an engineer who's coming in and trying to build that model [...] but [I am] not sure what their client needs.''} [E09]  \\ 
%& &SMC& \textit{``The developer has to make these model cards, but they are difficult to make, which is why these are not very informative.'' } [I07]\\ 
& &All& \textit{``There’s a lot of jargon, some of it that can be inferred, but it’s not something that is immediately apparent or made explicit'' }[E10]\\ 
& &RGR&\textit{``[Precision, recall, accuracy], those are terms that are also going to be very confusing for someone with layman's background [...] I would also say that those terms are terms of art in many ways.''} [E09]\\  \hline


%%% DESIGN
\multirow[t]{4}{7.5em}{Design Considerations} & \multirow[t]{4}{11.5em}{Information Design, Visual and Interaction Design, Implementation, Integrated Tooling}
%&SMC& \textit{``Things could be more visual, there’s too much text.''}[I06] \\
%
%&IMC&\textit{``Everything that’s standard [model card] should be its own thing, and [everything else] should be less prominent''[E07]}\\
%
%& &IMC&\textit{``I love the visualization, because it's pretty but..but what would I do [with it?]''} [I02]\\
%
&IMC&\textit{[Hovering over points in the data comparison chart] I would want to see sentences because it breaks the abstract representation into some concrete things''} [E08]\\
%
&&IMC&\textit{``It is hard to discover the interaction, so make it clearer what you get with the interactivity and make it clearer that interaction is possible.''}[E09]\\
%
%& &IMC&\textit{``The domain specifically of where these cards are deployed might alter the UI, so it would look different for ML models or even high-vs-low impact ML situations you might want different model cards.''} [E09]\\ 
& &SMC& \textit{``The developer has to make these model cards, but they are difficult to make, which is why these are not very informative.'' } [E08]\\ \hline


%%% GUIDANCE
\multirow[t]{3}{7.5em}{Guidance} & \multirow[t]{3}{11.5em}{Actionability, Defaults, Education, Explanations } 
&All&\textit{``People who aren't trained in ML don't necessarily know what they're looking out for or what questions to ask of both the data and the model  [...] nudges could be useful.''} [E04] \\
%
& &All&\textit{``Supporting analysis that says how to interpret this would be much more useful, but just even if it's formatted nicely with definitions, it's still not going to be super useful. Help me understand why this matters.''}[E02]\\
%
%& &All&\textit{``What are the examples that she [Jenn] needs to pay attention to? And kind of thing I think it would be cool to help her [Jenn] in this case [...] her build a better mental model of how the model works and, like, what it lacks.} [I04]\\
%
& &All&\textit{``I wish that this [model card] would pull [me in more]. Tell me what to look at [...] maybe you could suggest the subpopulations that I might want to look at.''} [E01] \\
%& &All&\textit{``help me understand why -- why this [information] matters.''} [I01] \\ 
&&IMC&\textit{``How much education about concepts do you need to bake in here? Do you have an intro in the beginning of this interactive model card?''}[E02]\\\hline

%%%% TRUST AND SAFETY
\multirow[t]{3}{7.5em}{Trust and Safety} & \multirow[t]{3}{11.5em}{Bias, Ethics, Misrepresentation} 
&All&\textit{``If I really am sort of coming in new to [model cards], I want to understand what my responsibility is [...] when I'm engaging with this model. I want to understand what agency I have.''} [E01]  \\
%
%& &All&\textit{``to be completely honest, I've never seen these [model cards] surface those [ethical challenges] better than actual conversations with communities that that are developing and deploying these systems''} [I08]\\
%
& &SMC&\textit{``Does this model card seem like it's showing a well-rounded representative model? Or is it one that has some big, ethical or transparent issues?''}[E03]\\ 
& &All&\textit{``Who gets to decide how to build those systems? And what is the end use case for evaluation? So in the healthcare space, specifically, a lot of times people get caught up with the area under the curve score F1 metrics for evaluating models about how they impact people's lives.''}[E09] \\ \hline
%&&RGR, IMC&\textit{``I can’t see risks for certain subpopulations, but it may give a sense of false confidence.''}[E07]\\\hline

%%%% SENSEMAKING And SKEPTICISM
\multirow[t]{4}{7.5em}{Sensemaking and Skepticism} & \multirow[t]{4}{11.5em}{Contextualization, Data Analysis, Examples, Information Seeking, Interpretation}
%&IMC&\textit{``we used visualizations in particular to help those particular customers, like explore what was going on with their data sets in their models.''} [I05] \\
%
&RGR&\textit{``[I] might not pay as much attention to it [size of subpopulation]. And that really matters because you can see some of these examples--they have high scores, but then the [...] sample size is very small.''}[E04]\\
%
& &RGR, IMC &\textit{``Just give [people] some example sentences and let them decide how they want to search or what they want to search for. And that way they can see model weaknesses and capabilities.''}[E05]\\ 
&&SMC&\textit{``Some people read all the documentation straight; others, only when [...] they run into a challenge. And so there's a lot of information [in the standard model card] so, one question is [...] how many people are going to read through all this in advance when they're actually on the job and in practice?''}[E04]\\
\bottomrule
\end{tabular}
\vspace{-6mm}
\end{table*}
}










==> Interactive Model Cards/tables/study_two_eval_quotes.tex <==
{\renewcommand{\arraystretch}{1.30}%
\begin{table*}[t!]
\caption{Themes from our evaluative studies with non-expert analyst. The reference model card represents the SMC in this study.}
\Description{A table with quotations that from the second study with non-ML/AI experts experts. The table has three columns, the last column has two nested columns. The first three columns are overall themes of the quotes, the second column has sub themes that emerged, and the last column has example quotations from the interviews. This last column is further broken down into two nested columns. The first is the context, indicates whether the participant's comment is toward the standard model card (SMC), robustness gym report (RGR), interactive model card (IMC), or all three (all). The second nested column contains the quote with the participants ID at the end. }
\vspace{-3mm}
\label{tab:studytwo_eval}
\scriptsize
\centering
\begin{tabular}{p{7.5em}p{12em}p{3em}p{43em}}
\toprule
%\textbf{Theme} & \textbf{Subtheme} &\textbf{Context}
\textbf{Theme}     & \textbf{Subthemes} & \multicolumn{2}{l}{\textbf{Example from interviews}} \\
& & Context & Quote \\ \midrule
%% PEOPLE
\multirow[t]{4}{7.5em}{Stakeholders} & \multirow[t]{4}{12em}{Community, Language, Sharing, Teams} & SMC, IMC & \textit{``Overall I am really impressed with the language clarity that is there right now, compared to [the reference model card]; the biggest difference is its clarity.''} [A2-09]\\
%& & SMC & \textit{``There's kind of the two stakeholders that I'm thinking about in this scenario. So for close internal stakeholders, I direct managers, I need a lot of those technical details for external stakeholders and internal stakeholders that are mainly just worried about the application of the model, they're going to want to know, metrics, so accuracy, precision, recall, and then examples''} [A2-04] \\
& & IMC &\textit{``We actually have had a lot of communication issues in the team  between our data science guru and the rest of the business and I think this actually might be really helpful''}[A2-02] \\
 & & IMC & \textit{``If you're trying to bring in a machine learning tool or a machine learning process, you've got to go through so many hoops to get that sign off, this is a sort of thing that would just be a godsend to have''} [A1-08]\\
 & & IMC & \textit{``This [IMC] is something that I could send in a pinch to any stakeholder. So if I was in a meeting with a whole bunch of stakeholders [...] and somebody's like, `Hey, what is the model? What does it do?' You know, I could answer most of these questions. But in a pinch, I'd say like, here's a link, go interact with it.''} [A2-04]\\ \hline
%% DESIGN
\multirow[t]{4}{7.5em}{Design} & \multirow[t]{4}{12em}{Assessment \& Validation, Comparison, Defaults, Information Priority,  Interaction, UX Patterns, Visualization} & SMC & \textit{``The first thing I am looking for is an introduction to the model and what it does and what it is used for. I don’t know if I see it here''} [A2-10]\\
& & IMC, SMC & \textit{``So, interactivity is the main one. This is more of an all or one, whereas the [SMC] makes me use another tool. It [SMC] is more like a shopping mall, where I need build it [the analysis] on my own at home.''} [A1-03]\\
& & IMC, SMC & \textit{``You want it all accessible, the fact that it’s one page is great. Like with the other one I had to click around a lot to get the information, but this model card doesn’t have that problem, which is great.''} [A2-02]\\ 
& & IMC & \textit{``It gives me a good outline of what I am looking at. The few examples, short, sweet, and to the point are helpful.''}[A1-07]\\
%& & SMC & \textit{``I would loose my patience after 30-40 seconds [if] I have to put a lot of effort into what I am looking for, I would start to search somewhere else.''} [A2-06]\\
&& IMC & \textit{``Maybe it’s my time working in finance, but bullet points work for me''} [A2-02] \\ \hline
%% SENSEMAKING
\multirow[t]{4}{7.5em}{Sensemaking \newline\& Skepticism} & \multirow[t]{4}{12em}{Awareness, Confidence, Contestability, Examples, Exploration, Prompts, Warnings, Risk Group Analysis} &  SMC, IMC  & \textit{``It [SMC] seemed more oriented towards somebody who wants to, like develop and train it [the model] and deploy it [...] this [IMC] does give me the same information, like it gives me the same context [...] but it's also giving me the tools to kind of look at the model on a higher level.''} [A2-04] \\ 
& & IMC &  \textit{``I absolutely like this quantitative analysis [...] which lets me play around, and I can see whether the model is working or not. So I'm not just taking the the word of the developer of the library''} [A2-09] \\
& & SMC, IMC & \textit{``if I ever see something that just reports one metric [...] I'm always like a little bit skeptical that maybe they just picked that up because that's what looks good''}[A2-01]\\
& & IMC & \textit{``I do like the fact that you can [...] agree or disagree [with the model's prediction], because sometimes it's nice to have that ability} [A1-06] \\ \hline
%% UNDERSTANDABILITY
\multirow[t]{4}{7.5em}{Understandability \newline \& Interpretability} & \multirow[t]{4}{12em}{Accessibility, Clarity, Data Understandability, Guidance, Model \& Result Interpretation, Information Overload, Information Sufficiency, Trust} & IMC & \textit{``This gives me more assurance that this is the right model or not''} [A2-09] \\
& & SMC &  \textit{``I can tell it, it's used for some text classification[...] But, in terms of what this thing does, it's not obviously intuitive enough, unless you've caught some context around it. So I filled in a lot of the blanks.'' }[A2-08] \\
& & SMC & \textit{``What is the sentiment treebank [SST-2 dataset]? Like, is it a list of sentences? Where did they come from? Who generated them? Because that was also what I was confused''} [A2-01] \\
& & SMC & \textit{I feel that it’s too much information on this model. If, maybe, could I  have a better summary?} [A1-10]\\
& & SMC & `\textit{`The most important bit is what the purpose of the model is, and it’s good at the top, otherwise I didn’t know what what I was looking at, I had to guess how it actually works and what is trying to tell me''} [A2-05]\\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}
}


%So if I was to come in here and be like, cool, I've got a data set that I want to run sentiment analysis on, I'm going to use this model, drop it into my CSV, boom, now I want to see the visualizations great. And they're going to look really good when I'm presenting to my boss. But then I kind of need the actual, like factual information that I can hand over to my team where I'm like, This is why we're doing it his his what the analysis brought to life.

==> Interactive Model Cards/tables/study_two_eval_quotes_tmp.tex <==
{\renewcommand{\arraystretch}{1.30}%
\begin{table*}[t!]
\caption{Study TWO themes.}
\label{tab:studytwo_eval}
\scriptsize
\centering
\begin{tabular}{p{8em}p{12em}p{3.5em}p{41.5em}}
\toprule
%\textbf{Theme} & \textbf{Subtheme} &\textbf{Context}
\textbf{Theme}     & \textbf{Subthemes} & \multicolumn{2}{l}{\textbf{Example from interviews}} \\
& & Context & Quote \\ \midrule
tooling & & IMC, SMC & So, interactivity is the main one. This is more of an all or one, whereas SMC makes me use another tool. So I feel like [SMC] is more like a shopping mall, where I need build it on my own at home. [A1-03]\\
stakeholder & & SMC & It seemed more oriented towards somebody who wants to, like develop and train it and deploy it [...] this [IMC] does give me the same information, like it gives me the same context [...] but it's also giving me the tools to kind of look at the model on a higher level. [A2-04] \\
& & IMC & [If] I can integrate [the IMC] with my current readme files, or the DevOps infrastructure, I would take that. [A2-09]\\
structure & & & \textit{``It’s much better, before I was confused I didn’t know what was going on. At least now there is a structure.''} [A2-05]\\
& & IMC & ``Overall it’s easier to find things here, everything is one page which is nice, you don’t have to to go the website to find it.'' [A2-10] \\ & & SMC & ``I would loose my patience after 30-40 seconds, I have to put a lot of effort into what I am looking for, I would have to search somewhere else. [A2-06]\\
& & IMC, SMC & `` So for the hugging face model card, I would want to see more about how it can be manipulated. For the Interactive model card, I feel like it needs to drill into it more.'' [A1-07]\\

&& IMC &``Overall I am really impressed with the language clarity that is there right now, compared to what it was earlier. If I just have to inform what the biggest difference is, its clarity.'' [A2-09]\\

&& IMC & The first thing I am looking for is an introduction to the model and what it does and what it is used for. I don’t know if I see it here [A2-10]\\
&& SMC & \textit{`` this is very technically focused, and very focused on the model and not why does this model exist''} [A1-03]\\

&& SMC &  ``I know what I am looking for, but I couldn’t show this to management [... ]we would always add something ontop [A1-06]\\
&& SMC & `\textit{`the most important bit is what the purpose of the model is, and it’s good at the top, otherwise I didn’t know what what I was looking at, I had to guess how it actually works and what is trying to tell me''} [A2-05]\\
%&& IMC & \textit{``A huge win would be getting this to integrate seamlessly with open-source frameworks'' }[A2-01] \\
&& SMC& \textit{``It would be more like playing a game but would be interested to gauge how this works''}[A1-01]\\
& & IMC &  I absolutely like this quantitative analysis and are short, which let me play around, and I can see whether the model is working or not. So I'm not just taking the the word of the developer of the library [A2-09] \\
&& IMC & ``I want to be able to actually get the model somehow, so make it clearer that you can download or use the model''[A2-01] \\
&& IMC & \textit{``I think the other one [SMC] the code listed. I don't think this [IMC] has the code, anywhere. But that's probably another  strength slash weakness''} [A1-04]\\

% Data
%% 
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}
}





==> Interactive Model Cards/tables/study_two_participants.tex <==
{\renewcommand{\arraystretch}{1.15}%
\begin{table}[t!]
\caption{Overview of Participants for the Second Study.}
\Description{A table summarizing the demographics of participants in our second study. The table was 8 columns. The first two columns concern the study details, with one column providing the participant's study ID and the second showing the category of analyst they are (Analyst I or Analyst II). The next four columns give background details on the participant; the columns in order have the participants' regions (Canada, US, UK, or others), their role (or job title), their industry, and the size of their organization. The final two columns concern the participants skills and proficiency with ML/DS and sentiment analysis, respectively. }
\vspace{-3mm}
%All participants reported on the job training as their highest level of CS, ML, or Data Science training. The two categories of analyst (type I and II) are determined by the criteria described in ~\autoref{fig:phaseII_criteria}.}
\scriptsize
\begin{tabular}{p{2.5em}p{4em}p{7em}p{13em}p{12em}p{5em}p{5em}p{4em}}
\toprule
\multicolumn{2}{l}{\textbf{Study Data}} & \multicolumn{4}{l}{\textbf{Background Details}} & \multicolumn{2}{l}{\textbf{Skills and Proficiency}} \\ 
ID & Category & Region & Role & Industry & Org. Size & ML/DS\newline Proficiency & Sentiment \newline Analysis\\ \midrule
% BUSINESS SCIENTIST I
A1-01 & Analyst I& United States &Business and Marketing Analyst& Media &10000+& Basic& No\\
A1-02 & Analyst I& Canada & Project Manager & Finance &5001-10000& Basic& No\\
A1-03 & Analyst I& United Kingdom &Product Analyst& Insurance &201-1000& Limited& Yes\\
A1-04 & Analyst I& United States &Finance Director& Finance &10000+& Limited& Yes\\
A1-05 & Analyst I& United States &Product Analyst& Finance &10000+& Basic& No\\
A1-06 & Analyst I& United States &Business Analyst & Information Technology &1001-5000&Advanced& No\\
A1-07 & Analyst I& United States &Project Analyst& Environmental Services &1001-5000& Basic& No\\
A1-08 & Analyst I& United Kingdom &Automation Developer& Information Technology &201-1000& Basic& No\\
A1-09 & Analyst I& Canada &Business Data Analyst& Finance &5-200& Basic& Yes\\
A1-10 & Analyst I& South Africa &Business Intelligence Analyst& Finance &1001-5000& Basic& No\\  \hline
% BUSINESS SCIENTIST II
A2-01 & Analyst II& United States &Data Scientist & Government&10000+& Advanced& Yes\\
A2-02 & Analyst II& United Kingdom &Analytics Manager & Marketing \& Advertising &51 - 200& Advanced & Yes\\
A2-03 & Analyst II& United States &Machine Learning Researcher& Material Engineering &1001-5000&Advanced & Yes\\
A2-04 & Analyst II& United States &Machine Learning Developer& Information Technology &51-200& Advanced& No\\
A2-05 & Analyst II& Canada &Business Data Scientist& Telecommunications &10000+& Advanced& Yes\\
A2-06 & Analyst II& United Kingdom &Business Analyst& Finance &1001-5000& Advanced& Yes\\
A2-07 & Analyst II& United Kingdom &Data Analyst& Information Technology &201-1000& Advanced& Yes\\
A2-08 & Analyst II& United States &Data Engineer & Education &51-200& Advanced& Yes\\
A2-09 & Analyst II& United States &VP Data \& Analytics & Education &51-2000& Advanced& No\\
A2-10 & Analyst II& Canada &Analytics Solutions Developer& Retail&1001-5000& Expert&No\\
\bottomrule
\end{tabular}
\vspace{-5mm}
\label{tab:study_two_participants}
\end{table}
}

==> Interactive Model Cards/tables/study_two_prompts.tex <==
{\renewcommand{\arraystretch}{1.30}%
\begin{table*}[t!]
\caption{Examples of participant responses on the usability, functionality, safety, and ethics of the IMC.} %When asking participants to reflect on the dimensions of safety and ethics, we explicitly prompted all participants with the definitions below (additional details in the full study protocol \hl{OM\#}). All quotes are in reference to the interactive model card prototype.}
\Description{A table with three columns that summarizes participants response to specific prompts on  usability, functionality, safety, and ethics of the IMC. The first column indicates the prompt, the second has the definition of the prompt, and the third has example quotes from the second study. }
\vspace{-3mm}
\label{tab:studytwo_prompts}
\scriptsize
\centering
\begin{tabular}{p{4.5em}p{10em}p{50em}}
\toprule
%\textbf{Theme} & \textbf{Subtheme} &\textbf{Context}
\textbf{Prompt}     & \textbf{Definition} &\textbf{Example from interviews} \\
\midrule
%%%%%%%%%% USABILITY 
\multirow[t]{3}{4em}{Usability} & \multirow[t]{3}{10em}{The efficacy of the design choices to help assess and digest the information in the model card} &  \textit{``This feels like plain English [...] like a very simple way of saying, `hey, this is what we have. this is what it does.' '' }[A1-01] \\
&& \textit{``I think this [IMC] tells a better story, [...] and this tells me, what's the model? What's it supposed to be used like?''} [A2-08] \\
& & \textit{``It's not only the numbers, but it's also the insights and  visually being able to see[...] what those numbers are saying''} [A2-04] \\
& &  \textit{``The visualization, as far as the reporting goes, it has got a good description of what all that means. A lot of the help text and description text is there.'' }[A1-06] \\ \hline
%%%%%%%%%% FUNCTIONALITY
\multirow[t]{3}{4em}{Functionality} & \multirow[t]{3}{10em}{The ability to use the IMC to assess the relevance and applicability of the model to their routine work}&  \textit{``This would be perfect for internal stakeholders, like technical stakeholders, direct managers, CTO, data science team, you know, people like that. I would want a simplified version of this for external stakeholders. But I also have all the data here and it looks like I can extract it if I want to.''} [A2-04] \\ 
&&\textit{``If I had a tool like this, I would start to explore, and pick out trends or phrases, in their data, so that I can start to see that there are opportunities from a features development perspective.''}[A1-03]\\
& & \textit{``I've got a data set that I want to run sentiment analysis on, I'm going to use this model, drop it in through my CSV, boom, now I want to see the visualizations great. And they're going to look really good when I'm presenting to my boss.''}[A1-03]\\
&&\textit{``It [the model card] would be more about ruling out that it's not the right model, you know, and then I might have like six or seven model cards open, as I'm going through all the models, I can find, like, here's my list of things we should try.''}[A2-07]\\ \hline
%%%%%%%%%% SAFETY
\multirow[t]{4}{4em}{Safety} & \multirow[t]{4}{10em}{The ability to assess safety risks for a model, including risks for security, privacy, robustness, and related dimensions} &  \textit{``I think it [the IMC] gives you the basis to have that conversation.''}[A2-02] \\
& &\textit{``It is the person’s responsibility to make sure they know what they are doing and not someone who is providing the model to them.'' }[A2-06] \\ 
& & \textit{``The safety risk is more in the problem itself and not the model you are applying.''} [A2-07] \\ 
& & \textit{``With the protected classes I think it’s a good feature to have, I think it’s one of the more important ones. Protected classes make me think that things are headed in the right direction. Also I like the warnings.''} [A2-08] \\
\hline
%%%%%%%%%% ETHICS
\multirow[t]{4}{4em}{Ethics} & \multirow[t]{4}{10em}{The ability to assess ethical consequences encompassing things like potential harm to vulnerable people or ecosystems, unintended bias, or similar issues}  &  \textit{``I think it's useful as well to say, `You know, what, you're gonna have to go and do your own research' [...] you can't just say `Oh, just go and read this.'[Use the] model card to assist you, but you're going to have to go and do a bit of learning yourself.''} [A1-08]\\
&&\textit{``I don’t think it helps me with ethical consequences, but it helps to give me some considerations.''} [A1-03]\\
& &\textit{``I think also having these categories [protected classes] made me curious and think about it.''} [A1-09]\\
&& \textit{``Bias is also like a term of art in machine learning, right? So it's like, I read it as bias, like, Oh, it's just talking about bias from the standpoint of overfitting. It has nothing to do with like, discrimination and ruining people's lives.''}[A2-07] \\
\bottomrule
\end{tabular}
\vspace{-6mm}
\end{table*}
}


==> Interactive Model Cards/tex/abstract.tex <==
\begin{abstract}
Deep learning models for natural language processing (NLP) are increasingly adopted and deployed by analysts without formal training in NLP or machine learning (ML). However, the documentation %intended to support 
% these non-expert analysts
%tuning and deploying these models
intended to convey the model's details and appropriate use 
is tailored primarily to individuals with ML or NLP expertise. To address this gap, we conduct a design inquiry into \textit{interactive model cards}, which augment traditionally static model cards with affordances for exploring model documentation and interacting with the models themselves. Our investigation consists of an initial conceptual study with experts in ML, NLP, and AI Ethics, followed by a separate evaluative study with non-expert analysts who use ML models in their work. Using a semi-structured interview format coupled with a think-aloud protocol, we collected feedback from a total of 30 participants who engaged with different versions of standard and interactive model cards. Through a thematic analysis of the collected data, 
% we identified several conceptual dimensions (stakeholders; design; guidance; understandability \& interpretability; sensemaking \& skepticism; and trust \& safety) that summarize the strengths and limitations of standard and interactive model cards.  
we identified several conceptual dimensions that summarize the strengths and limitations of standard and interactive model cards, including: stakeholders; design; guidance; understandability \& interpretability; sensemaking \& skepticism; and trust \& safety.  
Our findings demonstrate the importance of carefully considered design and interactivity for orienting and supporting non-expert analysts using deep learning models,
% , also considering 
along with a need for consideration of
broader sociotechnical contexts and organizational dynamics. We have also identified design elements, such as language, visual cues, and warnings, among others, that support interactivity and make non-interactive content accessible. We summarize our findings as design guidelines and discuss their implications for a human-centered approach towards AI/ML documentation.
% Deep learning models for natural language processing (NLP) are increasingly being adopted and deployed by analysts without formal training in NLP or machine learning (ML). However, the documentation intended to support these non-expert analysts is tailored primarily to individuals with ML or NLP expertise. Using model cards as a scaffold, we conduct a design inquiry to explore whether adding interactivity to model cards can address this gap. Our investigation consists of an initial conceptual study with experts in ML, NLP, and AI Ethics, followed by a separate evaluative study with non-expert analysts who use ML models in their work. We recruited 10 and 20 participants for each study phase, respectively, and asked them to engage with different versions of a standard and interactive model card. We used a semi-structured interview format coupled with a think-aloud protocol to collect participants' impressions and reflections. A thematic analysis of these data resulted in conceptual dimensions that summarize the strengths and limitations of standard and interactive model cards. These dimensions include considerations toward stakeholders, design, guidance, understandability \& interpretability, sensemaking \& skepticism, and trust \& safety. Compared to experts, the non-expert analysts articulated with greater nuance the role of model cards as a sociotechnical artifacts for sharing information across organizations. Moreover, their feedback highlighted the relationship between design and the effectiveness of model cards, both standard and interactive, to serve this sociotechnical role. Our findings demonstrate the importance of carefully considered interactivity for orienting and supporting non-expert analysts using deep learning models. We also identified design elements, such as language, visual cues, and warnings, among others, that support interactivity and make non-interactive content accessible. We summarize our findings as design guidelines and discuss their implications toward a human-centered approach towards AI/ML documentation.
\end{abstract}





%We recruited 30 participants across both studies and conducted semi-structured interviews that asked them to engage with and reflect upon versions of a standard and interactive model card.

%%%%% OLDER VERSIONS %%%%%%%

%v4
%Deep learning models for natural language processing have become easier to use and more widely available. Consequently, they are increasingly being adopted and deployed by people without formal training in machine learning, linguistics, or statistics. However, the documentation developed to describe details, contexts of intended use, and other relevant considerations for these models is tailored mainly toward individuals with such formal training while non-expert users remain underserved. In this work, we use the concept of a model card to scaffold design inquiry into documentation for large-scale language models. Our investigation comprises two studies. The first was a formative study conducted with ten individuals who have expertise in AI ethics, auditability, AI/ML development, or NLP. We asked participants to reflect on the value and limitations of three model card design probes with consideration for their own needs as experts and with concern for users' needs without formal ML or NLP training. Synthesized findings from this study guided our design for an interactive model card, which we evaluated in our second study. For the second study, we recruited 20 participants who use AI/ML models in their work but who do not have any formal training. We asked participants to engage with an existing model card and with our interactive model card in a think-aloud protocol. The studies generated 34 hours of interviews for analysis. Our findings validate some design patterns in existing model cards but also highlight the limitations for non-expert AI/ML users. In this work, we present design recommendations surfaced through these studies, and we articulate broader implications for a more human-centered approach towards documentation of AI/ML systems.
%\vspace{1mm}  
%\noindent\textbf{Availability of Code and Supplemental Materials:} %\url{https://osf.io/9d83t/?view_only=7359695185b04468a7ae4a2e189691c0}

%V3

%The increasing ease of use and availability of deep learning models for natural language processing have led to broader adoption and deployment by people without formal training in machine learning, linguistics, or statistics. However, we contend that much of the model documentation created to describe the details, intended uses, and other considerations of these models are largely tailored toward individuals that do have such formal training. For example, model cards with their goal of defining intended use cases are bespoke documentation for domain experts, and ML experts and non-expert users remain largely under-served. Here, we use model cards as a scaffold for a design critique of documentation for large-scale language models. We take a human-centered lens to compare and contrast model cards, robustness reports, and a novel concept for an interactive model card. Our investigation comprises two studies. The first was an interview and abbreviated concept study with ten individuals with expertise in AI ethics, auditability, ML/AI development, and NLP. Within a semi-structured interview format, these individuals were prompted with three design probes for a sentiment analysis model. They were asked to consider the design of the probes, both from their personal use of model documentation and then from the perspective of a potential end-user that does not have an ML background. We conducted a thematic analysis of the transcripts and notes from these hour-long sessions. The results were used to redesign the interactive model card concept. In a second study, we recruited 20 individuals that were self-taught ML/AI learners, but that applied this technology in their daily work. These participants were presented with interactive versions of a model card and our concept. Participants were prompted to explore the model cards and think out loud about their experience. They were also prompted with specific questions about their functionality, operationalizability, safety, and ethics. We again conducted a thematic analysis on interview transcripts and notes. Our findings support some design choices of existing model cards, but largely also highlight their limitations for non-ML/AI experts. Our research and it’s findings have implications for making model documentation more human-centered and accessible to a wider pool of people that use NLP models.

% V2

%As deep learning models for natural language processing have become easier to use and more widely available, they are increasingly being adopted and deployed by people without formal training in machine learning, linguistics, or statistics. However, the documentation developed to describe details, intended use contexts, and other relevant considerations for these models is largely tailored toward individuals that do have such formal training. For example, model cards and similar artifacts can provide consistent summaries of model details, but the burden is on model developers to create bespoke artifacts, and some categories of information--such as disaggregated quantitative analysis--are prohibitively labor intensive to produce. Moreover, the forms these model cards have taken generally target domain experts, while other ML practitioners and non-expert users remain underserved. In this work, we use the concept of a model card to scaffold design inquiry into documentation for large-scale language models. We apply a human-centered design lens to examine the affordances, opportunities, and limitations for standard model cards, robustness reports, and for our novel concept for an interactive model card. Our investigation comprises two studies. The first was a formative study conducted with ten individuals who have expertise in AI ethics, auditability, AI/ML development, and/or NLP. Following a brief semi-structured interview about participants’ backgrounds, we asked them to engage in a think-aloud protocol with three model card design probes for a sentiment analysis model. We asked participants to reflect on the value and limitations for each probe with consideration for their own concerns as experts and with concern for the needs of users without formal ML or NLP training. Synthesized findings from this study guided our design for an interactive model card, which we evaluated in our second study. For the second study, we recruited 20 participants who use AI/ML models in their work but did not have any formal training. We asked participants to engage with an existing model card and with our interactive model card in a think-aloud protocol. We concluded the session with a semi-structured interview to capture participants’ perspectives on how these model cards helped them understand the model’s functionality, operationalizability, safety, and potential ethical risks. Our findings validated some design patterns in existing model cards but also highlighted the limitations for non-expert AI/ML users. In this work, we present design recommendations surfaced through these studies, and we articulate broader implications for the documentation of AI/ML systems.

% V1
%The ease of use and availability of deep learning models for natural language processing are increasingly used and deployed by people without formal training in machine learning, linguistics, or statistics. However, we contend that much of the model documentation created to describe the details, intended uses, and other considerations of these models are largely tailored toward individuals that do have such formal training. For example, model cards with their goal of defining intended use cases are bespoke documentation for domain experts, and ML experts and non-expert users remain largely under-served. Here, we use models cards as a scaffold for a design critique of documentation for large-scale language models. We take a human-centered lens to compare and contrast model cards, robustness reports, and a novel concept for an interactive model card. Our investigation comprises two studies. The first was an abbreviated concept study that recruited ten individuals with expertise in AI ethics, auditability, ML/AI development, and NLP. Within a semi-structured interview format, these individuals were prompted with three design probes for a sentiment analysis model. They were asked to consider the design of the probes, both from their personal use of model documentation and then from the perspective of a potential end-user that does not have an ML background. We conducted a thematic analysis of the transcripts and notes from these hour-long sessions. The results were used to redesign the interactive model card concept. In a second study, we recruited 20 individuals that were self-taught ML/AI learners, but that applied this technology in their daily work. These participants were presented with interactive versions of a model card and our concept. Participants were prompted to explore the model cards and think out loud about their experience. They were also prompted with specific questions about their functionality, operationalizability, safety, and ethics. We again conducted a thematic analysis on interview transcripts and notes. Our findings support some design choices of existing model cards, but largely also highlight their limitations for non-ML/AI experts. Our research and it’s findings have implications for making model document more human-centered and accessible to wider pool of people that use NLP models.


==> Interactive Model Cards/tex/background.tex <==
% \section{Making the Case for Interactive Model Cards}
\section{Motivation}
\hl{I think we actually address these with sufficient depth in the intro and related work and it would be hard to extract what is intro vs. motivation/background in particular. Keeping this as a placeholder for now.}

These are the questions that this section should aim to answer:

\begin{itemize}
    \item What are the limitations of existing model cards
    \item Why do we need interaction in model cards?
    \item Is this just a dashboard?
    \item Who are these for? 
\end{itemize}


This paper also supports our motivation fairly clearly: Explainable machine learning in deployment~\cite{bhatt10.1145/3351095.3375624}

==> Interactive Model Cards/tex/conclusion.tex <==
\vspace{-3mm}
\section{Conclusion}
Together with ML/AI experts and non-experts, we co-developed a concept and functional prototype for an interactive model card for a large language model. %Our findings emphasize the important of a deliberate, design processes to ensure model cards are interpretable, usable, and relevant to a broad group of stakeholders. %These findings also underscore the value of interaction to promote productive skepticism and demonstrate the value of model cards within existing sociotechnical systems. 
%Through two complimentary studies with experts and non-experts in ML/AI or NLP, respectively, we have developed and assessed a functional prototype of an interactive model card. Our thematic analysis of over 34 hours of transcript texts reveal important conceptual dimensions that describe not only how participants respond to different elements of the interactive model cards designs and its overall strengths and limitations, but also its sociotechnial value to individuals and their organizations.
Within the broader range of stakeholders using and deploying NLP and other ML/AI models, our work presents a timely and important examination of model cards from a human-centered design perspective. 
% We foresee future opportunities for other ML/AI researchers, practitioners, and developers to build from our findings to ensure that large language models, and other types of machine learning models, are responsibly created and deployed.
We foresee future opportunities for other researchers, practitioners, and developers to build from our findings to ensure that 
% large language models--and other ML/AI models--
ML/AI models
are interrogable, contestable, and documented responsibly.


==> Interactive Model Cards/tex/discussion.tex <==
\vspace{-3mm}
\section{Discussion}\label{sec:discussion}
Technology that enables low or no code data analysis is lowering barriers to developing and deploying deep learning models. As E02 astutely observed (Section~\ref{study_one:res_stakeholders}), the net effect is to broaden 
% the diversity of analysis and 
the field of
stakeholders who will need access to model cards in the future. 
% While these individuals may routinely use ML or deep learning models in their work, they are unlikely to have a formal education related to the theoretical and technical underpinnings of these models. We posited that, for this group, the inclusion of interaction to the existing structure of a model card would help them engage with model's information -- and especially with large scale language models.
Increasingly, the data workers taking on AI/ML development do not have formal education in the theoretical and technical underpinnings of these systems. We posited that, for this group, augmenting model cards with interactivity would make AI/ML systems 
% (especially large language models) 
more interpretable.

% In our research, we have 
We
recruited and explored the perspectives of people who we believe are representative of the future data workforce. Our findings show that 
% adding interaction to 
interaction in
model cards helped participants better understand 
% what the ML model does and how they can use it in their work. 
model behavior and implications for their work.
Critically, the benefits of interaction were realized primarily through the careful architecture of information that included the choice of data visualizations, 
% information hierarchies, 
layout, language, visual cues, warnings and prompts. 
% While the original proposal for model cards~\cite{mitchell10.1145/3287560.3287596} does not exclude such design elements, we take the more prescriptive stance 
% that without them model cards are inaccessible to many who use deep learning models in their work. Moreover, our findings go further by showing that sociotechnical uses of model cards are deeply intertwined with the value stakeholders place on model cards.  
We contend that without these careful design choices, model cards are inaccessible to many individuals who use AI/ML models in their work. 
Our studies have also surfaced the value proposition data workers identify for model cards to support organizational decision-making and traceability.
% as communicative artifacts within sociotechnical systems. 
From our collective findings we draw four key insights:

\vspace{1mm}
\noindent\textbf{1) Interactive model cards are a bridge to further analysis, not a substitute.} 
% What is the right level of interaction to add to a model card and at what point does cross-over to being a light-weight analysis interface? 
% This was balance that we considered in our study, and a topic that participants challenged us on. 
How interactive should a model card be? At what point does it cross over into an analysis interface?
In designing the IMC, we wrestled with these questions, and study participants were divided on the appropriate balance.
% We argue with tactical and considerate inclusion of interaction, 
% model cards can serve a more productive role in eliciting worthwhile analysis directions.  
We argue that with thoughtfully designed interaction, model cards can be a first step for data workers to explore how trustworthy a model is and whether it might meet their needs, serving as a guide to deeper interrogation when desired.
% The extend and modalities of interaction for model cards remains an open problem, and future research directions can probe the effects of these design decisions on factors of model and data understandability, interpretability, and actionability.
For individual stakeholders, the most effective form for interactivity in model cards will be situated and contextual. 
However, future research could deepen our understanding of how particular design decisions impact the understandability and actionability of model cards.

\vspace{1mm}
% \noindent\textbf{2) Productive skepticism is bolstered by guidance.}
\noindent\textbf{2) Interactivity and guidance bolster productive skepticism.}
% Interaction allows participants to frame the information in a context that is relevant to them, 
Interaction supports individuals in contextualizing and interrogating model behavior (e.g., by adding their own data or contesting the model's results). The opportunity to \textit{``be really curious to just kind of play around''} [A2-05] can help mitigate anchoring bias~\cite{Nourani:anchoring:2021}. 
% A productive form of skepticism, which is neither overly dismissive and nor trusting, may be encouraged through interaction with the model and the data. Importantly, our findings point to the importance of scaffolding these interactions with appropriate guidance that help orient
% % the analyst, or their stakeholder, in the
% individuals to the
% information they are consuming. Our research has only scratched the surface of what this guidance looks like and the effects it has on the ways people create mental constructs of the model and data. 
This sort of interactivity may encourage \textit{productive skepticism,} an orientation that is neither overly dismissive nor trusting.
Importantly, we found that scaffolding these interactions to support sensemaking requires clear and actionable guidance.
Our research has only scratched the surface of the dimensions and forms of guidance that help people understand and act on model behavior.
There remain many avenues to explore with IMCs as a foundation for this inquiry.

\vspace{1mm}
\noindent\textbf{3) Model cards should support the data work community, not just an individual.} Decision-making with data and deep learning models 
% involves multiple individuals sharing information with each other over time and across organizational processes. 
is a collaborative and distributed process involving information sharing over time and across organizational roles. 
% Diverse stakeholders occupy different roles and bring different expertise and perspectives. 
% Developing model cards in way that they can be shared across these groups, is integral to their adoption. 
For model cards to be adopted and impact organizational processes, they must support knowledge sharing and negotiation across  stakeholders with diverse backgrounds and perspectives.
% To further reduce some of the overhead an burden of creating model cards, collaborative modes of co-development and integration with programmatic tooling should be explored. 
% Such collaborative engagements can allow for the reuse and refinement of model card components. 
Furthermore, the creation of interactive model cards need not be so burdensome. Our findings suggest that collaborative development, along with integrated programmatic tooling, could lower the burdens for model card generation, reuse, and refinement.
% Moreover, there may even be mechanisms to collectively distribute these refinements rather than relying on an individual to make the modifications, for example, to improve the use of jargon or visual cues. 
 

\vspace{1mm}
\noindent\textbf{4) Unintended uses, ethics, and safety are too ambiguous to be actionable.} Model cards are intended to surface, among other things, ethical and safety implications
% of models 
-- a topic that is especially pressing for deep learning models. 
However, our research supports prior findings that these concepts are 
% difficult to people to integrate in their work
challenging to integrate into decision-making~\cite{sambasivan:datawork:2021,morley:what_to_how:2019}, 
% worse we identified dismissal and cynicism toward ethical statements in particular. 
and we identified some 
% attitudes of dismissal and 
cynicism toward ethics statements, as well as 
% explicit 
assertions that ethical questions require contextual, situated examination.
% Rather than see this as a discouraging result, it points to the challenges of conveying these concepts through a medium of model documentation. 
Our findings indicate, unsurprisingly, that model documentation can spark ethical thinking, but will never substitute for it. 
% There do also exist other avenues for summarizing fairness and bias that we did not explore here, most notably as 
% Our studies did not address other strategies for summarizing bias, such as metrics~\cite{czarnowska2021quantifying,thomas2020problem}. 
% While we do encourage further examining these other avenues, we also urge  
We encourage further inquiry into other strategies toward fairness (e.g., metrics~\cite{czarnowska2021quantifying,thomas2020problem}), and we urge caution to ensure that these approaches are understandable and actionable for non-experts. 
Importantly, our analysis 
% shows a deeply personal dimension to contextualizing ethics and bias that is unlikely to be encapsulated entirely with any single approach. 
reinforces that considerations of ethics 
% and bias 
are personal and contextual, so they are unlikely to be addressed with a single approach.


%\subsection{Limitations}
\vspace{1mm}
% \noindent\textbf{Our research is not without its limitations}. 
\noindent\textbf{Limitations and Future Work}.
% Choices of interactions, sentiment analysis tasks, and the range of design elements that we explored 
Design choices and the choice of sentiment analysis tasks
(Section~\ref{sec:studyone_probes}) 
% do influence the conclusions that we drew. 
likely influenced our findings.
% While we anticipate that some of the specific design elements of our IMC prototype (i.e., the choice of visual cues, data visualizations etc.) may change in follow on studies, 
We anticipate that specific IMC design elements (i.e., the choice of visual cues, data visualizations, etc.) will be refined and adapted in future work.
However, we believe that the 
% more general set of design guides
broader design guidelines
(Section~\ref{study_one:design_guide}) and conceptual dimensions that we surfaced 
% in our analysis 
(Tables~\ref{tab:studyone_tab},~\ref{tab:studytwo_eval}, and \ref{tab:studytwo_prompts}) are robust and will generalize to other tasks and contexts. %For some, our choice of conducting a primarily qualitative study with a thematic analysis instead of a controlled trial (A/B test) or capturing quantitative participant feedback (i.e. Likert scale responses) will also appear a limitation. Quantitative assessments are useful when trying to answer \textit{how much} a design is preferred, but they are far less effective for interrogating \textit{what} participants cared about and most importantly \textit{why}. These latter considerations are more important for our study, whereas the former are pertinent to follow-on work that further optimizes the design. Moreover, the conceptual dimensions that we articulate in this work can be operationalized into survey instruments for conducting such quantitative analyses. 
We also recognize that creating and learning how to use IMCs is a heavier burden than for text-based model cards. We have taken steps in this work to build toward adaptable and extensible model card generators. Future work will explore further strategies for reducing and re-distributing the work of model documentation.

% 
 

%We also found that for nearly all participants, the ability of the model card to function as a sociotechnical artifact was also a critical lens through which they appraised the design. 
%Tentatively some possible topics:

%\begin{itemize}
%    \item It takes a village: model cards from a person-centric to a community-centric activity. Thinking about how the community can make artifacts available that in turn makes it easier to generate model cards. \hl{(REF: community-centered technical practice)}
%    \item Promoting productive skepticism : the model card doesn't answer all questions (so how can we help people at least think of all the questions)
%    \item As technologists, we also recognize that model building, deployment, evaluation, and use are becoming more and more distributed across organizations. How could we imagine that model cards will or should be taken up as epistemic or boundary objects?
%\end{itemize}


%\section{Limitations}
%Because you always need to include a limitations section
    

==> Interactive Model Cards/tex/ideation.tex <==
\section{Interactive Model Card Concept Formation and Ideation}

The goal of our work was to apply a human-centred design approach to interrogate the value of adding interactivity to model cards for model reporting. Model cards are a proposed structure for creating documentation on a machine learning or ML/AI model. As they were initially proposed, model cards are static, but this does not exclude the possibility of including interactivity. Model cards developed by  HuggingFace (\url{https://huggingface.co/} )and also Google Cloud Model Cards (\url{https://modelcards.withgoogle.com/}), for example, including interaction modalities for people to add their own data when evaluating model performance. Complementary to model cards, but not conforming strictly to their structure, are highly bespoke interactive `explorables', for example, those created by PAIR(\url{https://pair.withgoogle.com/explorables/}), distill (\url{https://distill.pub/}), or other narrative forms of visual and interactive model explanation. These two extremes between fully static and highly interactive, but bespoke, model documentation was the spectrum we considered for exploring the potential of interactive model cards. 

\textbf{The question of what to make interactive in a model card and how to do so is what we primarily investigate in our research.} We hypothesized that two primary areas of a model card that would benefit from interaction : the model training and evaluation data and the quantitative analysis portions.

\hl{<finish this this>}



%As model cards are primarily static in their proposed implementation we analyzed several existing model cards to propose areas where interactivity could be added

==> Interactive Model Cards/tex/introduction.tex <==
\section{Introduction}
Open source development has made it easier to share and deploy complex models, including large language models. This ease-of-use has lowered barriers to non-expert analysts~\cite{yang2018grounding} who 
% lack 
do not have
formal training in machine learning (ML), data science (DS), or linguistics.
% but routinely use these models. 
To accommodate a spectrum of ML expertise,  Mitchell et al.~\cite{mitchell10.1145/3287560.3287596} have proposed model cards as a means of providing consistent summaries of model details and their potential for misuse and harm. The format they propose is text-based and concise, making it both broadly accessible and applicable across model types.
However, these model cards
% , or other 
and
similar forms of 
% model 
documentation rely on the developer to accurately and clearly report on the model and its performance. Often, this process is labor-intensive and many important details, such as unintended uses or disaggregated model performance, are omitted. 
% Experts and non-experts alike 
Both experts and non-experts
who want to interrogate the model further must do so by implementing their own analysis. Not only does this mode of interrogation leave many non-experts underserved, it also exacerbates the potential for harm once these models are deployed~\cite{Crisan:fits_and_starts:2021,bender2021dangers,Benjamin2019AssessingRA,buolamwini:gender_shades:2018}. 

Prior work has shown that non-expert analysts benefit from interacting with machine learning models and their data~\cite{Amershi:Power:2014,dudley:IML:2018,scaha:HCD:2017}. Recently, others have experimented with adding interactive elements to model cards. Both HuggingFace~\cite{wolf:huggingfaces:2020} and Google Cloud platforms introduced interactive modalities for interrogating the model’s performance through customizable examples of the model’s inputs. Robustness Gym reports~\cite{goel2021robustness} 
% sought 
seek
to overcome the development burden of model cards by allowing end-users to interactively create new slices of the data to interrogate a model's performance. Complementary to model cards are ‘explainables’, which are generally bespoke and interactive~\cite{hohman:explainable:2020}. While these early explorations are promising, they do not explore how much or what kind of interactivity is beneficial. %Moreover, they do not examine the value of this interaction with non-experts.

In this work, we use the concept of a model card to scaffold a design inquiry into alternative and expanded forms of model documentation, focusing in particular on the needs of non-experts.  We propose a novel concept for an \textit{interactive model card} (IMC) that: (1) lowers barriers to accessing key information about model behavior; (2) supports deeper interrogation of models; and (3) surfaces some attendant risks and limitations without additional work on the part of model developers. We 
% created 
built
this idea out through an initial conceptual study with experts in ML, Ethics, and NLP to co-create a set of design guidelines for a functional IMC prototype. 
% In this study, \textit{we draw on experts' experiential knowledge on the wider implications on ML and NLP models and how they are used within organizations to inform our design processes. We conduct a subsequent study with non-expert analysts to assess our design choices}. Across both studies, we apply a human centered lens to examine the affordances, opportunities, and limitations for standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, RobustnessGym Reports (RGRs)~\cite{goel2021robustness}, and IMCs.
In this first study, we drew on experts' experiential knowledge of the wider implications of ML and NLP models, along with applications of these models within organizations, to 
\textit{better understand implications of design choices in model documentation and inform our development of an IMC.} 
We conducted a subsequent study with non-expert analysts to 
\textit{deepen our understanding of documentation needs and evaluate our IMC design.} 
Across both studies, we apply a human-centered lens to examine the affordances, opportunities, and limitations for standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, Robustness Gym reports (RGRs)~\cite{goel2021robustness}, and IMCs.

\textit{\textbf{Through this research, we provide the following three contributions:}}
% 1) Design guidelines for developing interactive model cards;
1) Design guidelines for interactive model cards and model documentation broadly;
2) A set of conceptual dimensions for evaluating model documentation with respect to AI/ML workers of 
% varying expertise; 
various backgrounds; and
3) A functional prototype for an interactive model card that can be adapted for further inquiries and usage scenarios. We make artifacts of our research process available online\footnote{\url{https://osf.io/9d83t}}.% and are linked to from the manuscript text via the \texttt{[OM\#]} notation.

%As deep learning models for natural language processing have become easier to use and more widely available, they are increasingly adopted and deployed by people without formal training in machine learning, linguistics, or statistics. Despite these shifts, the  types of documentation that encompass model purpose, training details, intended use contexts, and other relevant considerations remain largely tailored toward individuals who do have such formal training. For example, model cards~\cite{mitchell10.1145/3287560.3287596} and similar artifacts can provide consistent summaries of model details, but the burden is on model developers to create bespoke artifacts, and some categories of information --such as disaggregated model performance--are prohibitively labor-intensive to produce. %Moreover, the forms that these model cards have taken generally target experts in a particular domain of machine learning (ML) (i.e., through jargon and design decisions around details to include), leaving other ML/AI practitioners and non-expert users underserved. 
%Moreover to interrogating the model further it is necessary for an individual implement their own analysis~\cite{yang2018grounding}. This mode of interrogation leaves many that may use or impacted by these models unsupported and exacerbate the potential for harm once these models are deployed~\cite{Crisan:fits_and_starts:2021,bender2021dangers,Benjamin2019AssessingRA,buolamwini:gender_shades:2018}. 



%Recently, model cards have begun to incorporate interactive elements as a way to enable a wider group of practitioners and stakeholders explore and make sense of more complex deep learning models. For example, model cards developed by \href{https://huggingface.co/}{HuggingFace} and   \href{https://modelcards.withgoogle.com/}{Google Cloud Model Cards} include interaction modalities for people 
% to add their own data when evaluating model performance.
%to test model behavior on their own data (by manually entering example data).
%Complementary to model cards, but not conforming strictly to their structure, are highly bespoke interactive `explorables', such as those created by \href{https://pair.withgoogle.com/explorables/}{PAIR}, \href{https://distill.pub/}{distill}, or other narrative forms of visual and interactive model explanation. 
% These two extremes between fully static and highly interactive, but bespoke, model documentation was the spectrum we considered for exploring the potential of interactive model cards. 
%Consideration of the spectrum of interactivity within these bespoke artifacts--from fully static to highly interactive--informed our exploration of the potential for interactive model cards to support model understandability.
%Importantly, we were motivated by the lack of studies assessing whether the design choices made across this spectrum of model documentation is accessible to the equally broad spectrum of data workers that engage with ML/AI models.

%In this work, we use the concept of a model card to scaffold design inquiry into alternative and expanded forms of model documentation, focusing in particular on the needs for non-expert users. Our approach seeks to support a virtuous cycle of contemplation, creation, and consolidation~\cite{goel2021robustness} through interactive and extensible model documentation. To that end, we propose a novel concept for an \textit{interactive model card} that: (1) lowers barriers to accessing key information about model behavior; (2) supports deeper interrogation of models; and (3) surfaces some attendant risks and limitations without additional work on the part of model developers. Applying a human-centered design lens, we examine the affordances, opportunities, and limitations for standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, robustness gym reports (RGRs)~\cite{goel2021robustness}, and interactive model cards (IMCs). 

%We carried out two connected studies, the first with ten experts in ML/AI, Ethics, and NLP, and the second with twenty data analysts who use ML/AI models in their daily work but lack formal (i.e., post secondary) education in either machine learning, data science, or statistics. 
% We asked participants in the first study to engage with a concept and also a functional prototype of an interactive model card and contrast it with a reference model card. 
%We asked participants in both studies to engage with examples of a reference model card and an IMC that incorporated the same information (as a conceptual probe in the first study and a functional prototype in the second).
%Through these studies our research contributes:
%\begin{itemize}
%    \item A set of conceptual dimensions for evaluating model documentation with respect to AI/ML workers of varying expertise
%    \item Design guidelines for developing interactive model cards.
%    \item A functional prototype for an interactive model card that can be adapted for further inquiries and usage scenarios.
%\end{itemize}
% Through these studies our research contributes:
% \begin{itemize}
%     \item Conceptual dimensions for probing the relationship between model documentation and data work that uses ML/AI models and that is performed by workers that occupy across a spectrum of expertise. 
%     \item Design guidelines for developing interactive model cards 
%     \item A functional prototype for an interactive model card that can be adapted for further inquiries and usage scenarios
% \end{itemize}

%As it becomes easier for a wider group of data workers to develop and deploy ML/AI models, via low- and no-code solutions, our work and its findings presents a timely examination of the accessibility of model cards and model documentation more generally. Moreover, our approach emphasizes the importance of  adopting a human-centered design lens to ensure equitable opportunities for understanding and evaluating ML/AI models.

%\vspace{1mm}
%\noindent{\textbf{Supplemental Materials}} : Are available online\footnote{\url{https://osf.io/9d83t/?view_only=7359695185b04468a7ae4a2e189691c0} is an anonymous view only link for review } and are linked to from the manuscript text via the \texttt{[OM\#]} notation.



%\hl{MOVED THIS FROM EARLIER, SHOULD GO IN INTRO THOUGH} : Prior studies~\cite{Wexler:whatif:2019} have shown the value of interactive probing for helping people understand models and contextualize their performance

% \hl{PLACEHOLDER: motivation: disaggregated quant analysis prohibitively difficult and often not included; SMCs don't adequately support deeper interrogation or oversights from viewers}
%To better understand needs and challenges for model documentation, we began by conducting a formative study with ten individuals who have expertise in AI ethics, auditability, AI/ML development, and/or NLP. Following a brief semi-structured interview about participants’ backgrounds, we asked them to engage in a think-aloud protocol with SMC, RGR, and IMC design probes for a sentiment analysis model. As they reflected on the value and limitations of each design, we asked participants to consider both their own needs as experts as well as the needs of users who do not have formal ML or NLP training. Through this formative investigation, we surfaced documentation needs across a range of stakeholders related to information design, guidance, trust, and sensemaking.

%After synthesizing insights shared by these experts, we used our findings to shape the design for a functional prototype of an interactive model card. We evaluated that prototype in a second study conducted with 20 participants who use AI/ML models in their work but did not have any formal training.  
% In this study, we first asked participants to engage organically with an existing model card and with our interactive model card in a think-aloud protocol.
%Participants were prompted with the scenario of trying to understand the behavior and limitations of a previously unfamiliar language model using first an existing model card and then the IMC prototype. For each model card, participants were asked first to explore the card in whatever manner they would choose to build out that understanding. We concluded the session with a semi-structured interview to capture participants’ perspectives on how these model cards helped them understand the model’s usability, functionality, operationalizability, safety, and potential ethical risks. Our findings validated some design patterns in existing model cards but also highlighted the limitations for non-expert AI/ML users. In the following sections, we share specific design recommendations for model cards surfaced through these studies. 
%\hl{PLACEHOLDER - overview of findings}.
%We also articulate broader implications for human-centered design approaches to documenting and assessing AI/ML systems

%\hl{Not yet integradted into text, but gives a sense of interactivity in model cards}
%The goal of our work was to apply a human-centred design approach to interrogate the value of adding interactivity to model cards for model reporting. Model cards are a proposed structure for creating documentation on a machine learning or ML/AI model. As they were initially proposed, model cards are static, but this does not exclude the possibility of including interactivity. Model cards developed by  HuggingFace (\url{https://huggingface.co/} )and also Google Cloud Model Cards (\url{https://modelcards.withgoogle.com/}), for example, including interaction modalities for people to add their own data when evaluating model performance. Complementary to model cards, but not conforming strictly to their structure, are highly bespoke interactive `explorables', for example, those created by PAIR(\url{https://pair.withgoogle.com/explorables/}), distill (\url{https://distill.pub/}), or other narrative forms of visual and interactive model explanation. These two extremes between fully static and highly interactive, but bespoke, model documentation was the spectrum we considered for exploring the potential of interactive model cards. 

%\hl{ALSO NOT YET INTEGRATED}
%The goal of our study was elicit and synthesize our informants' experiences, perspectives, and reactions to different modalities of documenting and reporting on machine learning models. Some aspects of standard models cards, for example, may be favorable to alternatives presented in the interactive model card, and vice versa.  However, we did not have a definitive signal (nor did we set out to find one) that one modality (SMC, RGR, or IMC) is better than the other. 

==> Interactive Model Cards/tex/related_work.tex <==
\section{Background and Related Work}

%%% NOTE: commented out sections in the text of this section include points that I think it would be valuable to include but have been cut for space requirements. Recommend leaving in the draft in case we decide to make space in other ways (and in an effort to be prepared for reviewer feedback). Likewise (and. for similar reasons), recommend retaining commented out notes at the bottom of this section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Potential Harms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{Potential for Harm in AI/ML Systems.}
The \textbf{\textit{potential for both broad and deep harm}} that AI/ML systems can pose to vulnerable people and ecosystems, 
%has been extensively documented
especially when impacted people do not have the opportunity to interrogate and contest decisions driven by AI/ML(e.g.,~\cite{barocas2016big,whittaker2018ai,hoffmann2019fairness,hamidi2018gender,hanna2020towards}). 
% Moreover, 
%These risks are exacerbated when such systems are deployed with minimal oversight and/or when impacted people do not have the opportunity to interrogate and contest decisions driven by AI/ML.
Large language models are especially predisposed to amplify harms,
% given the opacity of their training data and the scale of their influence through fine-tuned versions.
since they are being deployed widely enough to result in homogenization while their inner workings and limitations are poorly understood~\cite{bommasani2021opportunities,bender2021dangers}. 
% Bommasani et al. elaborate on the risks presented by foundation models, noting that although these large models are being deployed widely enough to result in homogenization (for example, in NLP), the inner workings and limitations of these models are poorly understood and inaccessible to end users~\cite{bommasani2021opportunities}.
% As Bender~\textit{et al.} have articulated, 
% % not only does environmental impact scale with model size, but 
% ``large datasets based on texts from the Internet overrepresent hegemonic viewpoints and encode biases potentially damaging to marginalized populations'' 
% % (e.g., white supremacy and misogyny)
% ~\cite{bender2021dangers}. 
% Large models also result in ``documentation debt'' with training datasets that are too large to adequately document, limiting opportunities to challenge or contest outputs from these models~\cite{bender2021dangers}.
Notably, even systems that seek to identify and mitigate racism, harassment and hate speech
% are vulnerable to reifying or c
% can 
may compound harms to vulnerable people (e.g.,~\cite{benthall2019racial,corbett2018measure,mozafari2020hate}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Explainability, Transparency, and Contestability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{Explainability, Transparency, and Contestability.}
In an effort to mitigate the risks for harm in AI/ML systems, researchers and developers have proposed strategies to make systems more \textbf{\textit{explainable, transparent,} and \textit{contestable}} (e.g.,~\cite{guidotti2018survey,yang2021intellige,madsen2021post,arrieta2020explainable,kaur2020interpreting,mittelstadt10.1145/3287560.3287574,molnar2020interpretable}). %Several have highlighted that the ``right to explanation'' extends from the European Union’s General Data Protection Regulation (GDPR)~\cite{selbst2018meaningful,langer2021we,shneiderman2020bridging}; our approach of prioritizing the needs of non-experts ascribes to this principle. 
Our study design (Sections~\ref{study_one:general_procedures} and~\ref{sec:study2_procedures}) has been informed by prior work related to measuring and improving model interpretability~\cite{poursabzi2021manipulating,mittelstadt10.1145/3287560.3287574}, and proposals for contrastive explanations~\cite{mittelstadt10.1145/3287560.3287574} are particularly aligned with our approach to interactivity and seeding the IMC with examples (as described in Section~\ref{study_two:functional-prototype}). Our approach to interactivity has also been informed by Amershi~\textit{et al.}'s guidelines for human-AI interaction~\cite{amershiGuidelines10.1145/3290605.3300233},
% (particularly with respect to clarity about the system's behavior, limitations, and opportunities for error correction)~\cite{amershiGuidelines10.1145/3290605.3300233}, 
as well as by other guidelines and taxonomies for human-centered AI~\cite{arrieta2020explainable,shneiderman2020bridging} and proposals for enabling human contestation of AI-driven decisions~\cite{lyons10.1145/3449180,hirsch2017designing}. 
% As Yang et al. have articulated, a unique challenge for designing human-AI systems is representing uncertainty about system capabilities and potential for harm~\cite{yang2020re-examining}. Findings from our first study with experts (Section~\ref{sec:study_one}) reinforce these findings, and we have proposed strategies to make clear system limitations and address harmful social implications in Section~\ref{sec:discussion}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Trust and Skepticism
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Related to explainability and contestability, some 
Prior work has also addressed dimensions of model behavior and documentation that impact \textbf{\textit{trust}} and \textbf{\textit{skepticism}}. 
Many studies have found that cognitive biases (particularly anchoring bias and automation bias more broadly) can lead users to misunderstand model behavior and place unwarranted trust in AI systems~\cite{kaur2020interpreting,Nourani:anchoring:2021,poursabzi2021manipulating,ehsan2021explainability}.
% ; notably, these biases have been observed even with technically sophisticated users.
We introduce the concept of \textit{productive skepticism} (Section~\ref{sec:discussion}), and we argue that stimulating productive skepticism--along with providing modalities for interaction and sensemaking--could be an effective strategy to mitigate the tendency to over-trust. Rather, opportunities to engage with productive skepticism can support stakeholders in calibrating appropriate trust in a model's behavior for a particular context and use case.
Our approach %to stimulating productive skepticism 
aligns with calls for new strategies of calibrating user trust in AI~\cite{zhang10.1145/3351095.3372852} and promoting reflection~\cite{ehsan2021explainability}, and our approach to guidance and warnings (discussed in Section~\ref{study_one:design_guide}) encompasses the requirements for extrinsic trust articulated by Jacovi~\textit{et al.}~\cite{jacovi2021formalizing}.
% In alignment with principles for responsible AI~\cite{amershiGuidelines10.1145/3290605.3300233,arrieta2020explainable}, we also assert that dimensions trust and skepticism should be evaluated with respect to particular stakeholders' needs and contexts of use (discussed further in Sections~\ref{study_one:res_stakeholders} and~\ref{sec:discussion}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Model Cards and Documentation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Various forms of \textbf{\textit{model documentation}} have been proposed to make AI/ML systems more transparent and help users establish trust.
\textit{Model cards} (SMCs)~\cite{mitchell10.1145/3287560.3287596}  
%were initially proposed as a framework for communicating benchmarked evaluation data and intended use contexts~\cite{mitchell10.1145/3287560.3287596}, and 
have been foundational in standardizing documentation for AI/ML model performance and characteristics, along with 
% its harms 
risks
and unintended uses. 
Robustness Gym helps model developers report on model behavior 
% across different subpopulations 
through the generation of \textit{robustness reports} (RGRs) that summarize model performance on various data slices~\cite{goel2021robustness}. We incorporate SMCs and RGRs as core elements of the IMC design.
%Neither SMCs nor RGRs include detailed information related to the training and evaluation data,
We also look to work on \textit{datasheets for datasets} to include more detailed information of the model's data~\cite{gebru2021datasheets}. The IMC design follows the SMC model for reporting on datasets, and our functional prototype (Section~\ref{study_two:functional-prototype}) also includes warnings related to age of the training dataset.
In evaluating the IMC,
% with respect to explainability, 
we also draw on dimensions articulated 
% by Sokol and Flach for their 
for 
\textit{explainability fact sheets}~\cite{sokol10.1145/3351095.3372870}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Governance and Accountability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Beyond the practical necessity of standardized documentation for AI/ML models to be useful and usable, 
Model cards and similar standardized artifacts can play a role in processes for \textbf{\textit{governance}} and \textbf{\textit{accountability}} of AI/ML systems. As many have studies have reinforced, mechanisms for governance and accountability of technical systems are prerequisites for informed consent~\cite{giannopoulou2020algorithmic,carroll2020care,viljoen2021relational} and equity~\cite{dombrowski2016social,lee2019webuildai,krafft2021Action}.
% ; requirements for governance have also been enshrined into standards and law in multiple countries~\cite{hleg2020assessment,lyons10.1145/3449180}. 
% Shneiderman proposes governance strategies at three levels of hierarchy: team, organization, and industry (including independent oversight)~\cite{shneiderman2020bridging}, and our findings indicate that IMCs can be useful artifact at each of these levels. 
Algorithmic audits are a key strategic approach toward governance and accountability.
Whether conducted through internal processes or by third-party actors, audits seek to evaluate AI models for issues of robustness, bias, and fairness.
Public audits have been shown to be effective at reducing bias in targeted companies (as compared to other companies) ~\cite{raji2019actionable}.
Auditing should be a structured, ongoing process that is designed from a system perspective~\cite{shneiderman2020bridging,kingsley2020auditing}. However, many challenges remain from conceptual, technical, economic, and organizational perspectives ~\cite{mokander2021ethics}.
% Many of these systems evaluate ML systems under normal operating conditions, which may not be sufficient in the case of an adversarial attack against a particular subgroup~\cite{nanda10.1145/3442188.3445910}.
In contrast to posthoc audits and evaluations, \textit{certificates} of robustness provide algorithmic guarantees on the performance of models under certain conditions ~\cite{zhang2021certified}. 
% Kroll highlights \textit{traceability} approaches an underpinning for auditability of AI/ML systems~\cite{kroll10.1145/3442188.3445937}.
%Raji et al.~\cite{raji2020closing} have proposed an end-to-end framework for internal algorithmic auditing 
% that encompasses scoping, mapping, artifact collection, testing, reflection, and post-audit 
%(SMACTR). 
% Experts in our first study raised the potential for IMCs to support algorithmic audits, and although Raji et al.~\cite{raji2020closing} situate model cards in the artifact collection stage, our findings suggest that IMCs could also contribute to the reflection and post-audit stages. 
%Raji~\textit{et al.}~\cite{raji2020closing} have proposed an end-to-end framework for internal algorithmic auditing that situates model cards in an early artifact collection stage. 
%Our findings suggest that IMCs could also contribute to later reflection and post-audit stages.
Human-in-the-loop auditing processes leverage everyday users to provide further protection once a system is deployed~\cite{shen10.1145/3479577}, and we heard from participants in both of our studies that they believed IMCs would be valuable for record-keeping and organizational alignment throughout deployment.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Needs for Industry Practitioners
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%As AI/ML systems have become ever more widely deployed and the need for governance to mitigate harm has become more recognized, the research community has turned to exploring \textbf{\textit{practitioners' needs}} for trust and transparency in order to deploy models safely. 
Recent research has surfaced implications for \textbf{\textit{practitioners' needs}} for trust and transparency.
Some have identified strategies practitioners use to build understanding 
% Researchers have identified various strategies that practitioners employ for building understanding 
% and trust 
of AI/ML models, including data- and model-centric patterns of exploration~\cite{mishra2021designing,sanchez10.1145/3449236} and investigation of data where a model performs particularly well and poorly~\cite{mishra2021designing,lucic10.1145/3351095.3372824,sanchez10.1145/3449236}.
Our considerations around trust and productive skepticism have been informed by prior work identifying domain expertise and predispositions for trust as risk factors in bringing models into practice~\cite{nourani2020role,Dietvorst:AlgorithmAP:2015,knijnenburg2011each,yang2018grounding,mishra2021designing}.
Furthermore, our support for exploration of sup-populations and sampling examples with low- and high-confidence scores address these needs in part.
Hong~\textit{et al.}~\cite{hong2020human} have also surfaced needs for integrated interpretability support with AI/ML tooling, which aligns with our findings.
In response to practitioners' needs to evaluate AI/ML models with respect to safety~\cite{wang2021ai} and ethical decision-making~\cite{holstein2019improving}, we have evaluated the IMC along these dimensions.
As many researchers have articulated, safe and effective deployment of AI/ML systems in practice requires a robust understanding of different stakeholders' needs and goals for explainability~\cite{bhatt10.1145/3351095.3375624,hong2020human}; support for traceability and auditing~\cite{wang2021ai}; and strategies to address concerns within existing organizational structures and dynamics~\cite{wang2021ai,holstein2019improving,bhatt10.1145/3351095.3375624,rakova10.1145/3449081,hong2020human}.
We found that our approach to guidance, shareability, and traceability begins to address these needs, and we surfaced additional relevant implications for design.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   NOTES - retain these for now
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   TODO - not currently in draft, maybe should be
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - Measuring and Mitigating Unintended Bias in Text Classification~\cite{dixon2018measuring}
% - A Survey of Human-Centered Evaluations in Human-Centered Machine Learning (possibly relevant for dimensions of auditing/reviewing IMC)~\cite{sperrle2021survey};
% - A Relational Theory of Data Governance~\cite{viljoen2021relational}
% - Add - ``the problem with metrics''~\cite{thomas2020problem}
% - Relevant but didn't make it in anywhere... Trust, but Verify: Informed Consent, AI Technologies, and Public Health Emergencies~\cite{pickering2021trust};
% - somewhat relevant but a little hard to parse and it isn't directly relevant Sentiment Analysis: What is the End User’s Requirement?~\cite{das2012sentiment};
% ~\cite{das2012sentiment}; 

% - TODO DISCUSSION - the problem with metrics is a fundamental problem for AI~\cite{thomas2020problem}
% all metrics can be gamed~\cite{thomas2020problem}

% - TODO DISCUSSION - Algorithmic Bias in Autonomous Systems: defining different dimensions algorithmic bias -- relevant for how experts and Bus Scis reflect on bias and their need to evaluate~\cite{danks2017algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Potential Harms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Harm to ecosystems and marginalized people:
% - (On the dangers of...) Stochastic parrots~\cite{bender2021dangers}
%  environmental impact scales with model size, ``large datasets based on texts from the Internet overrepresent hegemonic viewpoints and encode biases potentially damaging to marginalized populations'' (e.g., white supremacy and misogyny), cited studies on Co2 emissions, noting risks and benefits don't accrue to the same people-- i.e., disparate climate impact on marginalized people in the global south while ``most language technol- ogy is built to serve the needs of those who already have the most privilege in society''; ``Even if populations who feel unwelcome in mainstream sites set up different fora for communication, these may be less likely to be included in training data for language models.''; filtering often suppressed discourses from marginalized people (e.g., sex workers, LGBTQ individuals); ``we note that moving beyond demonstrating the existence of bias to building systems that verify the ‘safety’ of some LM (even for a given protected class) requires engaging with the systems of power that lead to the harmful outcomes such a system would seek to prevent''; ``documentation debt:'' ``datasets are both undocumented and too large to document post hoc. While documentation allows for potential accountability [13, 52, 86], undocumented training data perpetuates harm without recourse.'' ~\cite{bender2021dangers} 

% - Opportunities and risks for foundation models~\cite{bommasani2021opportunities};
% ``Despite the impending widespread deployment of foundation models, we currently lack a clear understanding of how they work, when they fail, and what they are even capable of due to their emergent properties.'';`While one can view this last wave of technical developments purely through the lens of self- supervised learning, there was a sociological inflection point around the introduction of BERT. Before 2019, self-supervised learning with language models was essentially a subarea in NLP, which progressed in parallel to other developments in NLP. After 2019, self-supervised learning with language models became more of a substrate of NLP, as using BERT has become the norm. The acceptance that a single model could be useful for such a wide range of tasks marks the beginning of the era of foundation models...Foundation models have led to an unprecedented level of homogenization: Almost all state-of- the-art NLP models are now adapted from one of a few foundation models, such as BERT, RoBERTa, BART, T5, etc. While this homogenization produces extremely high leverage (any improvements in the foundation models can lead to immediate benefits across all of NLP), it is also a liability; all AI systems might inherit the same problematic biases of a few foundation models '';``In this section, we consider misuse of foundation models — situations where people use foundation models as they are intended to be used (e.g., to generate language), but where their capabilities are intentionally leveraged to cause harm to populations or individuals. This definition positions misuse concerns between those of inequity (where models can cause harm without bad intentions; §5.1: fairness) and security (where bad actors exploit unintentional abilities or vulnerabilities in models to cause harm; §4.7: security). Below, we outline how foundation models both enable new forms of misuse and support new tools for misuse detection and mitigation.''`` Improvements in automatic detection systems for both model-generated and human-generated harmful content will make these systems more prevalent online, yielding potential negative consequences. Any detection system will have false positive cases where human-generated fair content will be flagged as harmful [Sap et al. 2019; Xu et al. 2021]. The rate at which algorithmic false positives affect users (or groups of users) may cause downstream harm (§5.1: fairness).''~\cite{bommasani2021opportunities}


% - Racial categories in machine learning~\cite{benthall2019racial}
% relates to our approach to considering protected categories: ``This creates a dilemma for so- ciety and designers: be blind to racial group disparities and thereby reify racialized social inequality by no longer measuring systemic inequality, or be conscious of racial categories in a way that itself reifies race. We propose a third option. By preceding group fairness interventions with unsupervised learning to dynamically detect patterns of segregation, machine learning systems can mitigate the root cause of social disparities, social segregation and stratification, without further anchoring status categories of disadvantage.''; ``Comparatively little attention is given to how the protected class labels, A, are assigned, why they are being protected and by whom, and what that means for the normative presumptions typical of `fair' machine learning design.'';``Race is a social and cultural hierarchical system of categories that stigmatizes differences in human bodies, but is not those body differences themselves [41]. Race differences are created by ascribing race classifications onto formerly racially unspecified individuals and linking them to stereotyped and stigmatized beliefs about non- white groups'';``We draw a distinction between the software used by a machine system and its input and output data. Further, we distinguish be- tween three categories of systems that are not mutually exclusive: those that are themselves racial projects, those that allow their users to engage in racial projects, and those that attempt to be “blind” to race. Racial projects may be racist, anti-racist, or neither.Machines that attempt to correct unfairness through explicit use of racial classification do so at the risk of reifying racial categories that are inherently unfair. Machine learning systems that allocate resources in ways that are blind to race will reproduce racial inequality in society. We propose a new design in Section 5 that avoids both these pitfalls.''~\cite{benthall2019racial}

% Fairness - an overview
% - The Measure and Mismeasure of Fairness: A Critical Review of Fair Machine Learning~\cite{corbett2018measure}
% ``From criminal justice to medicine, practitioners are increasingly turning to statistical risk assessments to help guide and improve human decisions. Algorithms can avoid many of the implicit and explicit biases of human decisions makers, but they can also exacerbate historical inequities if not developed with care. Policymakers, in response, have rightly demanded that these high-stakes decision systems be designed and audited to ensure outcomes are equitable. The research community has responded to the challenge, coalescing around three mathematical definitions of fairness: anti-classification, classification parity, and calibration. Over the last several years, dozens of papers have applied one or more of these measures either to audit existing systems or as constraints when developing new algorithms. However, as we have aimed to articulate, these popular measures of fairness suffer from significant statistical limitations. Indeed, enforcing anti-classification or classification parity can often harm the very groups that these measures were designed to protect.''~\cite{corbett2018measure}  ---- relate this to model auditing issues listed in stochastic parrots paper

% - Detecting hate speech, identifying categories of text with higher risk- Hate speech detection and racial bias mitigation in social media based on BERT model~\cite{mozafari2020hate};
% ``This study reveals that the benchmark datasets for hate speech and abusive language identifi- cation tasks are containing oddities that cause a high preference for classifiers to classify some samples to the specific classes.''; ``As we are dealing with textual content from social media in our task and the BERT model is pre-trained on general corpora, it is crucial to analyze the contex- tual information extracted from pre-trained BERT’s transformer layers.''; proposes Opportunities to mitigate bias in hate speech by extending hate speech detection algs with transfer learning~\cite{mozafari2020hate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Explainability, Transparency, and Contestability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% SURVEYS AND OVERVIEWS of explainability and interpretability approaches:
% - Survey of methods for explainability~\cite{guidotti2018survey};
% - Intellige: A User-Facing Model Explainer for Narrative Explanations~\cite{yang2021intellige}
% - Post-hoc Interpretability for Neural NLP: A Survey~\cite{madsen2021post}
% - Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI - relevant taxonomy for our evaluative dimensions~\cite{arrieta2020explainable}
% - Explaining Explanations in AI: human explanations are contrastive; XAI descriptions are simplified mathematical models, not human interpretable, selective, social -- relevant for our arguments around documentation as socially constructed and contested/challenged; also relates to human meaning described in stochastic parrots paper; TODO: come back to this for the discussion of model cards as sociotechnical artifacts/boundary negotiating artifacts; also tied to contestability~\cite{mittelstadt10.1145/3287560.3287574}
% - Meaningful Information and the Right to Explanation - sadly this is just an extended abstract; I think it was presentation only~\cite{selbst2018meaningful}
% - Interpretable Machine Learning – A Brief History, State-of-the-Art and Challenges~\cite{molnar2020interpretable}

%%% RIGHT TO EXPLANATION
% - What Do We Want From Explainable Artificial Intelligence (XAI)?~\cite{langer2021we};
% explanation needs aligned with particular stakeholders - TODO DISCUSSION link to our stakeholder finding; various, interrelated aims of understanding including verification, improving performance, ``right to explanation'' GDPR, and accountability to stakeholders~\cite{langer2021we}

% ``Designers of HCAI systems have come to realize that consequential decisions that influence people’s lives, such as rejections for mortgages, parole, or job interviews, often raise questions from those who are affected. Therefore, these systems must come with explanations that enable people to understand the decisions, so they know what they need to change or whether they should challenge the decision.  Furthermore, explanations have become a legal requirement in many countries based on the European Union’s General Data Protection Regulation (GDPR) requirement of a `right to explanation'''~\cite{shneiderman2020bridging}

%%% MEASURING AND IMPROVING INTERPRETABILITY
% Measuring and explaining interpretability and explanations (meta-explanations)~\cite{poursabzi2021manipulating,mittelstadt10.1145/3287560.3287574}

%%% GUIDELINES AND TAXONOMIES
% - Guidelines for Human-AI Interaction~\cite{amershiGuidelines10.1145/3290605.3300233}
% ``We propose 18 generally applicable design guide- lines for human-AI interaction. These guidelines are vali- dated through multiple rounds of evaluation including a user study with 49 design practitioners who tested the guidelines against 20 popular AI-infused products.''- Many of the guidelines relate to user understanding of the what the system can and can't do, why it did what it did, and on predictability and correction of errors, also show contextually relevant information, mitigate social biases, TODO more here~\cite{amershiGuidelines10.1145/3290605.3300233}

% - Taxonomies and guidelines for responsible AI - Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI -~\cite{arrieta2020explainable} 
% TODO DISCUSSION relevant taxonomy for our evaluative dimensions~\cite{arrieta2020explainable} 

% - TODO DISCUSSION OR REL WORK - this should probably Re-examining Whether, Why, and How Human-AI Interaction is Uniquely Difficult to Design~\cite{yang2020re-examining}
% AI systems can make unpredictable errors that damage UX or cause social harm; two key challenges in HCAI design are uncertainty about AI capabilities and out complexity of models~\cite{yang2020re-examining}

%%% CONTESTABILITY
% Designing Contestability: Interaction Design, Machine Learning, and Mental Health~\cite{hirsch2017designing}
% ``illustrate challenges with creating interactive machine learning (ML) systems, particularly in contexts where human life, livelihood, and wellbeing are at stake. We explore how existing theories of interaction design and machine learning apply to the psychotherapy context, and identify “contestability” as a new principle for designing systems that evaluate human behavior''; ``The problem of contestation, of challenging machine predictions, becomes particularly acute when we recognize that our models are, and will continue to be, fallible, and the risks of “getting it wrong” can be quite high for therapists and patients alike.''``This concern is somewhat speculative, as systems like ours are fairly novel. Nonetheless, we identify several design strategies that can be put in place now, to help mitigate future misuse.''~\cite{hirsch2017designing}

% - Conceptualising Contestability: Perspectives on Contesting Algorithmic Decisions~\cite{lyons10.1145/3449180}
% ``describing and analysing the perspectives of people and organisations who made submissions in response to Australia’s proposed ‘AI Ethics Framework’, the first framework of its kind to include ‘contestability’ as a core ethical principle. Our fndings reveal that while the nature of contestability is disputed, it is seen as a way to protect individuals, and it resembles contestability in relation to human decision-making.'';``Little is known about what contestability in relation to algorithmic decisions entails, and whether the same processes used to contest human decisions, which range from informal complaints mechanisms to formal legal processes, are suitable for algorithmic decision-making'';TODO - relate to accountability and governance~\cite{lyons10.1145/3449180}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Trust and Skepticism
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MISPLACED TRUST
% data scientists over-trust and misuse interpretability tool--points to need for stimulating productive skepticism~\cite{kaur2020interpreting}

% anchoring bias and automation bias broadly~\cite{Nourani:anchoring:2021}

% - Manipulating and Measuring Model Interpretability~\cite{poursabzi2021manipulating}
% ``Predictably, participants who saw a clear model with few features could better simulate the model’s predictions. However, we did not find that participants more closely followed its predictions. Furthermore, showing participants a clear model meant that they were less able to detect and correct for the model’s sizable mistakes, seemingly due to information overload.'' -- information overload leads to over-trusting TODO link to productive skepticism; ``importance of testing over intuition when developing interpretable models.'' -- TODO relate this significance o design decisions in model cards; ````We found that people can better simulate the predictions of a clear model with few features compared to the predictions of a clear model with more features or the predictions of a black-box model. However, contrary to our expectations, we did not find a significant improvement in the extent to which people follow the predictions of a clear model with few features when it is beneficial for them to do so compared to the predictions of a black-box model with more features. We also found that using a clear model hampers people’s abilities to detect when the model had made a mistake. All three of these findings are based on highly-powered, pre-registered experiments with multiple, representative stimuli. Our latter two findings are notable and surprising because they contradict common intuition about interpretability.TODO DISCUSSION- much more here that is relevant -- clear models don't necessarily make people more likely to follow recs - aligned with our productive skepticism findings''~\cite{poursabzi2021manipulating}

% - Explainability pitfalls and understanding potential harm~\cite{ehsan2021explainability}
% unwarranted trust as a key pitfall - TODO relate to Kaur et al. and productive skepticism; ``At the research level, we need to conduct more situated and empirically diverse human-centered research to obtain a refined understanding of the stakeholders as well as the dimensions of explanations that affect different stakeholders in XAI. '' - motivation for our work; ``One possible strategy can be to shift our explanation design philosophy to emphasize user reflection (as opposed to acceptance) during interpretation of explanations. Recent human-centered XAI work has also advocated for conceptualizing ways to foster trust via reflection ''~\cite{ehsan2021explainability}

%%% CALIBRATING TRUST AND REFLECTION
% - (Skepticism and Critical Evaluation) Effect of Confidence and Explanation on Accuracy and Trust Calibration in AI-Assisted Decision Making~\cite{zhang10.1145/3351095.3372852}
% ``we show that confidence score can help calibrate people’s trust in an AI model, but trust calibration alone is not sufficient to improve AI-assisted decision making, which may also depend on whether the human can bring in enough unique knowledge to complement the AI’s errors. We also highlight the problems in using local explanation for AI-assisted decision making scenarios and invite the research community to explore new approaches to explainability for calibrating human trust in AI.''~\cite{zhang10.1145/3351095.3372852}

% - Explainability pitfalls and understanding potential harm~\cite{ehsan2021explainability}
% unwarranted trust as a key pitfall - TODO relate to Kaur et al. and productive skepticism; ``At the research level, we need to conduct more situated and empirically diverse human-centered research to obtain a refined understanding of the stakeholders as well as the dimensions of explanations that affect different stakeholders in XAI. '' - motivation for our work; ``One possible strategy can be to shift our explanation design philosophy to emphasize user reflection (as opposed to acceptance) during interpretation of explanations. Recent human-centered XAI work has also advocated for conceptualizing ways to foster trust via reflection ''~\cite{ehsan2021explainability}

%%% EXTRINSIC TRUST
% - extrinsic trust~\cite{jacovi2021formalizing}
% extrinsic trust requires documentation and demonstration of validity of model or evaluation scheme (supported by IMCs):``Extrinsic trust is gained by two independent requirements: (1) when the model is trustworthy, and (2) when the evaluation scheme is trustworthy. To show that some evaluation scheme is ‘trustworthy’ is to justify that the distribution of instances during evaluation matches the distribution of the true unseen instances that will require trust (in a specific contract) by the user in the future''; ``A key motivation of XAI and interpretability is to (1) increase the trustworthiness of the AI, (2) in- crease the trust of the user in a trustworthy AI, or (3) increase the distrust of the user in a non-trustworthy AI, all corresponding to a stated contract, so that the user develops warranted trust or distrust in that contract.''~\cite{jacovi2021formalizing}
% - Formalizing Trust in Artificial Intelligence: Prerequisites, Causes and Goals of Human Trust in AI~\cite{jacovi2021formalizing}
% trust and skepticism:`` We discuss a model of trust inspired by, but not identical to, interpersonal trust (i.e., trust between people) as defined by sociologists. This model rests on two key properties: the vulnerability of the user; and the ability to anticipate the im- pact of the AI model’s decisions. We incorporate a formalization of ‘contractual trust’, such that trust between a user and an AI model is trust that some implicit or explicit contract will hold, and a formalization of ‘trustworthiness’ (that detaches from the notion of trustworthiness in sociology), and with it concepts of ‘warranted’ and ‘unwarranted’ trust.; ``The ability to anticipate is a goal, but not necessarily a symp- tom, of Human-AI trust. The ability or inability of the user to anticipate the behavior of an AI model in the presence of uncertainty or risk, is not indicative of the existence or absence of trust. We illustrate this in §4. We stress that anticipating intended behavior is the user’s goal in developing trust, but not necessarily the AI developer’s goal.'' acknowledgment of risk:``The assessment of risk is necessary prior to the assessment of trust. When deciding whether an AI requires trust, or when evaluating trust, verify the existence of vulnerability of the user in the actions of the AI, by: (1) verifying that the user considers some of the actions of the AI as unfavorable to them; and (2) verifying that the user considers both the favorable and unfavorable outcomes as realistic.''~\cite{jacovi2021formalizing}
% acknowledgment of risk:``The assessment of risk is necessary prior to the assessment of trust. When deciding whether an AI requires trust, or when evaluating trust, verify the existence of vulnerability of the user in the actions of the AI, by: (1) verifying that the user considers some of the actions of the AI as unfavorable to them; and (2) verifying that the user considers both the favorable and unfavorable outcomes as realistic.''~\cite{jacovi2021formalizing}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Model Cards and Documentation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Nazneen's original text:
% Model cards have been foundational in standardizing documentation for communicating and sharing AI/ML model performance and characteristics~\cite{mitchell10.1145/3287560.3287596}. The motivation behind model cards has been to convey intended use cases for a trained ML model which in turn requires evaluating the model on different subpopulations of data. With the very limited evaluation information in model cards, it is difficult for most users to infer such use cases. Robustness Gym overcomes this limitation by generating robustness reports that summarizes model performance on various data slices via the process of contemplate, create, and consolidate~\cite{goel2021robustness}. Both model cards and robustness reports have limited information on the training data and its characteristics. The work on datasheets for datasets has been instrumental in bridging this gap~\cite{gebru2021datasheets}. 

% Building on the work on documenting model and data is the line of work on documenting model explanation characteristics via \textit{factsheets} and \textit{worksheets}~\cite{sokol10.1145/3351095.3372870}. The authors lay out five dimensions for evaluating explainable systems -- functional, operational, usability,
% safety and validation, some of which have been the basis for our work on evaluating and comparing various model documentation works including SMC, RGR, and the IMC (Section ~\ref{sec:study_one}). Our visual design of the IMC builds on some of the same design principles as the VBridge, a framework for standardized reporting of features, explanations, and data for healthcare models~\cite{cheng2021vbridge}.



% TODO - didn't use this but it is relevant: Fifty Shades of Grey: In Praise of a Nuanced Approach Towards Trustworthy Design~\cite{thornton10.1145/3442188.3445871}
% context: virtual labs for data scientists to collaborate: ``In the early stages of designing this Virtual Lab, it was presumed that well-known trust- supporting properties would need to be incorporated to achieve intended trust: (1) Transparency: providing collaborators access to relevant in- formation to determine trustworthiness of the items in the repository; (2) Provenance: preserving workflow through notebook tech- nologies integrated with version control (possibly incorpo- rating blockchain); (3) Security: balancing openness with some assurance of privacy for collaborators.'';``Before launching into our examination of how provenance and transparency relate to trust in the context of Virtual Labs, we must briefly expand upon the point made within Sect. 2.3 that they are both delivered via the mechanism of documentation. Documen- tation is thought to afford trust through visibility, inspectability, and the provision of contextual information for stakeholders to use relative to their needs and goals, e.g. functional affordances ''~\cite{thornton10.1145/3442188.3445871}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Governance and Accountability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% INFORMED CONSENT
% - Governance and consent~\cite{giannopoulou2020algorithmic};
% - Indigenous principles for consent~\cite{carroll2020care} 

%%% GOVERNANCE STRATEGIES
% - Effective governance for HCAI requires opportunities for independent oversight (the focus of this paper diverges from our goals but the points about trustworthiness requiring oversight are relevant enough to be included)~\cite{shneiderman2020bridging};
% ``This article attempts to bridge the gap between widely discussed ethical principles of Human-centered AI (HCAI) and practical steps for effective governance. Since HCAI systems are developed and implemented in multiple organizational structures, I propose 15 recommendations at three levels of governance: team, organization, and industry. The recommendations are intended to increase the reliability, safety, and trust- worthiness of HCAI systems: (1) reliable systems based on sound software engineering practices, (2) safety culture through business management strategies, and (3) trustworthy certification by independent oversight.''-audit trails, bias testing, explainable UIs, internal reviews, industry standards, regulation, auditing firms, NGOs and civil society, and beyond; ``right to explanation''~\cite{shneiderman2020bridging}

%%% FRAMEWORKS AND TOOLKITS
% - Closing the AI Accountability Gap: Defining an End-to-End Framework for Internal Algorithmic Auditing~\cite{raji2020closing};
% ``In this paper, we introduce a framework for algorithmic auditing that supports artificial intelligence system development end-to-end, to be applied throughout the internal organization development life- cycle. Each stage of the audit yields a set of documents that together form an overall audit report, drawing on an organization’s values or principles to assess the fit of decisions made throughout the pro- cess. The proposed auditing framework is intended to contribute to closing the accountability gap in the development and deployment of large-scale artificial intelligence systems by embedding a robust process to ensure audit integrity.''``Nevertheless, such principles are becoming common methods to define the ethical priorities of an organization and thus the operational goals for which to aim [34, 83]. Thus, in the absence of more formalized and universal standards, they can be used as a North Star to guide the evaluation of the development lifecycle, and internal audits can investigate alignment with declared AI principles prior to model deployment. We propose a framing of risk analyses centered on the failure to achieve AI principle objectives, outlining an audit practice that can begin translating ethical principles into practice.''lessons from other industries: design s, traceability, failure modes and effects analysis, `design control' procedures to ensure that design requirements are met and designs and development processes are auditable'' - and associated design history files; intended use documentation; structural vulnerabilities assessments; audit infrastructure - e.g., internal auditors should identify, analyze, evaluate and record sufficient information to achieve the audit objectives. The head of internal audit determines how internal auditors carry out their work and the level of evidence required to support their conclusions. SMACTR internal audit framework including artifacts produced by auditors, engineering/product teams, and jointly developed artifacts -- scoping, mapping, artifact collection, testing, reflection, post-audit -- incorporates AI principles, model cards, datasheets, and human-centered auditing approaches;``Fair- ness, justice and ethics require that those bearing these risks are given due attention and that organizations that build and deploy artificial intelligence systems internalize and proactively address these social risks as well, being seriously held to account for system compliance to declared ethical principles.''~\cite{raji2020closing}

% - WeBuildAI: Participatory Framework for Algorithmic Governance~\cite{lee2019webuildai}

% - Outlining Traceability: A Principle for Operationalizing Accountability in Computing Systems~\cite{kroll10.1145/3442188.3445937}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Auditing or Certifying AI/ML Systems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{Auditing or Certifying AI/ML systems}
% \textcolor{blue}{This will be integrated into governance/accountability section but leaving it here for now}
% Algorithmic audits seek to evaluate AI models for issues of robustness, bias, and fairness. \textcolor{blue}{<- Draws from several references}
% - Actionable Auditing: Investigating the Impact of Publicly Naming Biased Performance Results of Commercial AI Products~\cite{raji2019actionable}
% Algorithmic audits seek to evaluate public AI systems in order to motivate the corporations to address algorithmic bias, and have been shown to be effective at reducing bias in targeted companies compared to other companies ~\cite{raji2019actionable}.
% Public audits have been shown to be effective at reducing bias in targeted companies compared to other companies ~\cite{raji2019actionable}.
% - Ethics‑Based Auditing to Develop Trustworthy AI~\cite{mokander2021ethics};
% Audits can be conducted by third-party actors, or incorporated into internal processes. Auditing should be a structured, ongoing process that is designed from a system perspective. However, many challenges remain from a conceptual, technical, economic, and organizational perspective ~\cite{mokander2021ethics}.
% - \textcolor{blue}{(maybe?)Auditing Digital Platforms for Discrimination in Economic Opportunity Advertising~\cite{kingsley2020auditing}};
% Large scale algorithmic audits have revealed discrepancies in the visibility of socionomic opportunities to different demographic groups~\cite{kingsley2020auditing}. \textcolor{blue}{<- This was mentioned as a "maybe". Could also be a second citation for the importance of systematic approaches as mentioned in previous reference, since this one also discuss importance of systematic approach.}
% - Fairness Through Robustness: Investigating Robustness Disparity in Deep Learning~\cite{nanda10.1145/3442188.3445910}
% Many of these systems evaluate ML systems under normal operating conditions, which may not be sufficient in the case of an adversarial attack against a particular subgroup~\cite{nanda10.1145/3442188.3445910}.
% - Certified Robustness to Programmable Transformations in LSTMs~\cite{zhang2021certified}
% In contrast to posthoc audits and evaluations, \textit{certificates} of robustness provide algorithmic guarantees on the performance of models under certain conditions ~\cite{zhang2021certified}. 
% - Everyday Algorithm Auditing: Understanding the Power of Everyday Users in Surfacing Harmful Algorithmic Behaviors~\cite{shen10.1145/3479577}
% Human-in-the-loop auditing processes can leverage everyday users to provide further protection once a system is deployed \cite{shen10.1145/3479577}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Practitioner Needs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{Particular Needs for Industry Practitioners}
% - Improving Fairness in Machine Learning Systems: What Do Industry Practitioners Need?~\cite{holstein2019improving};
% % ``Through 35 semi-structured interviews and an anonymous survey of 267 ML practitioners, we conduct the first systematic investigation of commercial product teams’ challenges and needs for support in developing fairer ML systems.'';``While media coverage of biases and unfairness in ML systems often uses a “bias in, bias out” framing, emphasizing the cen- tral role of dataset quality [42, 107], the fair ML research lit- erature has overwhelmingly focused on the development of algorithmic methods to mitigate biases, viewing the dataset as fixed [23, 59]. However, many of our interviewees reported that their teams typically look to their training datasets, not their ML models, as the most important place to intervene to improve fairness in their products''``It’s almost like the wild west." Most interviewees reported that their teams do not currently have processes in place to support the collection and curation of balanced or repre- sentative datasets. A software engineer (R7) described their team’s current data collection practices as “almost like the wild west” and a data scientist (R10) noted that “there isn’t really a thought process surrounding... ‘Should [our team] in- gest this data in?’ [...] If it is available to us, we ingest it.'';``Detecting potential fairness issues presents many unique au- diting challenges. Interviewees often described their teams’ current fairness auditing processes as reactive—with efforts tightly focused around specific customer complaints—in con- trast to their teams’ proactive approaches for detecting po- tential security risks.''``Much of the existing fair ML literature has focused on do- mains such as recidivism prediction, automated hiring, and face recognition, where fairness can be at least partially understood in terms of well-defined quantitative metrics (e.g., between-group parity in error rates or decisions [21, 26, 65]). However, interviewees working on applications in- volving richer, complex interactions between the user and the system—such as chatbots, automated writing evaluation, adaptive tutoring and mentoring, and web search—brought up needs for more holistic, system-level auditing methods.''``Interviewees revealed a range of challenges and needs around debugging and remediation of fairness issues once detected. These included, among others, needs for support in identify- ing the cheapest, most effective strategies to address particu- lar issues; methods to estimate how much additional data to collect for particular subpopulations; processes to anticipate potential trade-offs between specific definitions of fairness and other desiderata for an ML system (not limited to pre- dictive accuracy); and frameworks to help navigate complex ethical decisions (e.g., the fairness of fairness interventions).'' ~\cite{holstein2019improving}
% - Each to His Own: How Different Users Call for Different Interaction Methods in Recommender Systems~\cite{knijnenburg2011each}
% % ``This paper compares five different ways of interacting with an attribute-based recommender system and shows that different types of users prefer different interaction methods. In an online experiment with an energy-saving recommender system the inter- action methods are compared in terms of perceived control, understandability, trust in the system, user interface satisfaction, system effectiveness and choice satisfaction. The comparison takes into account several user characteristics, namely domain knowledge, trusting propensity and persistence.''-relevance: granular control is preferred; ``A recommender system is in essence a persuasive system [8]; it tries to persuade its users to follow its recommendations. Komiak and Benbasat show that users’ trust in the system influences how well this persuasion works: only users who trust the system will continue to use it [15]. Trust in the system can be developed over an extended period of interaction with a recommender system. However, in the initial interaction period, trust in the system is mainly influenced by users’ general trusting propensity [27].''TODO - check how they are defining trusting propensity. I'm suspicious~\cite{knijnenburg2011each}
% - Grounding Interactive Machine Learning Tool Design in How Non-Experts Actually Build Models~\cite{yang2018grounding}
% % appropriate modes of interaction depend on upon user characteristics, including a priori propensity for trust in AI/ML-driven systems as well as domain expertise~\cite{yang2018grounding}
% - The Role of Domain Expertise in User Trust and the Impact of First Impressions with Intelligent Systems~\cite{nourani2020role}
% % domain expertise and prior knowledge shapes trust in systems as well as confidence in detecting system errors, novice users show higher tendency toward automation bias; implications for design: ``more detailed explanation interface to pro- vide more information. Rather than allowing users to use a system with zero understanding or a poor mental model of how the system works, designers can incorporate intro- ductory sessions to alert users about system strengths and shortcomings so that users can decide whether and when they should trust the system’s outputs'' - implications for guidance; ``Additionally, one approach for consideration could be showcasing examples of both correct and incorrect predictions or outcomes in the beginning of usage to help experts develop first impressions, covering the variability of system capabilities to reduce the risk of encountering an unrepresentative sample by chance. Further research would need to explore the implications of such an approach. The showcasing method could also con- sider attempts to more strongly encourage users to review explanations for both correct and incorrect examples'' - different sampling opportunities for examples in each subpop (or full training/testing set) including examples with low and high confidence ~\cite{nourani2020role}
% - AI Trust Score: A User-Centered Approach to Building, Designing, and Measuring the Success of Intelligent Workplace Features~\cite{wang2021ai}
% % ``how to help product teams move increasingly towards responsible AI experiences by examining user trust within business contexts. We discuss the development, application, and validation of the AI Trust Score, which allows teams to measure the success of an AI feature from enterprise users’ perspectives. The Trust Score is a multi-dimensional metric which consists of sev- eral statements users respond to that inform their trust, including whether an AI feature helps with job efciency and efectiveness and understanding how and when to use the feature for their job role. The metric, along with usability feedback, can be adapted to encourage UX-related conversations and actions within product or feature development processes.'' - implications for how to integrate findings into product teams; ``There are at least three major distinctions with enterprise AI UX: the emphasis on users’ job efciency and efectiveness, data protection concerns, and need for understanding and control in AI features.'' - implications for sociotechnical systems and being able to defend decisions made with reliance on AI/ML systems -- documentation trails; ``Second, trust in AI is often tied to data protection concerns (e.g., privacy and security) across many industries, such as in healthcare, fnance, and banking. For example, serious ramifcations can occur when a fraud protection predictor inaccurately predicts compro- mised accounts. Furthermore, data breaches can have a profound impact on a company’s perceived privacy and security and over- all brand perception [6]. In our research, we have found that data protection is a top priority for enterprise users across industries because of compliance and usage requirements (e.g., GDPR).'' - implications for evaluating IMC wrt to safety~\cite{wang2021ai}
% - Designing Interactive Transfer Learning Tools for ML Non-Experts~\cite{mishra2021designing}
% % ``we design a prototype to understand non-expert user behavior in an interactive environ- ment that supports transfer learning. Our fndings reveal a series of data- and perception-driven decision-making strategies non-expert users employ, to (in)efectively transfer elements using their do- main expertise. Finally, we synthesize design implications which might inform future interactive transfer learning environments.''; ``Finding patterns across model outcomes: Almost all par- ticipants used the investigate output tab to identify a class where the model performed especially poorly'' - implications for samplign methods; data-centric and model-centric patterns of exploration and trust-building -- implications for IMC design incorporating both~\cite{mishra2021designing}
% - Why Does My Model Fail? Contrastive Local Explanations for Retail Forecasting~\cite{lucic10.1145/3351095.3372824}
% % ``It is difficult to convince analysts, along with their superiors, to adopt these techniques since the models are considered to be “black boxes,” even if they perform better than current models in use. We examine the impact of contrastive explanations about large errors on users’ attitudes towards a “black-box” model.'' - explanations needed for models to be adopted; ``1) feature values that would result in a reasonable prediction, and (2) general trends between each feature and the target, both based on Monte Carlo simulations. '' - instead of `why' does it fail, we offer users `when' does it fail, more interpretable for NLP~\cite{lucic10.1145/3351095.3372824}
% - Explainable machine learning in deployment~\cite{bhatt10.1145/3351095.3375624}
% % ``Explainable machine learning offers the potential to provide stake- holders with insights into model behavior by using various meth- ods such as feature importance scores, counterfactual explanations, or influential training data. Yet there is little understanding of how organizations use these methods in practice. This study explores how organizations view and use explainability for stakeholder con- sumption. We find that, currently, the majority of deployments are not for end users affected by the model but rather for machine learning engineers, who use explainability to debug the model it- self. There is thus a gap between explainability in practice and the goal of transparency, since explanations primarily serve internal stakeholders rather than external ones. Our study synthesizes the limitations of current explainability techniques that hamper their use for end users. To facilitate end user interaction, we develop a framework for establishing clear goals for explainability.''; their recommendations: identify and engage with stakeholders and understand the purpose of explanation~\cite{bhatt10.1145/3351095.3375624}
% - Where Responsible AI meets Reality: Practitioner Perspectives on Enablers for Shifting Organizational Practices~\cite{rakova10.1145/3449081}
% % ``We present the results of semi-structured qualitative interviews with practitioners working in industry, investigating common challenges, ethical tensions, and effective enablers for responsible AI initiatives. Focusing on major companies developing or utilizing AI, we have mapped what organizational structures currently support or hinder responsible AI initiatives, what aspirational future processes and structures would best enable effective initiatives, and what key elements comprise the transition from current work practices to the aspirational future.''; ``Three recruit- ing criteria were used to find interviewees: (1) did they work closely with product, policy, and/or legal teams, (2) did the outputs of their work have a direct impact on ML products and services, and (3) were some aspects of their work related to the field of responsible AI.''; ``This means pushing for changes in those structures and processes, as their goals may be an- tithetical to what is currently supported by the organizational structure. Thus, individuals who want to bring responsible AI issues into their work must do their own jobs, do the responsible AI work if that is not their official job, do the difficult work of redesigning organizational structures around them to accommodate the responsible AI work, and on top of it all, do the change manage- ment to get those new organizational practices to be adopted.'' - need for organizational structures to support change (we do not address but share these implications)~\cite{rakova10.1145/3449081}
% - How do People Train a Machine?: Strategies and (Mis)Understandings~\cite{sanchez10.1145/3449236}
% % ``Machine learning systems became pervasive in modern interactive technology but provide users with little, if any, agency with respect to how their models are trained from data. In this paper, we are interested in the way novices handle learning algorithms, what they understand from their behavior and what strategy they may use to “make it work”. We developed a web-based sketch recognition algorithm based on Deep Neural Network (DNN), called Marcelle-Sketch, that end-users can train incrementally. We present an experimental study that investigate people’s strategies and (mis)understandings in a realistic algorithm-teaching task. Our study involved 12 participants who performed individual teaching sessions using a think-aloud protocol. Our results show that participants adopted heterogeneous strategies in which variability affected the model performances. We highlighted the importance of sketch sequencing, particularly at the early stage of the teaching task.''; recommendations: guidance for building teaching curricula; allow modification of teaching actions and sequences of actions; assist supervised data augmentation; show optimization inertia and model's state changes; -- primarily implications for guidance ~\cite{sanchez10.1145/3449236}
% - Human Factors in Model Interpretability: Industry Practices, Challenges, and Needs~\cite{hong2020human}
% % ``As the use of machine learning (ML) models in product development and data-driven decision-making processes became pervasive in many domains, people’s focus on building a well-performing model has increasingly shifted to understanding how their model works. While scholarly interest in model interpretability has grown rapidly in research communities like HCI, ML, and beyond, little is known about how practitioners perceive and aim to provide interpretability in the context of their existing workflows.''; ``The characterization of interpretability work that emerges from our analysis suggests that model interpretability frequently involves cooperation and mental model comparison between people in different roles, often aimed at building trust not only between people and models but also between people within the organization. ''; recommendations: Identifying, Representing, and Integrating Human Expectations, Communicating and Summarizing Model Behavior, Scalable and Integratable Interpretability Tools, Post-Deployment Support -- implications for IMCs broadly, integrations, and approach cognizant of organizational dynamics~\cite{hong2020human}

==> Interactive Model Cards/tex/study_one.tex <==
\vspace{-2mm}
\section{Study 1 : Concept Study with ML, AI, and NLP Experts}\label{sec:study_one}

Ahead of engaging with non-expert analysts, we leveraged the expertise of researchers and practitioners in  ML/AI development, AI Ethics, and Natural Language Processing (NLP), to co-create a set of design guidelines for IMCs.

%and asked them to compare examples of standard~\cite{mitchell10.1145/3287560.3287596} and interactive model cards for a sentiment analysis tasks.  %We also ask them to reflect on their experience and practices using standard model cards (SMCs) in their work as well as from the perspective of a non-expert analyst. 

%Our first study aimed to develop a functional prototype of an interactive model card. Rather than rely solely on our expertise to develop this prototype, we sought to draw on the perspectives of experts in ML/AI development and design, AI ethics, and Natural Language Processing (NLP). \
%, asking them to engage with three different forms of model documentation: standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, robustness gym reports (RGRs)~\cite{goel2021robustness}, and a concept we propose for an interactive model card (IMC). We asked them to reflect on the strengths and limitations of different modalities of documenting and explaining model behavior both from their experiences as experts in their respective fields and how they would expect a less technical data worker to respond. 

%Our findings from this study provide a set of design guidelines that inform the development of an IMC prototype that we assessed in a second study with non-experts (Section~\ref{sec:study_two}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONCEPT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{-2mm}
\subsection{Design Probes}\label{sec:studyone_probes}
%In this conceptual study, we compared three designs of model cards : the standard model card~(SMC) from Mitchell~\textit{et al.}~\cite{mitchell10.1145/3287560.3287596}, and robustness gym report~(RGR), and our concept for an interactive model card~(IMC). %We develop design probes~\cite{Wallace:design_probes:2013} of these model cards using a reference model card for a sentiment analysis task.
%Ahead of the study we created conceptual prototypes of an SMC, RGR, and IMC that would serve as design probes in our study.  Here we briefly describe the source material used to develop these design probes and the IMC specifically. Additionally, we delineate the scope of our initial design investigations. We evaluate the soundness of these design assumptions with experts.


\noindent\textbf{Design Scope for Interaction.} There are many ways that interactivity could be theoretically added to model cards. In this study, we have scoped the goals of interaction design to focus on disaggregated performance metrics, as well as understanding the model's training data and how it compares to the analyst's. 
% Other ways to add interactivity that could have explored, but which we did not, include: 
We chose not to explore other sorts of interactivity, such as: comparing models (i.e., multiple sentiment analysis models), comparisons across multiple datasets, or training the model on the analyst's own data. We focus on disaggregated model performance and dataset understanding and comparison because we 
% argue these are important 
view these as key
tasks for understanding a single model that are undersupported with an SMC. Moreover, understanding the model's performance and data conforms to what we consider the spirit of the SMC, which is to inform the reader about a single model.
% , without adding the significant analytic overhead that multiple model or dataset comparisons would require. 
%. Within the scope of a model card we see potential to add such interactivity to help people understand the model's training and test data as well as its performance. There exist many alternative designs that would support this interaction and here we focus on two. The first was disaggregating performance metrics with custom subpopulations in the model's training and testing data. We see opportunities to use interaction to allow others to define subpopulations that are pertinent to them. The second area of focus was a set of  visualizations that enable people to compare data pertinent to them against the model's training and testing data. 

%We developed elements of both visual and information design that are intended to provide a scaffolding to encourage engagement of the interactive elements. Moreover, if people would choose not to interact, these elements could still offer a comprehensive and static overview of the model.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Phase_I_concept_probes.pdf}
    \caption{Concept of an Interactive Model Card. Larger images of the SMC, RGR, and IMC are available in the \href{https://osf.io/9d83t/?view_only=7359695185b04468a7ae4a2e189691c0}{online materials}}
    \Description{An illustration of the interactive model card conceptual probe that was used to in the first study with AI/ML experts. The probe is annotated with boxes in three colors : orange, purple, and green that show elements of the standard model card, robustness gym report, and the new elements of the interactive model card - respectively. The Standard model card sections contain abbreviated text from the SMC, which we describe in the main text. The robustness gym report shows a bar chart with three facets; each facet is a different model metric. The rows of the bar chart show different slices of the data that are automatically generated by Robustness Gym. The three new elements of the interactive model card as a follows. First, a data upload panel that sits underneath the standard model card and allows users to upload their own dataset. Next, a data comparison panel that is adjacent to the Robustness Gym report and shows a scatter plot to the dataset that the model was trained on. Below that is the Example Generation panel where the user can dynamically create new sentence or data set slices to evaluate the model on. }
    \label{fig:phaseI_concepts}
    \vspace{-5mm}
\end{wrapfigure}

\noindent\textbf{Reference Model Card: Task, Model, and Data}. We use a reference model card of DistilBERT~\cite{sanh:distilbert:2020} fine-tuned on the SST-2~\cite{socher:sst-2:2013} dataset for a sentiment analysis task; this reference mode is sourced from \href{https://huggingface.co/}{HuggingFace}~\cite{wolf:huggingfaces:2020}. We chose to focus on a sentiment analysis task because it is widely known and easily understood, while still being representative of NLP model development regimens for other tasks. Moreover, the DistilBERT SST-2 fine-tuned model presented a unique challenge for generating design probes because it is technically three models: a pretrained general language model, its distillation, and the fine-tuned version optimized for a sentiment analysis task. We found that this challenged the SMC paradigm, since it was not clear how much information to include (if any) of the prior base models. To explore this problem, we decided to use the text from \textit{both} the DistilBERT and SST-2 fine-tuned model cards\footnote{\href{https://huggingface.co/distilbert-base-uncased-finetuned-sst-2-english}{distilbert-base-uncased-finetuned-sst-2-english} commit \texttt{03b4d19}}. %We also saw opportunities to explore how much experts and non-experts alike rely on information for all of these models.


%To create the SMC and IMC, we use the text for both the fine-tune and base DistilBERT model card. 

%\noindent\textbf{Task, Model, and Data.} We chose a single sentiment analysis task for this study because we believed this approach would allow for a focused study and analysis. We also acknowledge this focus as a potential limitation of our study, and we will return to this discussion in Section~\ref{sec:discussion}. We target sentiment analysis because it is a relatively common task and as such the scenario would require little to no explanation for study participants. 
%We constructed an SMC, RGR, and IMC based upon a DistilBERT model that was fine-tuned on the SST-2 dataset. We used a specific DistilBERT SST-2 fine-tuned checkpoint that is available on HuggingFace (\url{https://huggingface.co/})\footnote{\href{https://huggingface.co/distilbert-base-uncased-finetuned-sst-2-english}{distilbert-base-uncased-finetuned-sst-2-english} commit \texttt{03b4d19}; \href{https://huggingface.co/distilbert-base-uncased}{distilbert-base-uncased} commit \texttt{b22dbc4}; SST-2 dataset} because it had a rich existing model card that we could adapt and use in our study. Hence forth we refer to this as the \textbf{\textit{reference model card}}. The DistilBERT SST-2 model presented a unique challenge for our overall design process because it is a fine-tuned, distilled version of a larger pre-trained general language model. We had open questions of how much information to include (if any) about the DistilBERT and BERT models.

\vspace{1mm}
\noindent\textbf{Design Probes and Interactive Model Card Concept.} We developed design probes~\cite{Wallace:design_probes:2013} of an SMC, RGR, and IMC. For the SMC, we used the all the text from the reference model card, with some exceptions, laid out according to the specifications in Mitchell~\textit{et al.}~\cite{mitchell10.1145/3287560.3287596}. Because the reference model card does have some interactivity (the ability to test your own sentence), we included that as well. An RGR unifies four common evaluation paradigms including performance on data subpopulations, which we explore in this concept study.  We developed an RGR probe using the built-in subpopulations to which we added a custom set of potentially sensitive subpopulations (i.e., race, gender, etc.).

Our IMC concept~(\autoref{fig:phaseI_concepts}) includes redeveloped elements of the SMC and RGR.
%Our concept for an interactive model card~(\autoref{fig:phaseI_concepts}) includes elements of the standard model card (shown with orange borders) and robustness gym report (shown with pink borders). 
We proposed adding interactive elements (shown with green border) that would allow users to upload their own data (\texttt{data upload panel}), add their own sentences (\texttt{example generation panel}), and/or define new subpopulations from the model's training and test datasets for exploration (\texttt{example generation panel}). We also include an interactive data comparison visualization (\texttt{data comparison panel}) that shows the sentence embeddings of the model's data together with the analyst's data. We implemented the design probes as paper prototypes using Google Slides. For the IMC we mocked up interactions through slide links, transitions, and animations. Text for these paper prototypes was taken verbatim, with some small exceptions, from the existing \texttt{DistilBERT} and the \texttt{SST-2 fine-tuned} model cards.

%We additionally arrived at defaults for the information and visual design (~\autoref{fig:phaseI_concepts}). %For the information design, we combined information from the fine-tune and based models and reduced the amount of initial viewable text, but enabling the person to get more details on demand. For the visual design, we use the robustness gym report but included pre-defined subpopulations within the models train and test data that may be indicative minority populations (i.e. Black Americans) alongside other categories (i.e. comedy). 

% of uploaded data and singleton sentences or subpopulations of the train and test data.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% STUDY PROCEDURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{-3mm}
\subsection{Study Procedures}\label{study_one:general_procedures}

\subsubsection{Study Design} 
% We conducted a semi-structured interviews. Ahead of the study, we prepared a study script and slide deck of conceptual design probes (Section~\ref{sec:studyone_probes}) that we used throughout the interviews. 
Our study comprised semi-structured interviews using a grounded approach~\cite{muller2014curiosity} and incorporated conceptual design probes (Section~\ref{sec:studyone_probes}).
Study sessions were scheduled for 60 minutes, and participants were offered an honorarium of \$150 upon completion.
% Study sessions are available in online materials, 
Full study protocols and materials are available in the online materials, 
while here we provide only a brief overview. During the study, participants were asked about their background and familiarity with model cards, Robustness Gym reports, or other types of model documentation. They were then shown examples of a standard model card, a Robustness Gym report, and our concept for an interactive model card (Section~\ref{sec:studyone_probes}). They were asked to explore each of the forms in a think-aloud protocol, and the study moderator also prompted them 
% with predefined questions from the protocol. 
with additional questions related to their interpretations and needs for understanding the model.
% When providing their feedback, participants were asked to additionally consider whether the model cards would be suitable for an analyst persona, Jenn, who uses a language model for a sentiment analysis task, but who did not have a formal education in computer science, statistics, or machine learning, and cannot write code:
As they considered each of these forms of model documentation, we asked participants to reflect on the strengths and limitations through two lenses: their own needs as experts and those of a non-expert analyst using a sentiment analysis model in their work (see the \href{https://osf.io/9d83t/?view_only=7359695185b04468a7ae4a2e189691c0}{online materials}).

%\begin{quote}
%\footnotesize
%\textit{Jenn is a marketing analyst with CloudyShoes Inc. She is running a campaign to %\textbf{analyze the sentiment of social media posts} that feature CloudyShoes’ products. She uses a sentiment analysis model to understand its performance across different customer segments. Jenn primarily uses a interface to do her analysis. \textbf{Though she has no formal training in machine learning or natural language modeling, she has a high-level understanding of natural language models} and has been using them for some time to help her work.}
%\end{quote}  

\input{tables/study_one_participants}
\vspace{-2mm}
\subsubsection{Recruitment}
We set a target of 10 participants aiming to recruit at least one participant from each of the following categories: ML/AI development and design,  Ethics, and NLP.  We reached out to 23 participants, recruiting until we had met our target study size. Of the 13 participants who were not included in our study, five declined and the rest did not respond.  We recruited participants based upon their publication or professional history using a combination of personal connections and cold emails. All participants had exposure to documentation for ML/AI models in some form, but only six were familiar with model cards and two with RGRs.

\vspace{-2mm}
\subsubsection{Data Collection and Analysis}\label{study_one:qual_coding}
Data collection included observer notes and video recordings for participants who consented to recording. We recorded approximately 11 hours and 15 minutes of video, including the interview and an on-camera debrief between the study moderator and note taker. Video transcripts were automatically generated, including speaker identification, and were verified for accuracy by the authors. We conducted iterative \textit{thematic analysis}~\cite{charmaz2014constructing}, surfacing initial codes through debriefs and review of transcripts. The first author then conducted focused coding for all transcripts, and both first authors synthesized themes and categories. All authors also surfaced implications that informed the design of our \textit{IMC functional prototype} (Section~\ref{study_two:functional-prototype}).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Results}
In~\autoref{tab:studyone_tab} we summarize five interconnected conceptual dimensions of participant perspectives on our probes. 
%We discuss each of these categories in detail below, along with the implications they raise for designing interpretable and useful model documentation.

%%%%%% QUOTE TABLE  %%%%%% 
\input{tables/study_one_quotes}
%%%%%% QUOTE TABLE  %%%%%% 


\subsubsection{Stakeholders}\label{study_one:res_stakeholders}
Without prompting, participants described additional stakeholders or students and the scenarios in which they share model cards or other documentation (e.g., related to model performance and tuning). One participant succinctly summarized that SMCs remained relatively untested with non-expert analysts: 
\vspace{-1mm}
\begin{quote}
\small
    \textit{``At least for the next couple of years, people are going to be using model cards for the first time. And these are going to be concepts that may be new for many individuals. And so giving them some hand-holding, as to `What does this mean, what am I supposed to do with this?' I think will be extremely helpful.''} [E02]
\end{quote}
\vspace{-1mm}

Several participants (n=6) articulated that the language and layout of the SMC appeared better suited for software or machine learning engineers. One participant suggested that the SMC seemed \textit{``very on the back end...like it feels like GitHub'' }[E01], which they felt would not resonate with stakeholders who are using, but not implementing, models. Moreover, three participants reflected that some of these specialized terms of art (i.e., accuracy, precision, recall) can be difficult for even students of ML and NLP; one participant said their students needed a `cheat sheet' of the terminology.

%n the model card can be inaccessible even to students of machine learning.% One informant offered that their graduate and undergraduate students regularly used a `cheat sheet' reminding them of the ML and NLP terminology.
% For Jenn's persona,  all participants expressed doubt that she would understand the model card information or know how to act on it.
All participants expressed doubt that a non-expert analyst would understand the model card or know how to act on the information it contained.
One participant suggested  that an IMC could be more accessible to individuals across different roles, particularly if the design supported different information architectures or prioritization of information.  In contrast, another participant [E07] was emphatic that standardization was a critical component of model cards and should be preserved. They argued that interactivity adds subjectivity to model cards that should be visually distinct.% from more standard information.
%They went further to suggest that adding interactivity could be beyond the scope of a model card and should be considered they advocated that if we were to pursue supporting user input to the model card via interactivity, then we should ensure that interactive components are visually distinct from the standard model card information.

\vspace{-1mm}
\subsubsection{Design Considerations}
Participants critiqued the information design of all model cards; for the RGR and IMC, they also offered feedback on visual and interaction design. Most (n=6) participants identified overly technical language and jargon as a key failing of all of the model cards, and they proposed alternative language to capture the same meaning in more accessible ways. All participants said the amount of text in the standard model card made it difficult to quickly skim and understand the model. % Participants appeared to prefer the ``overview first, details on demand''~\cite{shneiderman1996eyes} view from the IMC, which we achieved through bullet point summaries with modal pop-ups for more details; one participant proposed a list expansion interaction over a modal pop-up. 
Most (n=8) participants expressed that the visual design and layout of the IMC helped their  \textit{``eyes [...] focus on information that [they] missed before''} [E04] compared to the SMC and RGR. However, a sense of focus/overwhelm varied among participants, and one participant articulated that the IMC contained \textit{``too much information and is very cluttered''} [E04]. Four participants stated that a summary of the model's purpose (i.e., ``this is a sentiment analysis model'') was needed and that it would improve the readability of the model card. Relatedly,  participants also pointed out areas in the RGR and IMC where they thought different information should be prioritized or emphasized (e.g., changing the color of the size column on the rightmost side of the RGR or emphasizing it in another way). Lastly, many participants suggested adding or emphasizing higher-level metrics about performance (e.g., making overall performance visually distinct from disaggregated performance).

\vspace{-1mm}
\subsubsection{Guidance} 
Participants indicated that various stakeholders would need help making sense of the information in the model card. Six participants emphasized the importance of providing specific guidance to help participants understand the information on the model card. 
% This guidance included simple actions like
Some forms of guidance suggested included
providing definitions, or visual cues in the form of nudges and warnings. One participant articulated that explainers for visualizations would be helpful because \textit{``it's pretty but..but what would I do [with it?]''} [E03]. One participant saw the direct potential for using interaction to provide guidance, suggesting that it \textit{``would help me [...] dig deeper''} [E01] into the model details.

Other forms of guidance were complex and geared more toward \textit{``help[ing] me understand why this matters [and] how does it help me make more informed decisions?''} [E02]. Supporting interpretability is complex but nearly all (n=7) participants indicated that examples could provide some useful guidance. However, having an effective default example to prompt end-users was also important 
% because \textit{``defaults are complex in language, so what  do you start with?''}
[E04]. Another participant suggested that leveraging examples with interactivity could help 
% people like Jenn 
non-expert analysts
\textit{``build a better mental model of how the model works and what it lacks''} [E05].

\vspace{-1mm}
\subsubsection{Trust and Safety}\label{study_one:trust_safety}
Ethics and safety considerations 
% resulted in a lively discussion. 
were a top concern.
The reference model card (Section~\ref{sec:studyone_probes}) had a short ethical considerations text, but many participants took exception with the training dataset being described as ``fairly neutral'' (\textit{``what does that mean even?''} [E08]).  One commented that Silicon Valley tends to apply a standard set of \textit{``moral values application across global and cultural contexts''} [E07], which diminishes the value of such ethical statements and assessments. Increasingly, such statements are seen as a \textit{``cop-out because it just kind of says `there is some bias somewhere' which is not entirely helpful.''} [E06]. Two participants suggested stating explicitly whether bias assessments had been conducted, and one suggested raising a warning if such bias analyses are not run. Several (n=4) participants expressed that it could be beneficial to add sensitive populations to the disaggregated model performance, but they suggested caution since the definition of these groups was culturally and geographically contextual. Moreover, they 
% also called out issues with displaying 
emphasized the need to prominently display
the total size of these subpopulations (and others) to support valid interpretation. 
% For example, one participant initially thought the model performed well in the `black' subpopulation, then saw the small sample size and revised their interpretation. 
For example, one participant initially thought the model performed well for a particular subpopulation, then saw the small sample size and revised their interpretation. 
Participants indicated that for these issues and overall, greater attention to information, visual, and interaction design would improve trust and safety. 
%Several participants also suggested pre-populating the RGR visualization with specific vulnerable populations, making them prominent, and pointed to risk taxonomies that defined such groups. However, one participant cautioned that at-risk or marginalized groups are different across the world, and the default inclusion of such populations is not always meaningful and needs to be customizable to regional contexts. Additionally, four participants specifically called out issues with the display of the sample size as an area for improvement. Tying together elements of both visual design and guidance, they emphasized that calling attention to potentially unreliable results here and other areas of the model card would improve trust and safety in the information.

\vspace{-3mm}
\subsubsection{Sensemaking and Skepticism} 
% The ideas of the previous themes came together 
Some of the themes above converged 
as participants discussed the ways they believed non-expert analysts 
% like Jenn 
would explore and make sense of information in the model cards. 
Participants tied interaction positively to these themes, indicating that it would be beneficial to \textit{``allow domain experts to be able to interrogate the models and formulate rules that are semantically meaningful to test against the model'' [E08]}. Importantly, the interactivity would enable people to \textit{``elicit more questions'' } [E04] that allowed them to form and test their mental models about the data and better \textit{``see the things that model lacks''} [E05].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Design Guidelines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\subsection{Summarizing Design Guidance for an Interactive Model Card}\label{study_one:design_guide}
From our findings in this first study, we distilled a set of design guidelines (\textbf{DG}) to inform our functional IMC prototype.
Based on what we learned from experts, these guidelines have broad implications for the documentation of AI/ML models and would be applicable beyond the task presented in the design probe.

% \noindent\textbf{DG1: Give careful deliberation to the design of information.}
\noindent\textbf{DG1: Give careful deliberation to the design of information hierarchies, representations, and interactions.}
%\hl{or DG1: Develop and evaluate design of information to meet with stakeholder experience and needs}
% Our concept study shows that the SMC is concerned primarily with the type of information that model documentation should contain. 
Prior work related to SMCs has focused primarily on the categories and depth of information that model documentation should include. However, to be sure that this content is effectively understood by a wide audience, the hierarchy and design of this content is equally important. Without this consideration, a model card may fail in its goals. Our conceptual study emphasized the importance of information design within both standard and interactive model cards. This includes the judicious use of language, visual cues, layout, data visualization, and interaction. Critically, our study cautions that the act of information design must be deliberate and, we argue, testable to be sure it is accurately interpreted.


%but this study shows that the design of the information is equation important. 

%While the standard model card provides a backbone for information hierarchy and design, it doesn't go far enough. The card's textual information needs to be further prioritized to help stakeholders read the document. Moreover, with the interactive model card a careful and visible delineation must be made between standard data that everyone sees and modifications made via interactions. We observed that participants preferred an `overview first, details on demand''~\cite{shneiderman1996eyes} to at first get a general overview of the model and then dive deeper as they desired. For fine-tuned models, information architecture is especially important balance what the different models might do.

%\vspace{0.25mm}
%\noindent\textbf{DG2: Emphasize actionability.} SMC cards prioritize technical details over actionability (i.e., `what can I do with this'). While the original goal of the SMC was to emphasize both intended and unintended uses, as well as call to action
%To make model cards accessible to a wider stakeholder group simpler and more descriptive language should be used. Moreover, emphasizing actionability (i.e., `what can I do with this?') over technical details (i.e., hyperparameters) will help stakeholders contextualize the model for their needs. 

%\vspace{0.25mm}
% \noindent\textbf{DG2: Use interaction to support conceptual understanding.}
\noindent\textbf{DG2: Use interaction to help users develop conceptual understandings.}
The reference model card primarily used interaction as a preview of the model's outputs. However, experts saw the opportunity to use interaction as a way to help non-expert analysts develop their conceptual understanding of the NLP model. 
% However, this interaction is also a double-edged sword that needs to balance the subjectivity of exploration with objective details of the model and its performance. 
Interaction modalities must balance the subjectivity of contextual explorations with objective details about the model and its performance, so they should be designed and evaluated accordingly.
The final consideration for interaction is that it must be  discoverable and supported with defaults that help people orient to the affordances. %Additional guidance will be necessary to support interpretability of the outputs. Design elements that guide the analyst  are also useful even for static elements of model cards.

%\vspace{0.25mm}
\noindent\textbf{DG3: Scaffold important information with actionable guidance.} Additional guidance will be necessary to support interpretability of the outputs. SMCs have been primarily tailored toward developers and machine learning experts, 
% and non-expert analysts will struggle to contextualize this information for their own needs.
which can cause challenges for non-expert analysts who need to interpret the documentation for their own contexts.
% To better support them, analysts need guidance to understand and act on the information. 
Clear guidance can support non-experts in understanding and knowing how to act on the information.
Warnings, prompts, and summaries are all examples of guidance that participants suggested could help guide analysts in making sense of 
% the information in the model card. 
model cards.
% Furthermore, using visual cues serves to 
Visual cues can also
support the overall architecture and flow of information in the model card. 

%\vspace{0.25mm}
\noindent\textbf{DG4: Implement defaults that promote productive skepticism.} Not all readers of a model card will want to interact with it. In addition to making interaction discoverable, it should also be enticing and promote a productive skepticism about what the model does and how it can be used. We argue that this productive skepticism would make ideas of intended and unintended uses more intuitive than simply being told what they are. Choosing appropriate default information is important to encourage this kind of engagement with a model card. We propose sensitive populations as a starting point and we used the Robustness Gym technology~\cite{goel2021robustness} to automatically implement these defaults.

%Irrespective of whether participants interact with the model card, initial defaults should be deliberately set to showcase the model's varied performance. Participants suggested including at risk groups as an example, but this can also include showing areas where the model performs poorly. We use productive skepticism to emphasize that stakeholders should be promoted to question the model in a way that showcases both its strengths and limitations.


%``overview first, details on demand''~\cite{shneiderman1996eyes} 

==> Interactive Model Cards/tex/study_one_v0.tex <==
\section{Study 1 : Concept Study with ML, AI, and NLP Experts}
In the first phase of our exploration, we drew on perspectives from participants with relevant expertise--ML/AI development and design; AI ethics; and Natural Language Processing (NLP)--to deepen our understanding of the strengths and limitations afforded by different modalities for documenting and explaining model behavior. \hl{PLACEHOLDER - more explanation about why we chose to do a study with experts (and different sorts of expertise) when we say we want to prioritize non-experts needs.}

We conducted a concept study with ten of these experts, asking them to engage with three different forms of model documentation: standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, robustness gym reports (RGRs)~\cite{goel2021robustness}, and a concept we propose for an interactive model card (IMC).
Our findings from this study informed the development of a functional prototype for an interactive model card that we assessed in a second study (Section~\ref{sec:study2}).
% In this initial study we presented participants with different modalities for documenting and reporting on machine learning models. Two modalities, the standard model card (SMC) and  a robustness gym report (RGR), have been previous described in the literature. In addition to these, we propose a concept for an interactive model card (IMC). To understand the strengths and limitations of SMC, RGR, and IMC, we conducted a concept study  with ten experts in ML/AI development and design, AI ethics, and Natural Language Processing (NLP). Their responses inform the development of a functional prototype for an interactive model card that we assess in a second study.

\subsection{Paper Prototype of Interactive Model Card Concept}\label{sec:studyone_probes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONCEPT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% >>>>>>> SOME STUFF HERE COULD GO IN THE INTRO <<<<<<
\noindent\textbf{Ideation.} Our concept for an interactive model card is informed both by our intuition 
as practitioners and researchers in ML, HCI, and NLP, as well as by
% as ML and NLP practitioners and researchers in addition to 
existing examples in the academic literature and beyond(~\hl{REF TO RW}). Furthermore, we focused our conceptual ideation toward a data professional who has expertise in applying machine learning technology, but might not be able to code or directly develop ML models. We 
% consider, and question, 
examine
how adding interactivity to models cards could better serve these sorts of users as they try to understand and evaluate models they might use, for example, through a low- or no-code data analysis environment. 
% There are many different areas to focus designing an interactive model card, with our data work persona in mind and we chose two to begin with two areas. 
While there are many design components that could shape interpretability and usefulness of IMCs, with this data professional in mind we chose to focus our initial analysis on two areas. 
The first was disaggregating performance metrics with custom subpopulations in the model's training and testing data. We see opportunities to use interaction to allow others to define subpopulations that are pertinent to them. The second area of focus was a set of  visualizations that enable people to compare data pertinent to them against the model's training and testing data. 
% Existing ideas for interactivity in model cards give people some ability to test usually just a single example and assess the model's performance. We sought to take this idea further by using interactive data visualization to compare a person's dataset against the model's.
Some existing model cards include interactions that enable users to test how the model will behave on input data they enter (usually a single example at a time, manually entered)(~\hl{REF TO HF? other examples?}).
We sought to take this concept further through an interactive data visualization that allows users to compare their own datasets against the model's training and testing data.

\vspace{1mm}
\begin{wrapfigure}{l}{0.6\textwidth}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/Phase_I_concept_probes.pdf}
    \caption{Paper Prototype Design Concept of an Interactive Model Card. Larger images of the standard model card, robustness gym report, and interactive model card are available in online materials \hl{\texttt{[OM\#]}}}
    \label{fig:phaseI_concepts}
\end{wrapfigure}
\noindent\textbf{Task, Model, and Data.} We chose a single sentiment analysis task for this study because we believed this approach would allow for a focused study and analysis. 
% This focus may also be viewed as a limitation of our study 
We also acknowledge this focus as a potential limitation of our study, 
and we will return to this discussion in Section~\ref{sec:discussion}. 
We target sentiment analysis because it is a relatively common task and as such the scenario would require little to no explanation for study participants. 
We constructed an SMC, RGR, and IMC based upon a DistilBERT model that was fine-tuned on the SST-2 dataset. We used a specific DistillBERT SST-2 fine-tuned checkpoint that is available on HuggingFace (\url{https://huggingface.co/})\footnote{\href{https://huggingface.co/distilbert-base-uncased-finetuned-sst-2-english}{distilbert-base-uncased-finetuned-sst-2-english} commit \texttt{03b4d19}; \href{https://huggingface.co/distilbert-base-uncased}{distilbert-base-uncased} commit \texttt{b22dbc4}; SST-2 dataset} because it had a rich existing model card that we could adapt and use in our study.

\vspace{1mm}
\noindent\textbf{Paper Prototype Design and Implementation of the Interactive Model Card.} Our concept for an interactive model card~(\autoref{fig:phaseI_concepts}) includes elements of the standard model card and robustness gym report (shown with orange borders). We proposed adding interactive elements (shown with green border) that would allow users to upload their own data (\texttt{data upload panel}), add their own sentences (\texttt{example generation panel}), and/or define new subpopulations from the model's training and test datasets for exploration (\texttt{example generation panel}). We also include an interactive data comparison visualization (\texttt{data comparison panel}) that shows sentence embeddings of uploaded data and singleton sentences or subpopulations of the train and test data. 

% In our design ideation we also considered what the base design of the IMC should be if an individual chooses not to interact. To that end, we also designed non-interactive components of the IMC with equal measures of deliberation. 
In our design ideation, we also sought to ensure that the IMC would be interpretable and useful whether or not an individual chooses to engage with the interactive components.
We arrived at a design with defaults for text and visual content that would be informative without requiring interactivity(~\autoref{fig:phaseI_concepts})
% . Our motivation was that the IMC should be informative 
while still supporting those individuals who want to dig deeper with interaction. The DistilBERT SST-2 model presented a unique challenge for our overall design process because it is a fine-tuned, distilled version of a larger pre-trained general language model. We had open questions of how much information to include (if any) about the DistilBERT and BERT models.%The IMC proposes an information design that provides a simplified high-level overview of a model card, with details available on demand via a modal window. 

We implemented paper prototypes for the SMC, RGR, and IMC using Google Slides. For the IMC we mocked up interactions through slide links, transitions, and animations. Text for these paper prototypes was taken verbatim, with some small exceptions, from the existing HuggingFace model card for DistilBERT and the SST-2 fine-tuned checkpoint.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% STUDY PROCEDURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Study Procedures}\label{study_one:general_procedures}
\input{tables/study_one_participants}
\subsubsection{Recruitment}
We set a target of 10 participants aiming to recruit at least one participant from on the following categories : ML/AI development and design,  Ethics, and NLP.  We reached out to 23 participants, recruiting until we had met our target study size. Of the 13 participants that were not included in our study, five declined to participate and the rest did not respond.  We recruited participants based upon their publication or professional history using a combination of personal connections and cold emails. While all participants had some awareness of model cards, only six reported having a familiarity with model cards and only two were familiar with robustness reports. 



%\subsubsection{Participant Demographics.} The distribution of participants across the recruitment categories were 2 (development and design), 5 (ethics), 1 (auditability), and 2 (NLP). Our study participants held a variety of roles across different academic, government, and industrial organizations. These roles included lead roles in AI ethics and user research efforts (n=3), ethics data scientist (n=1), an ethnographer (n=1), and researchers  (n=5) in NLP, Ethics, or Machine Learning.  The majority of participants reported identifying as female (n=7). 


\subsubsection{Study Sessions} 
% We conducted a semi-structured interviews. Ahead of the study, we prepared a study script and slide deck of conceptual design probes (Section~\ref{sec:studyone_probes}) that we used throughout the interviews. 
Our study comprised semi-structured interviews that incorporated conceptual design probes (Section~\ref{sec:studyone_probes}).
Study sessions were scheduled for 60 minutes, and participants were offered an honorarium of \$150 upon completion.
% Study sessions are available in online materials, 
Full study protocols and materials are available in the online materials, 
while here we provide only a brief overview. During the study, participants were asked about their background and familiarity with model cards, Robustness Gym reports, or other types of model documentation. They were then shown examples of a standard model card, a Robustness Gym report, and our concept for an interactive model card (Section~\ref{sec:studyone_probes}). They were asked to explore each of the forms in a think-aloud protocol, and the study administrator also prompted them with predefined questions from the protocol. 
% When providing their feedback, participants were asked to additionally consider whether the model cards would be suitable for an analyst persona, Jenn, who uses a language model for a sentiment analysis task, but who did not have a formal education in computer science, statistics, or machine learning, and cannot write code:
As they considered each of these forms of model documentation, we asked participants to reflect on the strengths and limitations through the lens of their own needs as experts and also with respect to the documentation needs for an analyst user in the following scenario:
% Each session included a primary administrator and one note taker. At the onset of the  session, participants were shown a consent detailing the goals, data collection processes, and the way the data would be used, and seeking permission to video record the session. People could participate in the study and decline to be recorded; in those instances (n=1) study observers still took detailed notes. Once consent was obtained we began to record the session and asked participants to describe the background, research, or work as it pertained of ML,AI, or DS and especially toward model transparency and ethics.
%Following this introductory phase the informants were asked to share their screen and was provided with a link to slide deck  of design probes. Informants were primed with a fictitious persona, Jenn, who uses a language model for a sentiment analysis task, but who did not have a formal education in computer science, statistics, or machine learning, and cannot write code~\hl{[OM\#]} : 
\begin{quote}
\footnotesize
\textit{Jenn is a marketing analyst with CloudyShoes Inc. She is running a campaign to \textbf{analyze the sentiment of social media posts} that feature CloudyShoes’ products. She is using a sentiment analysis model and wants to understand its performance across different customer segments. Jenn primarily uses a point-and-click user interface to do her analysis. \textbf{Though she has no formal training in machine learning or natural language modeling, she has a high-level understanding of natural language models} and has been using them for some time to help her work.}
\end{quote}  
%Participants were asked to review the standard, robustness, and conceptual model cards in this order and prompted to review and talk-out-loud of their perception on the model content and design. They were asked to consider these model cards from their own perspective as expert, if applicable with experience of these model cards work in practice, and also how they would perceive someone like Jenn interpreting this information. In the final phase of the study participants were given the opportunity to raise topics or concerns that they felt we had not covered. The study administrator followed the pre-defined script, but modified existing questions or added new ones as needed. 

\subsubsection{Data Collection and Analysis}\label{study_one:qual_coding}
%I Like how they wrote about it in this paper : https://arxiv.org/pdf/2004.11440.pdf
% We recorded approximately 11 hours and 15 minutes of video, which included an approximately 60-minute interview and an additional on-camera debrief between the study administrator and note taker. Data was collected in the form of observer notes and video recordings. The video transcripts were automatically generated, including speaker identification, and were verified for accuracy by the authors. The transcripts amounted to 84,849 total words (including on-camera debriefs) of which 38,321 words (43\%) were attributed solely to the informant. 
Data collection included observer notes and video recordings for participants who consented to recording. 
We recorded approximately 11 hours and 15 minutes of video, which included an approximately 60-minute interview and an additional on-camera debrief between the study administrator and note taker. 
Video transcripts were automatically generated, including speaker identification, and were verified for accuracy by the authors. 
We conducted iterative \textit{thematic analysis}~\cite{charmaz2014constructing}, surfacing initial codes through debriefs and review of transcripts. The \hl{nth} author then conducted focused coding for all transcripts, and the \hl{nth and nth} authors synthesized themes and categories. The \hl{nth and nth} authors also surfaced implications that informed the design of our \textit{interactive model card functional prototype} (Section~\ref{sec:functional-prototype}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}
The goal of our study was elicit and synthesize our informants' experiences, perspectives, and reactions to different modalities of documenting and reporting on machine learning models. Some aspects of standard models cards, for example, may be favorable to alternatives presented in the interactive model card, and vice versa. 
However, we did not have a definitive signal (nor did we set out to find one) that one modality (SMC, RGR, or IMC) is better than the other. 
% To that end, we conducted a thematic analysis  that results in 
Our analysis surfaced
five interconnected categories summarizing informant perspectives, an overview of which is available in~\autoref{tab:studyone_tab}. 
We discuss each of these categories in detail below, along with the implications they raise for designing interpretable and useful model documentation.
%that are summarized inalong with examples of informant statements. %Below, we provide a summary of these themes and their attendant subthemes.
\input{tables/study_one_quotes}

\subsubsection{People} Informants were prompted to consider how a fictitious data analyst, Jenn, would respond to the information presented in the SMC, RGR, and IMC.  
% Organically informants as described other stakeholders or students to whom they have presented model cards or concepts found within them (i.e. model performance). 
Unprompted, participants also described additional stakeholders or students and the scenarios in which they share model cards or other documentation (e.g., related to model performance and tuning).
One participant succinctly summarised that SMC remained relatively untested with individuals who do not have formal training in ML or NLP: 

\begin{quote}
\small
    \textit{``At least for the next couple of years, people are going to be using model cards for the first time. And these are going to be concepts that may be new for many individuals. And so giving them some some hand holding, as to what does this mean? What am I supposed to do with this, I think will be extremely helpful.''} [I01]
\end{quote}

One participant went further to suggest that if models card were inaccessible to a wider audience it would be \textit{``dangerous [..] when our customers are using the model''} [I02]. Several informants (n=\hl{X}) indicated that much of the language used across all model cards was academic or technical jargon that was largely inaccessible more broadly. Several participants (6) also
% felt 
articulated that
the language and layout of the SMC appeared better suited for software or machine learning engineers. One informant suggested that the SMC seemed \textit{``very like on the back end like it feels like GitHub'' }[I00], which they felt would not resonate with a more general audience that is using, but not implementing, models. Moreover, three informants reflected that some of these specialized terms of art in the model card are often inaccessible even to students of machine learning. One informant offered that their graduate and undergraduate students regularly used a `cheat sheet' reminding them of the ML and NLP terminology. 

When considering Jenn specifically, all informants expressed doubt that she would understand the model card information or know how to act on it. One participant anchored on Jenn's role, 
% suggesting that an interactive model card could be more adaptive to individuals with different roles; one simple way they suggested to do so is even to prioritize model card information differently for different roles. 
suggesting that an interactive model card could be more accessible to individuals across different roles, particularly if the design supported different information architectures or prioritization of information. 
In contrast, another informant [I06] was emphatic that standardization was a critical component of model cards and should be preserved. They went further to suggest that adding interactivity could be beyond the scope of a model card and should be considered something else altogether. Finally, 
% they advocated that if we were to pursue adding user input, via interactivity, to the model card, then we should ensure this visually distinct from the standard model card information.
they advocated that if we were to pursue supporting user input to the model card via interactivity, then we should ensure that interactive components are visually distinct from the standard model card information.
 
\subsubsection{Design Considerations} Informants critiqued the information design of all model cards; for the RGR and IMC, they also offered feedback on visual and interaction design. 
% Many of their comments on information design concerned issues of technical jargon, but participants also proposed ways to present this information more clearly. 
Most (\hl{n=X}) participants identified overly technical language and jargon as a key failing of all of the model cards, and they proposed alternative language to capture the same meaning in more accessible ways.
All informants said the amount of text in the standard model card made it difficult to quickly skim and understand the model. Participants appeared to prefer the ``overview first, details on demand''\footnote{Distilled from Ben Shneiderman's mantra ``Overview first, zoom and filter, then details-on-demand''~\cite{shneiderman1996eyes}.} 
view from the IMC, which we achieved through bullet point summaries with modal pop-ups for more details; one participant proposed a list expansion interaction over a modal pop-up. Most participants expressed that the visual design and layout of the IMC was \textit{``very clean''}[I08] and that their \textit{``eyes were able to focus on information that [they] missed before''}[I03] compared to the SMC and RGR. However, 
% this impression was dependent on informant as one felt 
a sense of focus/overwhelm varied among participants, and one participant articulated
that the IMC contained \textit{``too much information and is very cluttered''} [I04]. 
Informants also offered general comments on aesthetics and visual encodings, from the color of bars in the RGR, to the use of headers and other means to emphasize relevant information in both text and visualizations. 
% % Finally, informants were in agreement that they needed a high-level description, or as one participant stated, they  \textit{``would want a high-level understanding, with DistilBERT being a high-level representation''}[I06]. This informant went further to suggest that model cards could also link more effectively to other documentation artifacts, such as datasheets, while preserving high-level details in the model card.
% Lastly, participants agreed that a high-level description of the model's purpose was needed (i.e., ``DistilBERT is a sentiment analysis model''). One participant suggested that model cards could integrate more effectively with other documentation artifacts (e.g., datasheets), while preserving the simplicity and high-level descriptions in the model card[I06]. 

% Informants also offered general comments on aesthetics and visual encodings, from the color of bars in the RGR, to the use of headers and other means to emphasize relevant information in both text and visualizations. 
% Four informants proposed placing much greater emphasis on the sample size information that is displayed in the rightmost column of the RGR. One suggested that \textit{``flagging ones where performance is too low, given the sample sizes.''}[I02] would be valuable. 

One of the most significant areas of concern participants raised with respect to information design was a need for more high-level descriptions and summaries across all model cards and subsections within each card. participants agreed that a high-level description of the model's purpose was needed (i.e., ``DistilBERT is a sentiment analysis model''). One participant suggested that model cards could integrate more effectively with other documentation artifacts (e.g., datasheets), while preserving the simplicity and high-level descriptions in the model card[I06]. Most \hl{(n=X)?} participants also pointed out areas in the RGR and IMC where they thought different information should be prioritized or emphasized (e.g., changing the color of the size column (rightmost column) in the RGR or emphasizing it in another way). Lastly, many participants suggested adding or emphasizing higher-level metrics about performance (e.g., making overall performance visually distinct from disaggregated performance). 


In general, participants expressed concern that interaction may be difficult to discover -- this is something that has also been observed in the academic literature~\hl{REF}. However, they did believe that it would be helpful for someone like Jenn to add her own examples and visually explore the data and model performances. However, even though informants felt that the IMC made some design decisions (simplified descriptions, visualizations, and easily ability to add data) could lower barriers for people like Jenn, emphasized that she would still need clear guidance and contextualization.

Finally, two informants raised the concern that \textit{``the developer has to make these model cards, but they are difficult to make, which is why these are not very informative.'' } [I07] and that \textit{``there's too much work getting model cards up''}[I06]. Their perspective underscores the importance of supporting both model card authoring and understandability, which ultimately target multiple (sometimes overlapping) audiences. 


\subsubsection{Guidance} Informants felt that participants need help making sense of an act on the information in the model card. Six informants emphasized the importance of providing specific guidance to help participants understand the information on the model card. This guidance included simple actions like providing definitions, or visual cues in the form of nudges and warnings. One participant felt that explainers for visualizations would be helpful because \textit{``it's pretty but..but what would I do [with it?]''}[I02]. One informant saw the direct potential for using interaction to provide guidance, suggesting that \textit{``would help me [...] dig deeper''} [I00] into the model details.

Other forms of guidance were complex and geared more toward \textit{``help[ing] me understand why this matters [and] how does it help me make more informed decisions?''}[I01]. Supporting interpretability is complex but nearly all (n=7) informants indicated that examples could provide some useful guidance. However, having an effective default example to prompt end-users was also important because \textit{``defaults are complex in language, so what  do you start with?''} [I03]. Another informant suggested that leveraging examples with interactivity could help people like Jenn \textit{``build a better mental model of how the model works and, like, what it lacks.''}[I04].

\subsubsection{Trust and Safety} Ethics and safety considerations resulted in a lively discussion. On our source model card (Section~\ref{sec:studyone_probes}) the ethical considerations text was short, but many informants took exception with the training dataset being described as ``fairly neutral'' (\textit{``what does that mean even?''}[I07]).  One commented that `Silicon Valley' tended to apply a standard set of \textit{``moral values application across global and cultural contexts''}[I06], which diminishes that value of such ethical statements and assessments. Increasingly such statements are seen as a \textit{``cop-out because it just kind of says `there is some bias somewhere' which is not entirely helpful.''}[I05]. Two informants suggested stating explicitly whether bias assessments had been conducted, and one suggested raising a warning if such bias analyses are not run. Several participants also suggested pre-populating the RGR visualization with specific vulnerable populations, making them prominent, and pointed to risk taxonomies that defined such groups. However, one participant cautioned that at-risk or marginalized groups are different across the world, and the default inclusion of such populations is not always meaningful and needs to be customizable to regional contexts. 

\hl{PLACEHOLDER - other warnings, including sample size for performance}

 Four informants proposed placing much greater emphasis on the sample size information that is displayed in the rightmost column of the RGR. One suggested that \textit{``flagging ones where performance is too low, given the sample sizes.''}[I02] would be valuable. 
 

\subsubsection{Sensemaking and Skepticism} The ideas of the previous themes come together as informants discussed the ways they believed end users like Jenn would make sense of, and explore, information in the model cards. Informants tied interaction positively to these themes, indicating that it would be beneficial to \textit{``allow domain experts to be able to interrogate the models and formulate rules that are semantically meaningful to test against the model''{I07]}}. Importantly, the interactivity would enable people to \textit{``elicit more questions'' }[I03] that allowed them to form and test their mental models about the data and better \textit{``see the things that model lacks''}[I04].

\subsubsection{Summary and Implications}
\hl{PLACEHOLDER - Either in this section or in in the overview of the prototype design I think we need to say more about which of these pieces shaped the design and which we take as broader implications. (I have notes for this but haven't integrated them into the text yet)}


==> Interactive Model Cards/tex/study_two.tex <==
\vspace{-2mm}
\section{Study 2 : Evaluation with non-expert Analysts}\label{sec:study_two}
We used the design guidelines from the initial concept study to implement a functional prototype for an interactive model card (IMC) that we assessed with 20 non-expert analysts. %These individuals use machine learning models in the daily work and have exposure to ML model documentation, but not necessarily model cards. Study participants had no formal training in data science, machine learning, or NLP, and were primarily self taught in use of ML or NLP models. 
%This second study implements a functional prototype of an interactive model card that follows the feedback and design guidance synthesis from the prior study. We assessed this prototype with 20 participants who analyze data with machine learning models as part of their job. Moreover, we sought to recruit participants who are primarily self taught through on-the-job experience rather than having a formal post-secondary education in data science, machine learning, or NLP. We expected that these individuals would have some familiarity with ML models, but might not have the same depth of technical understanding as individuals with more structured education or training.% We also anticipated this group to have little to no exposure to model cards.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% FUNCTIONAL PROTOTYPE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{-3mm}
\subsection{Interactive Model Card Functional Prototype}\label{study_two:functional-prototype}
\begin{figure}
    \centering
    \includegraphics[width=0.97\textwidth]{figures/phaseII_imc_concept.pdf}
    \vspace{-3mm}
    \caption{IMC Functional prototype that we presented to participants in the second study. Overlain are some examples of how feedback from the first study influenced the prototype design. The code for this prototype is available in the online materials.}
    \Description{An image of of the functional prototype of the interactive model card. Two panels are shown. The larger panel shows the main view of the interactive model card, while the second smaller panel shows the data comparison. The emergent themes that influenced the model card design are overlain. Each theme is shown as a color coded rectangular box with an arrow indicating the specific element of the functional prototype that was influenced by that theme.}
    \label{fig:phaseII_imc_concept}
    \vspace{-5mm}
\end{figure}

The functional prototype of the IMC %is a software application that
reifies the design guidelines; in ~\autoref{fig:phaseII_imc_concept} we show %a screenshot of 
our IMC with themes from~\autoref{tab:studyone_tab} overlain to emphasize the sources of design guidance. %In~\autoref{fig:phaseII_imc_concept} we have summarized how the themes in~\autoref{tab:studyone_tab} influenced the design of our interaction model card functional prototype. A detailed walkthrough of the IMC prototype is available in~\hl{\texttt{OM\#}}, while here we summarize these elements relative to the design guidance Section~\ref{study_one:design_guide}.
We visually separated information between a model overview component--reference model card information--and the `contextual' component, where interactivity is used to probe the model's performance and underlying data.  Within these components, we introduced elements of information and visual design to present the content (\textbf{DG1}) and create avenues of interactive engagement (\textbf{DG2}). 
% Across both components, we use text font faces, color, and highlighting to emphasize important content like the model's task (i.e., sentiment analysis) and its range of outputs. 
Across both components, we use font faces, color, and highlighting to emphasize important content like the model's task (i.e., sentiment analysis) and its range of outputs. 
We also introduce two levels of information hierarchy. The first level summarizes vital information as a bulleted list; the second level
% contains 
provides
technical details that are only visible when the analyst expands the content. In the overview component we also reduced the jargon from the SMC text. %Some design elements are specific to each component. In the overview component, we attempted to  reduce the jargon from the reference model card text.  To the contextual component, we added interactive data visualizations that show the model's performance and enabled exploration of its data.

We use interaction to support concept building, sensemaking, and skepticism around the model and its performance (\textbf{DG2}). 
% We have developed
The interactive data visualizations 
% that 
show the model's performance and explore the model's data. The performance visualization shows the overall train and test data set performance according to accuracy, precision, and recall (the reference model card only shows accuracy). Using Robustness Gym~\cite{goel2021robustness} we developed a set of terms that 
% define 
relate to
subpopulations of US protected classes (e.g., race, gender, veteran status; \textbf{DG4}) that are also visualized
%These default subpopulations  are visualized in the data as well. 
We introduce three ways for analysts to further probe model performance: defining custom subpopulations within the model's data, adding their own sentences, and adding their own dataset. When an analyst chooses to add a sentence, they will see a summary of the model's sentiment prediction and have the option to contest the result; the `sentiment label' for the new sentence is based on the participant's choice.  We have also defined a set of default sentence templates of mixed sentiment~\cite{potts2020dynasent} and with sensitive attributes~\cite{czarnowska2021quantifying} to help analysts further explore examples that are distinct from the model's data. Finally, the data visualizations are updated in real-time to reflect the model's performance in these newly defined subpopulations or data (sentence or dataset).

We scaffold the information in the model card with guidance that supports the interpretation of 
% model card 
textual
information and visualizations~(\textbf{DG3}).  Examples of guidance include simple statements explaining how to interpret visualizations or interact with them, definitions of terms, and 
% ways to add new data. 
instructions for adding new data.
Lastly, we include a `Guidance' section that includes more general information about sentiment analysis models and the interpretation of performance metrics. We 
% also introduce 
incorporate
warnings to alert the analyst to potentially unreliable or incomplete information in the model card. The performance visualization also alerts analysts 
% to subpopulation sizes lower than a default threshold.
when a subpopulation's size is lower than a specified threshold.

%we introduce different elements of visual and interactive design to make content accessible and invite engagement (\textbf{DG1})
%We architected information to exist at two levels of hierarchy (\textbf{DG1}). The first level of hierarchy separates the objective and subjective model information in two adjacent panels. Within each panel, we introduce a second level of hierarchy that promotes important information, as established in the prior study, to a prominent and visible position on the card, while less important information is hidden but available via interaction. In both panels we use visual cues like text color or decoration or icons to guide the reader.

%The information architecture and design is scaffolded with guidance for interpreting and acting on the information. Guidance is provided throughout the model card  (\textbf{DG4}) via brief textual explanations of how to interpret certain types information (for example, in  chart), links of definitions, and finally a specific section for more general guidance on NLP models and model metrics. In this latter section, documents are sourced from existing guidelines and summaries available online. We have also introduced warnings \textit{about the model card content} to alert readers when information is absent of incomplete. In this study, we have experimented with alerts about the intended uses, ethics, and dataset quality, which are three areas that experts suggested were underreported in the reference model card, and others,  and that could consequently mislead stakeholders. To complement this guidance we have also revised the language through the model card to make it clear what the model is, what is does, and how it can be used (\textbf{DG21}).

%Finally, we use interaction to support concept building, sensemaking, and skepticism of the model and its performance (\textbf{DG3}). Some experts articulated a set of (contextually dependent) defaults that included protected or at-risk groups that we leveraged (\textbf{DG5}). We used the Robustness Gym technology~\cite{goel2021robustness} to automatically detect protected classes as they are defined by the US; note that we use this an initial prompt, and argue these could (and should) be developed and customized to different regional or organizational contexts. The model's performance in these protected classes is visualized along with its overall performance in the training and test data. Finally, to help participants test the model with novel sentences, but also of potentially ethical consequence, we developed a set of sentence templates of mixed sentiment~\cite{potts2020dynasent} and with sensitive attributes~\cite{czarnowska2021quantifying}. In addition to these defaults, the IMC enables stakeholders to define their own subpopulations within the model's training and test data, add their own sentences, and upload their own dataset. Model performance is updated in real time. Moreover, these custom examples are added to the data comparison panel as well via a pre-trained Doc2Vec model~\cite{le2014distributed}; this default view of the data comparison is pre-populated with a 2D representation of the model's training and testing data.

The IMC is implemented in Python %. The interface and interactions are implemented and hosted 
using \texttt{streamlit}\footnote{\url{www.streamlit.io}}, with visualizations and data interactions supported by \texttt{Altair}~\cite{vanderplas:altair:2018}. \texttt{Robustness Gym}~\cite{goel2021robustness} and \texttt{Gensim}~\cite{rehurek:gensim:2011} are primarily used to handle data inputs and outputs between the cards visual components, and are supported by other packages (\texttt{nltk}~\cite{bird:nltk:2009}, \texttt{numpy}~\cite{harris:numpy:2020}, \texttt{pandas}~\cite{mckinney:pandas:2010}, \texttt{sklearn}~\cite{scikit-learn}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% STUDY PROCEDURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Study Procedures}\label{sec:study2_procedures}

%\vspace{-2mm}
%\subsubsection{Recruitment}
%\begin{wrapfigure}{l}{0.5\textwidth}
%\begin{figure}[th!]
%    \centering
%    \includegraphics[width=0.5\textwidth]{figures/Phase_II_flow_diagram.pdf}
%    \caption{Flow diagram of participant selection.}
%    \vspace{-5mm}
%    \label{fig:phaseII_criteria}
%\end{figure}
%\end{wrapfigure}

\subsubsection{Study Design} We conducted a 60 minute semi-structured interview with each of the participants,
% . We asked participants to expand upon 
asking them to describe
their use of ML or NLP models as well as the type of model documentation they consume or, if applicable, produce. Participants were then introduced to the format of a model card and directed to the DistilBERT SST-2 fine-tuned reference model card (Section~\ref{sec:studyone_probes}). They were asked to explore this model card and think out loud about what information they would want to gather, whether it was available, and 
% if not 
how they would wish to see this information. Next, participants were given a demonstration of the interactive model card and were asked to explore it as they had the reference model card. In the final 15 minutes of the session, participants were asked to consider the IMC with respect to its usability, functionality, safety, and ethics. These question prompts were developed based on the findings of the previous study and a set of explainability characteristics
that we adapted from those
% that have been previously 
described by Sokol and Flach~\cite{sokol10.1145/3351095.3372870}.
% that we adapted to this study. 
We also asked participants to compare the IMC to the reference model card. At the conclusion of the study participants were compensated \$125.

\vspace{-1mm}
\subsubsection{Recruitment} We set a target of 20 participants and recruited using the \href{https://userinterviews.com}{User Interviews} platform. We screened eligible participants using a questionnaire and  \textit{a priori} inclusion and exclusion criteria. In total 176 participants responded. A total 117 participants were excluded, in some cases because they indicated never using ML or NLP models (n=89), while others (n=28) had graduate or undergraduate training in ML, statistics, or computer science. The remaining 59 candidates were separated into two groups according to the frequency with which they use code-based tools (i.e., Python, R, etc). Type I (n=35) analysts do not use programming tools at all or very infrequently (less than once a quarter), whereas Type II  (n=24) analysts report daily or weekly use.  
% Within these categories, we further ranked participants according to their responses and invited them to participate. 
We recruited an even number of participants from both categories of analysts (\autoref{tab:study_two_participants}), anticipating each group might offer a different perspective to our study.Participants were compensated \$125

%We recruited participants from \url{userinterviews.com}, an online user testing platform. We created a questionnaire \hl{SUPPLINK} and screened participants according to their responses (~\autoref{fig:phaseII_criteria}). A total of~\hl{128} people responded to our questionnaire through the platform. We categorized interested candidates according to two criteria: their formal education in computer science (CS), machine learning (ML), or statistics (stats) and the frequency that they use DS or ML tools in their daily work as well as their their use of tools of code-based (python, R, etc) tools. Participants were classified as analysts \hl{(n=49)} or data scientist \hl{(n=26)} based upon their responses, while about half \hl{(n=53)} were excluded because they did not meet the qualifying criteria (e.g., did not use ML in their work, did not respond to all questions in the screener, provided inconsistent responses, etc.). We also asked participants about their familiarity with text analysis, sentiment analysis, and their AutoML or NLP tool usage. We also populated our tooling list with fake tools and excluded individuals selecting those tools.

%We focused this study on analysts, which we further subclassified into Type I \hl{(n=29)} and II \hl{(n=20)} analysts according to their frequency of ML and DS tooling use.  Finally, we ranked participants according to the relevance of use cases they identified in their work, which they detailed in a free-text field in the questionnaire. Relevance was established according to extent to which they describe using DS and ML in a business use case, as opposed to, for example, a side project. We aimed to recruit a total of 20 participants, with ten from each category. The final set of participants is shown in~\autoref{tab:study_two_participants}; none of the participants in our study had been previously exposed to a model card but all had exposure to some form of machine learning model documentation. Type II analysts tended to produce their own model documentation, whereas Type I analysts tended to be consumers of such documentation.

\input{tables/study_two_participants}

%Qualifying participants were scheduled through \url{userinterviews.com} to participate in a 60-minute session. Participants were asked about their background, their job responsibilities, and the types of machine learning model documentation they consume or produce. Following this participants were introduced to model cards and then given an opportunity to interact with the reference model card for the DistilBERT SST-2 fine tune (Section~\ref{sec:studyone_probes}). Participants were left to organically explore the model card, but were prompted after a period of time to engage with the hosted API or view the more details DistilBERT model card if they had not done so; participants could, and did, indicate if they wished to act on the prompt or not. Finally, participants were introduced to the interactive model card. First, they were given an approximately ten-minute overview of the model card (\hl{OM LINK}) and asked to organically explore the IMC. After about 15 minutes of exploration, participants were asked to respond to a set of questions about the model's operational, functional, safety, and ethical characteristics {\hl{OM LINK}}. These characteristics are based on the explainability fact sheets~\cite{Skol:XAIFacts:2020}, with modifications for our study, to assess the extent that our prototype was understandable and actionable.  

\vspace{-1mm}
\subsubsection{Data Collection and Analysis}
%I Like how they wrote about it in this paper : https://arxiv.org/pdf/2004.11440.pdf
Data was collected and analyzed in the same manner as reported in Section~\ref{study_one:general_procedures}. In this study we recorded approximately 23 hours and 30 minutes of video, which included both the interview and an additional on-camera debrief between the study moderator and notetaker. We used the themes surfaced in the first study to seed this analysis.
% Data were analyze in the same manner as reported in Section~\ref{study_one:general_procedures}. 
% The transcripts from these sessions amounted to 235,216 total words (including on camera debriefs) of which \hl{106,968} words (~46\%) were attributed to solely to the informant. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Results}
The reference model card (Section~\ref{sec:studyone_probes}), here acting as the SMC, and the IMC each had features that were 
% favored
preferred 
by both types of analysts. However, overall the IMC was favored over the SMC, with participants echoing the concerns that were previously articulated by the experts in Section~\ref{sec:study_one}. A summary of participant responses is shown in~\autoref{tab:studytwo_eval}. Compared to the prior study, non-expert analysts provided greater depth towards the themes of \textit{stakeholders}; \textit{design considerations}; and \textit{sensemaking \& skepticism} in particular. This depth allowed us to expand on the subthemes from~\autoref{tab:studyone_tab} and 
% add breadth to our conceptual understanding 
broaden our conceptions
of how model cards 
% could 
might
be used. 
% Where experts could on speculate, 
% the non-expert analysts provided more detailed and compelling insights toward the \textit{understandability \& interpretability} of information between the SMC and IMC. 
In comparison to experts, non-expert analysts contrasted the \textit{understandability \& interpretability} of information between the SMC and IMC with more concrete details, leading to compelling insights around design implications.
% Separately, we also prompted participants with questions towards the IMC's usability, functionality, safety, and ethics. Their responses, summarized in~\autoref{tab:studytwo_prompts}, also add to the dimensions from the first study and add context to participants' overall impressions of the IMC in~\autoref{tab:studytwo_eval}. 
Additionally, participants' responses to our explicit prompts around usability, functionality, safety, and ethics (summarized in ~\autoref{tab:studytwo_prompts}) allowed us to expand upon dimensions surfaced in our first study. They also helped us contextualize participants' overall impressions of the IMC, summarized in~\autoref{tab:studytwo_eval}.
% Despite the (self-reported) proficiency differences between the analyst groups, we did not observe large differences in their responses.
We did not observe large differences in patterns of responses between the two analyst groups.
% We highlight the key findings by first presenting participants overall responses towards the SMC and IMC. Next, we focus on three findings that emerged from the study that emphasize the importance of human-centered design approaches for contextualizing the uses of model cards in organizational settings.
In Section~\ref{sec:study2-findings-overall}, we outline participants' overall impressions of the IMC. After that we focus on three themes that 
% emerged that emphasize 
highlight
the importance of human-centered design in making model cards useful and usable in organizational settings.

%%%% OVERALL 
\subsubsection{Evaluating our Design Choices}\label{sec:study2-findings-overall} 
\input{tables/study_two_eval_quotes}
Nearly all participants (n=18) %reflected on the sufficiency of information presented between the two model cards, and 
found the IMC easier to read and understand (with some caveats discussed below). One participant said that the IMC showed information that \textit{``allowed [them] to understand what this model actually is supposed to be used for'}' and \textit{``this is a lot better at level setting''} [A2-08]. 
% Participants explicitly referenced  the layout of information (n=13), the language (n=6), the ability to add examples (n=15), and the visual and interactive elements (n=16) as helping them to engage with the model and its data more effectively by providing a sense of information priority. 
Participants articulated that several components of the IMC helped them engage with the model and data more effectively 
% by providing a sense of information priority, including: 
by clarifying and prioritizing information, 
particularly:
layout of information (n=13); language (n=6); ability to add examples (n=15); and visual and interactive elements (n=16).
Three participants voiced the importance of being able to contest the model's results, and wanted to see this ability expanded beyond adding sentences (Section~\ref{study_two:functional-prototype}) to the model's training and testing data or uploading their own dataset. One participant stated that the ability to \textit{``agree [or] disagree is kind of a check and balance''}[A1-06]. Nearly all (n=16) participants also made suggestions for improvements to the IMC design. These included changes to elements of the interface that were confusing (n=5), the layout (n=6), and types of guidance (n=1) provided. 
A few participants (n=4) expressed that 
% they felt information overload from  text, visuals, and interaction options. 
text, visuals, and interaction options led to information overload.
Participants suggested that 
% access to the model's code and files, which were present on the SMC, would be valuable on the IMC as well.
integrating the model's code and files, present in the SMC, would be valuable for the IMC.

When asked, nearly all participants (n=15) indicated that the IMC was something they would use in their daily work, while some (n=2) indicated it was context-dependent.
% for certain stakeholders. 
% The same participants 
Participants
reported that the IMC, with or without interactivity, was preferable to the SMC because the information was easier to understand. Notably, the addition of guiding elements, suggested in the previous study~(\autoref{tab:studyone_tab}), were well received and did help participants understand and interpret the model card information. Many of these non-interactive elements, which include visual cues, warnings, and prompts, among others, can be used to augment SMCs without having to add interactivity. 
% However, interactivity was still a critical component 
However, participants indicated that interactivity added substantially to the SCM
because it allowed participants to \textit{``play with the data and see the results [in a way that] that feels super intuitive instead of explaining everything''} [A1-09]. %This participant went further to reflect that when understand the capabilities and limitations of a language model \textit{``it’s easier to show it than explain sometimes.''}. %In~\autoref{tab:studytwo_eval}  we summarize additional participant perspectives on both the SMC and IMC. In~\autoref{tab:studytwo_prompts} we summarized participant perspectives on the IMC with respect to its usability, functionality, safety, and ethics dimensions.

\input{tables/study_two_prompts}


%%% MODEL UNDERSTANDABILITY

\subsubsection{Model Understandability - Getting the Basics Right}
One of the most salient 
% consequences 
implications
of the IMC design was that it helped participants accurately understand what the model was and what it did. In this study, we were surprised to discover that, when using the SMC, it was hard for participants to articulate \textit{that the model performed sentiment analysis}. While experts had expressed that non-expert analysts would have some difficulties interpreting that information, this finding went beyond our expectations. Overall, 
% more than seven 
almost half of the
participants were not able to provide the correct interpretation of what the model did using the SMC alone. Among these participants, four thought it was a general text classification model, but could not anticipate its outputs (positive or negative sentiment classification), two thought that DistilBERT and its fine-tuned version were both sentiment analysis models, one participant did not answer (\textit{``I would have a tough time understanding what it does.''}[A2-08]), one thought that SST-2 dataset was the model but could not articulate what the model did. Even three participants who did correctly describe the model were not confident in their interpretation : \textit{``I would guess that it's sentiment analysis based on text, but I really don’t know''}[A1-03]. 

% One source of confusion was how participants consumed the information between the DistilBERT base model and SST-2 fine-tune. 
One source of confusion was the need to consume information across two model cards (DistilBERT base model and SST-2 fine-tuned).
Guided by our earlier study, we tackled this challenge directly and used the design elements of the IMC to draw attention to what the fine-tuned model did and how it differed from the base model. The response of participants validated this 
% considered 
approach, with one stating that \textit{``the side panel was exactly what I was looking for and it highlighted some of the words, then I know that this is something that I might be interested in looking at'' }[A2-06].

%This had not come up at all in the expert studies nor in our own discussions. However, when asked during the session to explain in their own words what the model did, more than half (n=13) of the participants reported an incorrect interpretation. In total, X said they could not answer the question, while X thought the model was a text classifier but could not articulate that it classified text in positive and negative sentiment. Using the hosted API, which allowed participants to view or add examples,  sometimes help them to deduce that the SMC referred to a sentiment analysis model. Even when participants correctly stated that the model card referred to a sentiment analysis model, they were not confident in their responses.  One participant summarized this issue succinctly, stating that \textit{``the other one [SMC], I like basically didn't even get to it's a sentiment [...] I just kind of was like, let's imagine it's a sentiment analyzer [then I realized]  Oh - it is!''}[A2-07]. While time with the SMC could be a factor in driving this result, participant responses also suggest that design was important.

%One source of confusion is that the SMC for the finetune model is very brief, and points participants to the DistilBERT model card for additional details. This action was disruptive and disorienting to participants and they could not context switch between the two types of models --- a problem that is likely to generalize to other types of pre-trained models. In contrast, when designing information for the IMC, the fact that the model was a sentiment analysis model was featured clearly and visually emphasized, something that participants (n=X) commented on. One participant stated that \textit{``the side panel exactly what I was looking for and it highlighted some of the words, then I know that this is something that I might be interested in looking at, and I think this format is much more useful if I am looking for data.'' }[A2-06].

%%% ARTIFACTS
\vspace{-2mm}
\subsubsection{The Role of Model Cards in Sociotechnical Systems} 
%Non-expert analysts emphasized the importance that a model card is \textit{shareable} with stakeholders across their organization . 
Nearly all (n=18) participants described, without being prompted, how the IMC would help them share information with internal and external stakeholders. The actionability of a model card was frequently (n=13) tied by participants to its ability to be shareable and understandable to others with whom they work.
%, whether that be teams of data scientists with whom they collaborate or external stakeholders.
Moreover, participants discussed 
% the interdependence of social and technological 
interwoven social and technical
processes and described where either an IMC or SMC would fit within them. 
% \textbf{\textit{Participants begin with the model details}} (overview component in the IMC, Section~\ref{study_two:functional-prototype}) \textbf{\textit{to assess if the model is valid for their use case.}} A quick answer is essential according to one participant who stated \textit{`` I would lose [their] patience after 30-40 seconds [if they' have to put a lot of effort into what I am looking for''}[A1-06]. \textbf{\textit{If the participants were convinced the model was suitable for their use case, they move on to the interactive components to explore it further.}} One benefit of this interactivity was that it allowed participants to conduct lightweight experimentation, which was cumbersome using the SMC because \textit{``you [had to] deploy the model in Python yourself, put in your own sentences''} whereas with the IMC \textit{``just being able to do it, like this is, like, ease of use is off the charts''} [A2-02]. \textbf{\textit{Finally, the model card was used to start a dialogue with other stakeholders.}} These stakeholders included executive or technical team members, including data scientists.
Participants described how the model details (overview component in the IMC, Section~\ref{study_two:functional-prototype}) could help them with an initial assessment of the model's validity for their use case. A quick answer is essential, and one participant stated,  
% \textit{`` I would lose [their] patience after 30-40 seconds [if they' have to put a lot of effort into what I am looking for''}[A1-06]. 
\textit{``I would lose patience after 30-40 seconds if I have to put a lot of effort into what I'm looking for''}[A2-06].
If the participants were convinced the model was suitable for their use case, they would move on to the interactive components to explore it further. One benefit of this interactivity was that it allowed participants to conduct lightweight experimentation, which was cumbersome using the SMC because \textit{``you [had to] deploy the model in Python yourself, put in your own sentences''} whereas with the IMC \textit{``just being able to do it like this...ease of use is off the charts''} [A2-02]. Finally, the model card would be used to start a dialogue with other stakeholders. These stakeholders included executive or technical team members, including data scientists.

%What this finding shows is that the social and technological  processes are interrelated and ordered.
%Moreover, echoing the observation of E08 from the first study, participants in this study emphasized that making model documentation was a time-consuming process.The majority (n=11) participant independent pointed out the value of the IMC as tool for communication about AI models in their business, either by directly sharing the IMC or leveraging the information in other formats (~\autoref{tab:studytwo_prompts}). 
Beyond integrating model cards with their social organization, analysts (n=7; the majority belonging to group II) saw the benefits of incorporating model cards into their existing technical infrastructure: \textit{``A huge win would be getting this to integrate seamlessly with open-source frameworks'' }[A2-01]. Here, the reference model card contained information and actions to obtain the model code and launch it --- something that was absent in the IMC. Moreover, three participants expressed that IMCs, if they could be easy to produce, would lower their existing model documentation burden.
%Several (n=X) participants explicitly describing using the model card as a way to decide, for themselves or together with stakeholders, whether a model is worth pursing. Viewing desegregated model performance, and being able to modify it with their own examples and data, was deemed important by participants arriving at the decision. Participants expressed a processes where they use the model card and to rule out models that were irrelevant to their use cases. Next they would use examples to further refine a candidate set of models. Only once they had arrived at a viable set would they want to dive into the model code and run it for themselves. One limitation a participant observed with the SMC card was that such lightweight experimentation was still too cumbersome because \textit{``you [had to] deploy the model in Python yourself, put in your own sentences''} whereas with the IMC \textit{``just being able to do it, like this is, like, ease of use is off the charts''} [A2-02].

%%% ETHICS AND SAFETY
\vspace{-2mm}
\subsubsection{Ethics and Safety are Challenging Topics} 
Participants had difficulty contextualizing the safety and ethical dimensions of either the SMC or IMC. 
% Despite the IMC including templates of ethical sentence examples (Section~\ref{study_two:functional-prototype}), 
Although the IMC included templates to examine ethically challenging examples (Section~\ref{study_two:functional-prototype}),
only four participants expressed that these features could stimulate discussion. The unintended uses of the model were similarly inaccessible, with one participant stating that \textit{``unintended uses are important [but] how would I know what [is] unintended?'' }[A1-01]. 
%Participants had difficulty articulating whether and how either the SMC or IMC could help them reason about safety and ethics. Some participants (n=4) said the inclusion of the protected classes, or some equivalent for their cultural context, raised awareness of these issues. Two others expressed that warnings did so as well. However, the general sentiment expressed by participants was that it was an individual responsibility and more closely tied to the data rather than the model itself.
One participant expressed doubt that any model documentation could really give an adequate picture of ethical and safety risks, emphasizing that `\textit{`this [model card] would not be my only data point or else, you know, that's a very quick way to lose your job''} [A1-04]. Although the goal of model cards is not to be a substitute for further analysis of ethical and safety risks, this participant's comment echoes earlier observations from experts (Section~\ref{study_one:trust_safety}) that information about ethical risks is often dismissed. Others felt that topics of safety and ethics were too abstract, with one participant stating that they \textit{``wouldn’t worry too much about that to be honest, I guess it depends on the type of analysis you're doing.''} [A2-05]. 
% So [if] I am working with sensitive data, it doesn’t have anything to do with ethical things.''} [A2-05]. 
While the IMC also provided template sentences to promote ethical thinking, participants largely favored their own examples.  Unexpectedly, two participants pushed back against the inclusion of more actionable ethical and safety content, articulating concerns that too much guidance could be detrimental and provide a false sense of security.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% SUMMARY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-3mm}
\subsection{Summary}
We assessed our functional prototype for an interactive model card with twenty non-expert analysts drawn from across industry. Their feedback validates many of our design choices, but also offers avenues for further improvements. These non-expert analysts also illuminated a more detailed view of how model cards, more generally, might be used within the sociotechnical systems in their organizational contexts. Our findings point to 
% the importance of information and visual design as critical to the understanding and interpretability of model cards.
the importance of information and visual design for transparency and interpretability of model cards.

%\textbf{Taken together, we found that design, and not just the textual content, is critical for convey an accurate interpretation of NLP models to a wider group of stakeholders.}
%The goal of our study was elicit and synthesize our participants experiences, perspectives, and reactions to different modalities of documenting and reporting on machine learning models. Some aspects of standard models cards, for example, may be favorable to alternatives presented in the interactive model card, and vice versa. Overall, we found that applying the design guidelines from the first study (Section~\ref{study_one:design_guide}) created a  model card that, even without any interaction, was more accessible to people who use ML/AI models but do not have formal training. We also found that targeted choices of for interaction helped participants examine and explore their assumptions about the model. Importantly, they believed the IMC was a shareable artifact could help their stakeholder's do the same. However, these two elements of design and interaction were not separable. 





==> tables/study_two_eval_quotes_tmp.tex <==
{\renewcommand{\arraystretch}{1.30}%
\begin{table*}[t!]
\caption{Study TWO themes.}
\label{tab:studytwo_eval}
\scriptsize
\centering
\begin{tabular}{p{8em}p{12em}p{3.5em}p{41.5em}}
\toprule
%\textbf{Theme} & \textbf{Subtheme} &\textbf{Context}
\textbf{Theme}     & \textbf{Subthemes} & \multicolumn{2}{l}{\textbf{Example from interviews}} \\
& & Context & Quote \\ \midrule
tooling & & IMC, SMC & So, interactivity is the main one. This is more of an all or one, whereas SMC makes me use another tool. So I feel like [SMC] is more like a shopping mall, where I need build it on my own at home. [A1-03]\\
stakeholder & & SMC & It seemed more oriented towards somebody who wants to, like develop and train it and deploy it [...] this [IMC] does give me the same information, like it gives me the same context [...] but it's also giving me the tools to kind of look at the model on a higher level. [A2-04] \\
& & IMC & [If] I can integrate [the IMC] with my current readme files, or the DevOps infrastructure, I would take that. [A2-09]\\
structure & & & \textit{``It’s much better, before I was confused I didn’t know what was going on. At least now there is a structure.''} [A2-05]\\
& & IMC & ``Overall it’s easier to find things here, everything is one page which is nice, you don’t have to to go the website to find it.'' [A2-10] \\ & & SMC & ``I would loose my patience after 30-40 seconds, I have to put a lot of effort into what I am looking for, I would have to search somewhere else. [A2-06]\\
& & IMC, SMC & `` So for the hugging face model card, I would want to see more about how it can be manipulated. For the Interactive model card, I feel like it needs to drill into it more.'' [A1-07]\\

&& IMC &``Overall I am really impressed with the language clarity that is there right now, compared to what it was earlier. If I just have to inform what the biggest difference is, its clarity.'' [A2-09]\\

&& IMC & The first thing I am looking for is an introduction to the model and what it does and what it is used for. I don’t know if I see it here [A2-10]\\
&& SMC & \textit{`` this is very technically focused, and very focused on the model and not why does this model exist''} [A1-03]\\

&& SMC &  ``I know what I am looking for, but I couldn’t show this to management [... ]we would always add something ontop [A1-06]\\
&& SMC & `\textit{`the most important bit is what the purpose of the model is, and it’s good at the top, otherwise I didn’t know what what I was looking at, I had to guess how it actually works and what is trying to tell me''} [A2-05]\\
%&& IMC & \textit{``A huge win would be getting this to integrate seamlessly with open-source frameworks'' }[A2-01] \\
&& SMC& \textit{``It would be more like playing a game but would be interested to gauge how this works''}[A1-01]\\
& & IMC &  I absolutely like this quantitative analysis and are short, which let me play around, and I can see whether the model is working or not. So I'm not just taking the the word of the developer of the library [A2-09] \\
&& IMC & ``I want to be able to actually get the model somehow, so make it clearer that you can download or use the model''[A2-01] \\
&& IMC & \textit{``I think the other one [SMC] the code listed. I don't think this [IMC] has the code, anywhere. But that's probably another  strength slash weakness''} [A1-04]\\

% Data
%% 
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table*}
}





==> tex/background.tex <==
% \section{Making the Case for Interactive Model Cards}
\section{Motivation}
\hl{I think we actually address these with sufficient depth in the intro and related work and it would be hard to extract what is intro vs. motivation/background in particular. Keeping this as a placeholder for now.}

These are the questions that this section should aim to answer:

\begin{itemize}
    \item What are the limitations of existing model cards
    \item Why do we need interaction in model cards?
    \item Is this just a dashboard?
    \item Who are these for? 
\end{itemize}


This paper also supports our motivation fairly clearly: Explainable machine learning in deployment~\cite{bhatt10.1145/3351095.3375624}

==> tex/ideation.tex <==
\section{Interactive Model Card Concept Formation and Ideation}

The goal of our work was to apply a human-centred design approach to interrogate the value of adding interactivity to model cards for model reporting. Model cards are a proposed structure for creating documentation on a machine learning or ML/AI model. As they were initially proposed, model cards are static, but this does not exclude the possibility of including interactivity. Model cards developed by  HuggingFace (\url{https://huggingface.co/} )and also Google Cloud Model Cards (\url{https://modelcards.withgoogle.com/}), for example, including interaction modalities for people to add their own data when evaluating model performance. Complementary to model cards, but not conforming strictly to their structure, are highly bespoke interactive `explorables', for example, those created by PAIR(\url{https://pair.withgoogle.com/explorables/}), distill (\url{https://distill.pub/}), or other narrative forms of visual and interactive model explanation. These two extremes between fully static and highly interactive, but bespoke, model documentation was the spectrum we considered for exploring the potential of interactive model cards. 

\textbf{The question of what to make interactive in a model card and how to do so is what we primarily investigate in our research.} We hypothesized that two primary areas of a model card that would benefit from interaction : the model training and evaluation data and the quantitative analysis portions.

\hl{<finish this this>}



%As model cards are primarily static in their proposed implementation we analyzed several existing model cards to propose areas where interactivity could be added

==> tex/study_one_v0.tex <==
\section{Study 1 : Concept Study with ML, AI, and NLP Experts}
In the first phase of our exploration, we drew on perspectives from participants with relevant expertise--ML/AI development and design; AI ethics; and Natural Language Processing (NLP)--to deepen our understanding of the strengths and limitations afforded by different modalities for documenting and explaining model behavior. \hl{PLACEHOLDER - more explanation about why we chose to do a study with experts (and different sorts of expertise) when we say we want to prioritize non-experts needs.}

We conducted a concept study with ten of these experts, asking them to engage with three different forms of model documentation: standard model cards (SMCs)~\cite{mitchell10.1145/3287560.3287596}, robustness gym reports (RGRs)~\cite{goel2021robustness}, and a concept we propose for an interactive model card (IMC).
Our findings from this study informed the development of a functional prototype for an interactive model card that we assessed in a second study (Section~\ref{sec:study2}).
% In this initial study we presented participants with different modalities for documenting and reporting on machine learning models. Two modalities, the standard model card (SMC) and  a robustness gym report (RGR), have been previous described in the literature. In addition to these, we propose a concept for an interactive model card (IMC). To understand the strengths and limitations of SMC, RGR, and IMC, we conducted a concept study  with ten experts in ML/AI development and design, AI ethics, and Natural Language Processing (NLP). Their responses inform the development of a functional prototype for an interactive model card that we assess in a second study.

\subsection{Paper Prototype of Interactive Model Card Concept}\label{sec:studyone_probes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% CONCEPT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% >>>>>>> SOME STUFF HERE COULD GO IN THE INTRO <<<<<<
\noindent\textbf{Ideation.} Our concept for an interactive model card is informed both by our intuition 
as practitioners and researchers in ML, HCI, and NLP, as well as by
% as ML and NLP practitioners and researchers in addition to 
existing examples in the academic literature and beyond(~\hl{REF TO RW}). Furthermore, we focused our conceptual ideation toward a data professional who has expertise in applying machine learning technology, but might not be able to code or directly develop ML models. We 
% consider, and question, 
examine
how adding interactivity to models cards could better serve these sorts of users as they try to understand and evaluate models they might use, for example, through a low- or no-code data analysis environment. 
% There are many different areas to focus designing an interactive model card, with our data work persona in mind and we chose two to begin with two areas. 
While there are many design components that could shape interpretability and usefulness of IMCs, with this data professional in mind we chose to focus our initial analysis on two areas. 
The first was disaggregating performance metrics with custom subpopulations in the model's training and testing data. We see opportunities to use interaction to allow others to define subpopulations that are pertinent to them. The second area of focus was a set of  visualizations that enable people to compare data pertinent to them against the model's training and testing data. 
% Existing ideas for interactivity in model cards give people some ability to test usually just a single example and assess the model's performance. We sought to take this idea further by using interactive data visualization to compare a person's dataset against the model's.
Some existing model cards include interactions that enable users to test how the model will behave on input data they enter (usually a single example at a time, manually entered)(~\hl{REF TO HF? other examples?}).
We sought to take this concept further through an interactive data visualization that allows users to compare their own datasets against the model's training and testing data.

\vspace{1mm}
\begin{wrapfigure}{l}{0.6\textwidth}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/Phase_I_concept_probes.pdf}
    \caption{Paper Prototype Design Concept of an Interactive Model Card. Larger images of the standard model card, robustness gym report, and interactive model card are available in online materials \hl{\texttt{[OM\#]}}}
    \label{fig:phaseI_concepts}
\end{wrapfigure}
\noindent\textbf{Task, Model, and Data.} We chose a single sentiment analysis task for this study because we believed this approach would allow for a focused study and analysis. 
% This focus may also be viewed as a limitation of our study 
We also acknowledge this focus as a potential limitation of our study, 
and we will return to this discussion in Section~\ref{sec:discussion}. 
We target sentiment analysis because it is a relatively common task and as such the scenario would require little to no explanation for study participants. 
We constructed an SMC, RGR, and IMC based upon a DistilBERT model that was fine-tuned on the SST-2 dataset. We used a specific DistillBERT SST-2 fine-tuned checkpoint that is available on HuggingFace (\url{https://huggingface.co/})\footnote{\href{https://huggingface.co/distilbert-base-uncased-finetuned-sst-2-english}{distilbert-base-uncased-finetuned-sst-2-english} commit \texttt{03b4d19}; \href{https://huggingface.co/distilbert-base-uncased}{distilbert-base-uncased} commit \texttt{b22dbc4}; SST-2 dataset} because it had a rich existing model card that we could adapt and use in our study.

\vspace{1mm}
\noindent\textbf{Paper Prototype Design and Implementation of the Interactive Model Card.} Our concept for an interactive model card~(\autoref{fig:phaseI_concepts}) includes elements of the standard model card and robustness gym report (shown with orange borders). We proposed adding interactive elements (shown with green border) that would allow users to upload their own data (\texttt{data upload panel}), add their own sentences (\texttt{example generation panel}), and/or define new subpopulations from the model's training and test datasets for exploration (\texttt{example generation panel}). We also include an interactive data comparison visualization (\texttt{data comparison panel}) that shows sentence embeddings of uploaded data and singleton sentences or subpopulations of the train and test data. 

% In our design ideation we also considered what the base design of the IMC should be if an individual chooses not to interact. To that end, we also designed non-interactive components of the IMC with equal measures of deliberation. 
In our design ideation, we also sought to ensure that the IMC would be interpretable and useful whether or not an individual chooses to engage with the interactive components.
We arrived at a design with defaults for text and visual content that would be informative without requiring interactivity(~\autoref{fig:phaseI_concepts})
% . Our motivation was that the IMC should be informative 
while still supporting those individuals who want to dig deeper with interaction. The DistilBERT SST-2 model presented a unique challenge for our overall design process because it is a fine-tuned, distilled version of a larger pre-trained general language model. We had open questions of how much information to include (if any) about the DistilBERT and BERT models.%The IMC proposes an information design that provides a simplified high-level overview of a model card, with details available on demand via a modal window. 

We implemented paper prototypes for the SMC, RGR, and IMC using Google Slides. For the IMC we mocked up interactions through slide links, transitions, and animations. Text for these paper prototypes was taken verbatim, with some small exceptions, from the existing HuggingFace model card for DistilBERT and the SST-2 fine-tuned checkpoint.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% STUDY PROCEDURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Study Procedures}\label{study_one:general_procedures}
\input{tables/study_one_participants}
\subsubsection{Recruitment}
We set a target of 10 participants aiming to recruit at least one participant from on the following categories : ML/AI development and design,  Ethics, and NLP.  We reached out to 23 participants, recruiting until we had met our target study size. Of the 13 participants that were not included in our study, five declined to participate and the rest did not respond.  We recruited participants based upon their publication or professional history using a combination of personal connections and cold emails. While all participants had some awareness of model cards, only six reported having a familiarity with model cards and only two were familiar with robustness reports. 



%\subsubsection{Participant Demographics.} The distribution of participants across the recruitment categories were 2 (development and design), 5 (ethics), 1 (auditability), and 2 (NLP). Our study participants held a variety of roles across different academic, government, and industrial organizations. These roles included lead roles in AI ethics and user research efforts (n=3), ethics data scientist (n=1), an ethnographer (n=1), and researchers  (n=5) in NLP, Ethics, or Machine Learning.  The majority of participants reported identifying as female (n=7). 


\subsubsection{Study Sessions} 
% We conducted a semi-structured interviews. Ahead of the study, we prepared a study script and slide deck of conceptual design probes (Section~\ref{sec:studyone_probes}) that we used throughout the interviews. 
Our study comprised semi-structured interviews that incorporated conceptual design probes (Section~\ref{sec:studyone_probes}).
Study sessions were scheduled for 60 minutes, and participants were offered an honorarium of \$150 upon completion.
% Study sessions are available in online materials, 
Full study protocols and materials are available in the online materials, 
while here we provide only a brief overview. During the study, participants were asked about their background and familiarity with model cards, Robustness Gym reports, or other types of model documentation. They were then shown examples of a standard model card, a Robustness Gym report, and our concept for an interactive model card (Section~\ref{sec:studyone_probes}). They were asked to explore each of the forms in a think-aloud protocol, and the study administrator also prompted them with predefined questions from the protocol. 
% When providing their feedback, participants were asked to additionally consider whether the model cards would be suitable for an analyst persona, Jenn, who uses a language model for a sentiment analysis task, but who did not have a formal education in computer science, statistics, or machine learning, and cannot write code:
As they considered each of these forms of model documentation, we asked participants to reflect on the strengths and limitations through the lens of their own needs as experts and also with respect to the documentation needs for an analyst user in the following scenario:
% Each session included a primary administrator and one note taker. At the onset of the  session, participants were shown a consent detailing the goals, data collection processes, and the way the data would be used, and seeking permission to video record the session. People could participate in the study and decline to be recorded; in those instances (n=1) study observers still took detailed notes. Once consent was obtained we began to record the session and asked participants to describe the background, research, or work as it pertained of ML,AI, or DS and especially toward model transparency and ethics.
%Following this introductory phase the informants were asked to share their screen and was provided with a link to slide deck  of design probes. Informants were primed with a fictitious persona, Jenn, who uses a language model for a sentiment analysis task, but who did not have a formal education in computer science, statistics, or machine learning, and cannot write code~\hl{[OM\#]} : 
\begin{quote}
\footnotesize
\textit{Jenn is a marketing analyst with CloudyShoes Inc. She is running a campaign to \textbf{analyze the sentiment of social media posts} that feature CloudyShoes’ products. She is using a sentiment analysis model and wants to understand its performance across different customer segments. Jenn primarily uses a point-and-click user interface to do her analysis. \textbf{Though she has no formal training in machine learning or natural language modeling, she has a high-level understanding of natural language models} and has been using them for some time to help her work.}
\end{quote}  
%Participants were asked to review the standard, robustness, and conceptual model cards in this order and prompted to review and talk-out-loud of their perception on the model content and design. They were asked to consider these model cards from their own perspective as expert, if applicable with experience of these model cards work in practice, and also how they would perceive someone like Jenn interpreting this information. In the final phase of the study participants were given the opportunity to raise topics or concerns that they felt we had not covered. The study administrator followed the pre-defined script, but modified existing questions or added new ones as needed. 

\subsubsection{Data Collection and Analysis}\label{study_one:qual_coding}
%I Like how they wrote about it in this paper : https://arxiv.org/pdf/2004.11440.pdf
% We recorded approximately 11 hours and 15 minutes of video, which included an approximately 60-minute interview and an additional on-camera debrief between the study administrator and note taker. Data was collected in the form of observer notes and video recordings. The video transcripts were automatically generated, including speaker identification, and were verified for accuracy by the authors. The transcripts amounted to 84,849 total words (including on-camera debriefs) of which 38,321 words (43\%) were attributed solely to the informant. 
Data collection included observer notes and video recordings for participants who consented to recording. 
We recorded approximately 11 hours and 15 minutes of video, which included an approximately 60-minute interview and an additional on-camera debrief between the study administrator and note taker. 
Video transcripts were automatically generated, including speaker identification, and were verified for accuracy by the authors. 
We conducted iterative \textit{thematic analysis}~\cite{charmaz2014constructing}, surfacing initial codes through debriefs and review of transcripts. The \hl{nth} author then conducted focused coding for all transcripts, and the \hl{nth and nth} authors synthesized themes and categories. The \hl{nth and nth} authors also surfaced implications that informed the design of our \textit{interactive model card functional prototype} (Section~\ref{sec:functional-prototype}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}
The goal of our study was elicit and synthesize our informants' experiences, perspectives, and reactions to different modalities of documenting and reporting on machine learning models. Some aspects of standard models cards, for example, may be favorable to alternatives presented in the interactive model card, and vice versa. 
However, we did not have a definitive signal (nor did we set out to find one) that one modality (SMC, RGR, or IMC) is better than the other. 
% To that end, we conducted a thematic analysis  that results in 
Our analysis surfaced
five interconnected categories summarizing informant perspectives, an overview of which is available in~\autoref{tab:studyone_tab}. 
We discuss each of these categories in detail below, along with the implications they raise for designing interpretable and useful model documentation.
%that are summarized inalong with examples of informant statements. %Below, we provide a summary of these themes and their attendant subthemes.
\input{tables/study_one_quotes}

\subsubsection{People} Informants were prompted to consider how a fictitious data analyst, Jenn, would respond to the information presented in the SMC, RGR, and IMC.  
% Organically informants as described other stakeholders or students to whom they have presented model cards or concepts found within them (i.e. model performance). 
Unprompted, participants also described additional stakeholders or students and the scenarios in which they share model cards or other documentation (e.g., related to model performance and tuning).
One participant succinctly summarised that SMC remained relatively untested with individuals who do not have formal training in ML or NLP: 

\begin{quote}
\small
    \textit{``At least for the next couple of years, people are going to be using model cards for the first time. And these are going to be concepts that may be new for many individuals. And so giving them some some hand holding, as to what does this mean? What am I supposed to do with this, I think will be extremely helpful.''} [I01]
\end{quote}

One participant went further to suggest that if models card were inaccessible to a wider audience it would be \textit{``dangerous [..] when our customers are using the model''} [I02]. Several informants (n=\hl{X}) indicated that much of the language used across all model cards was academic or technical jargon that was largely inaccessible more broadly. Several participants (6) also
% felt 
articulated that
the language and layout of the SMC appeared better suited for software or machine learning engineers. One informant suggested that the SMC seemed \textit{``very like on the back end like it feels like GitHub'' }[I00], which they felt would not resonate with a more general audience that is using, but not implementing, models. Moreover, three informants reflected that some of these specialized terms of art in the model card are often inaccessible even to students of machine learning. One informant offered that their graduate and undergraduate students regularly used a `cheat sheet' reminding them of the ML and NLP terminology. 

When considering Jenn specifically, all informants expressed doubt that she would understand the model card information or know how to act on it. One participant anchored on Jenn's role, 
% suggesting that an interactive model card could be more adaptive to individuals with different roles; one simple way they suggested to do so is even to prioritize model card information differently for different roles. 
suggesting that an interactive model card could be more accessible to individuals across different roles, particularly if the design supported different information architectures or prioritization of information. 
In contrast, another informant [I06] was emphatic that standardization was a critical component of model cards and should be preserved. They went further to suggest that adding interactivity could be beyond the scope of a model card and should be considered something else altogether. Finally, 
% they advocated that if we were to pursue adding user input, via interactivity, to the model card, then we should ensure this visually distinct from the standard model card information.
they advocated that if we were to pursue supporting user input to the model card via interactivity, then we should ensure that interactive components are visually distinct from the standard model card information.
 
\subsubsection{Design Considerations} Informants critiqued the information design of all model cards; for the RGR and IMC, they also offered feedback on visual and interaction design. 
% Many of their comments on information design concerned issues of technical jargon, but participants also proposed ways to present this information more clearly. 
Most (\hl{n=X}) participants identified overly technical language and jargon as a key failing of all of the model cards, and they proposed alternative language to capture the same meaning in more accessible ways.
All informants said the amount of text in the standard model card made it difficult to quickly skim and understand the model. Participants appeared to prefer the ``overview first, details on demand''\footnote{Distilled from Ben Shneiderman's mantra ``Overview first, zoom and filter, then details-on-demand''~\cite{shneiderman1996eyes}.} 
view from the IMC, which we achieved through bullet point summaries with modal pop-ups for more details; one participant proposed a list expansion interaction over a modal pop-up. Most participants expressed that the visual design and layout of the IMC was \textit{``very clean''}[I08] and that their \textit{``eyes were able to focus on information that [they] missed before''}[I03] compared to the SMC and RGR. However, 
% this impression was dependent on informant as one felt 
a sense of focus/overwhelm varied among participants, and one participant articulated
that the IMC contained \textit{``too much information and is very cluttered''} [I04]. 
Informants also offered general comments on aesthetics and visual encodings, from the color of bars in the RGR, to the use of headers and other means to emphasize relevant information in both text and visualizations. 
% % Finally, informants were in agreement that they needed a high-level description, or as one participant stated, they  \textit{``would want a high-level understanding, with DistilBERT being a high-level representation''}[I06]. This informant went further to suggest that model cards could also link more effectively to other documentation artifacts, such as datasheets, while preserving high-level details in the model card.
% Lastly, participants agreed that a high-level description of the model's purpose was needed (i.e., ``DistilBERT is a sentiment analysis model''). One participant suggested that model cards could integrate more effectively with other documentation artifacts (e.g., datasheets), while preserving the simplicity and high-level descriptions in the model card[I06]. 

% Informants also offered general comments on aesthetics and visual encodings, from the color of bars in the RGR, to the use of headers and other means to emphasize relevant information in both text and visualizations. 
% Four informants proposed placing much greater emphasis on the sample size information that is displayed in the rightmost column of the RGR. One suggested that \textit{``flagging ones where performance is too low, given the sample sizes.''}[I02] would be valuable. 

One of the most significant areas of concern participants raised with respect to information design was a need for more high-level descriptions and summaries across all model cards and subsections within each card. participants agreed that a high-level description of the model's purpose was needed (i.e., ``DistilBERT is a sentiment analysis model''). One participant suggested that model cards could integrate more effectively with other documentation artifacts (e.g., datasheets), while preserving the simplicity and high-level descriptions in the model card[I06]. Most \hl{(n=X)?} participants also pointed out areas in the RGR and IMC where they thought different information should be prioritized or emphasized (e.g., changing the color of the size column (rightmost column) in the RGR or emphasizing it in another way). Lastly, many participants suggested adding or emphasizing higher-level metrics about performance (e.g., making overall performance visually distinct from disaggregated performance). 


In general, participants expressed concern that interaction may be difficult to discover -- this is something that has also been observed in the academic literature~\hl{REF}. However, they did believe that it would be helpful for someone like Jenn to add her own examples and visually explore the data and model performances. However, even though informants felt that the IMC made some design decisions (simplified descriptions, visualizations, and easily ability to add data) could lower barriers for people like Jenn, emphasized that she would still need clear guidance and contextualization.

Finally, two informants raised the concern that \textit{``the developer has to make these model cards, but they are difficult to make, which is why these are not very informative.'' } [I07] and that \textit{``there's too much work getting model cards up''}[I06]. Their perspective underscores the importance of supporting both model card authoring and understandability, which ultimately target multiple (sometimes overlapping) audiences. 


\subsubsection{Guidance} Informants felt that participants need help making sense of an act on the information in the model card. Six informants emphasized the importance of providing specific guidance to help participants understand the information on the model card. This guidance included simple actions like providing definitions, or visual cues in the form of nudges and warnings. One participant felt that explainers for visualizations would be helpful because \textit{``it's pretty but..but what would I do [with it?]''}[I02]. One informant saw the direct potential for using interaction to provide guidance, suggesting that \textit{``would help me [...] dig deeper''} [I00] into the model details.

Other forms of guidance were complex and geared more toward \textit{``help[ing] me understand why this matters [and] how does it help me make more informed decisions?''}[I01]. Supporting interpretability is complex but nearly all (n=7) informants indicated that examples could provide some useful guidance. However, having an effective default example to prompt end-users was also important because \textit{``defaults are complex in language, so what  do you start with?''} [I03]. Another informant suggested that leveraging examples with interactivity could help people like Jenn \textit{``build a better mental model of how the model works and, like, what it lacks.''}[I04].

\subsubsection{Trust and Safety} Ethics and safety considerations resulted in a lively discussion. On our source model card (Section~\ref{sec:studyone_probes}) the ethical considerations text was short, but many informants took exception with the training dataset being described as ``fairly neutral'' (\textit{``what does that mean even?''}[I07]).  One commented that `Silicon Valley' tended to apply a standard set of \textit{``moral values application across global and cultural contexts''}[I06], which diminishes that value of such ethical statements and assessments. Increasingly such statements are seen as a \textit{``cop-out because it just kind of says `there is some bias somewhere' which is not entirely helpful.''}[I05]. Two informants suggested stating explicitly whether bias assessments had been conducted, and one suggested raising a warning if such bias analyses are not run. Several participants also suggested pre-populating the RGR visualization with specific vulnerable populations, making them prominent, and pointed to risk taxonomies that defined such groups. However, one participant cautioned that at-risk or marginalized groups are different across the world, and the default inclusion of such populations is not always meaningful and needs to be customizable to regional contexts. 

\hl{PLACEHOLDER - other warnings, including sample size for performance}

 Four informants proposed placing much greater emphasis on the sample size information that is displayed in the rightmost column of the RGR. One suggested that \textit{``flagging ones where performance is too low, given the sample sizes.''}[I02] would be valuable. 
 

\subsubsection{Sensemaking and Skepticism} The ideas of the previous themes come together as informants discussed the ways they believed end users like Jenn would make sense of, and explore, information in the model cards. Informants tied interaction positively to these themes, indicating that it would be beneficial to \textit{``allow domain experts to be able to interrogate the models and formulate rules that are semantically meaningful to test against the model''{I07]}}. Importantly, the interactivity would enable people to \textit{``elicit more questions'' }[I03] that allowed them to form and test their mental models about the data and better \textit{``see the things that model lacks''}[I04].

\subsubsection{Summary and Implications}
\hl{PLACEHOLDER - Either in this section or in in the overview of the prototype design I think we need to say more about which of these pieces shaped the design and which we take as broader implications. (I have notes for this but haven't integrated them into the text yet)}

